Pushing the Accuracy-Group Robustness Frontier with Introspective Self-play

Standard empirical risk minimization (ERM) training can produce deep neural network (DNN) models that are accurate on average but under-perform in under-represented population subgroups, especially when there are imbalanced group distributions in the long-tailed training data. Therefore, approaches that improve the accuracy-group robustness trade-off frontier of a DNN model (i.e. improving worst-group accuracy without sacrificing average accuracy, or vice versa) is of crucial importance. Uncertainty-based active learning (AL) can potentially improve the frontier by preferentially sampling underrepresented subgroups to create a more balanced training dataset. However, the quality of uncertainty estimates from modern DNNs tend to degrade in the presence of spurious correlations and dataset bias, compromising the effectiveness of AL for sampling tail groups. In this work, we propose Introspective Self-play (ISP), a simple approach to improve the uncertainty estimation of a deep neural network under dataset bias, by adding an auxiliary introspection task requiring a model to predict the bias for each data point in addition to the label. We show that ISP provably improves the bias-awareness of the model representation and the resulting uncertainty estimates. On two real-world tabular and language tasks, ISP serves as a simple "plug-in" for AL model training, consistently improving both the tail-group sampling rate and the final accuracy-fairness trade-off frontier of popular AL methods.

==> figures/cv_ensemble_introspective_self_play_backup.tex <==
\begin{figure}[ht]
\centering
\begin{subfigure}{.24\textwidth}
\includegraphics[trim=1.5cm 0cm 0cm 0cm, width=\linewidth]{figures/self_play_ensemble.png}
\caption{}
\label{fig:self_play_ensemble}
\end{subfigure}
\qquad
\begin{subfigure}{.7\textwidth}
  \centering
  \includegraphics[trim=0.5cm 16cm 6cm 1cm, width=\columnwidth]{figures/introspective_self_play}
  \caption{}
  \label{fig:introspective_self_play}
\end{subfigure}%
\caption{
(\textbf{Left}) An example of 5-fold cross-validated ensemble. Each ensemble member received $60\%$ of the data (highlighted in orange), and each data split receives 3 in-sample $f_{in,k}$ and 2 out-of-sample predictions $f_{out,k}$.
\textbf{(Right)} An illustration of the two-stage \glsfirst{ISP} model.
}
\vspace{-1.5em}
\end{figure}

==> introspective ensemble/figures/2d_example.tex <==
\begin{figure}[ht]
\captionsetup[subfigure]{justification=centering}
\centering
\begin{adjustbox}{minipage=\linewidth,scale=0.9}
\begin{subfigure}{.23\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figures/prediction_introspection.png}
  \caption{Predicted Probability \\ \quad Introspective Training}
  \label{fig:2d_prediction_isp}
\end{subfigure}
%
\begin{subfigure}{.23\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figures/variance_introspection.png}
  \caption{Predictive Variance \\ \quad Introspective Training}
  \label{fig:2d_uncertainty_isp}
\end{subfigure}
%
\begin{subfigure}{.23\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figures/representation_introspection_target.png}
  \caption{Representation Space \\ \quad Introspective Training \\ {\tiny Colored by Predicted Probability.}}
  \label{fig:2d_representation_isp}
\end{subfigure}
%
\begin{subfigure}{.23\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figures/representation_introspection_bias.png}
  \caption{Representation Space \\ \quad Introspective Training \\ {\tiny Colored by Predicted Underrep.}}
  \label{fig:2d_representation_isp_bias}
\end{subfigure}


\begin{subfigure}{.23\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figures/prediction_base.png}
  \caption{Predicted Probability \\ \quad ERM Training}
  \label{fig:2d_prediction_base}
\end{subfigure}
%
\begin{subfigure}{.23\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figures/variance_base.png}
  \caption{Predictive Variance \\ \quad ERM Training}
  \label{fig:2d_uncertainty_base}
\end{subfigure}
%
\begin{subfigure}{.23\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figures/representation_base_target.png}
  \caption{Representation Space \\ \quad ERM Training}
  \label{fig:2d_representation_base}
\end{subfigure}
%
\begin{subfigure}{.23\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figures/bias_introspection.png}
  \caption{Predicted Underreprentation \\ \quad Introspective Training}
  \label{fig:2d_bias_isp}
\end{subfigure}

\caption{Prediction, uncertainty quantification, and representation learning behavior of introspective training v.s. ERM training in a binary classification task under severe group imbalance ($n=5000$) \citep{sagawa2020investigation}. Here, blue and orange indicates the two classes, and each class contains a minority group (the tiny clusters on the diagonal with $n<5$) and a majority group (the large clusters on the off-diagonal).
%
\textbf{Column 1-2} depicts the models' predictive probability and predictive uncertain surface in the data space. 
%
\textbf{Column 3} depicts the models' decision surface in the last-layer representation space, colored by the predictive probability of the target label. \textbf{Column 4} depicts the introspective-trained model's predicted bias probability in the representation space (\cref{fig:2d_representation_isp_bias}) and in the data space (\cref{fig:2d_bias_isp}), colored by the predictive probability of the underrepresentation.
\Cref{sec:exp_2d_app} described further detail.
}
\label{fig:2d_example}
\end{adjustbox}
\vspace{-0.5em}
\end{figure}


==> introspective ensemble/figures/acc_fair_intro.tex <==
\begin{wrapfigure}[12]{R}{0.25\textwidth}
\vspace{-2em}
\centering
\includegraphics[width=0.25\textwidth]{figures/acc_fair_frontier_intro}
\vspace{-2em}
\caption{Example of accuracy-fairness frontier. 
Under a more balanced training data distribution, the model can attain a better accuracy-fairness frontier ({\color{red}\textbf{Red}}) when compared to training under an imbalanced distribution ({\color{blue}\textbf{Blue}}) at every tradeoff level $\lambda$ (\Cref{eq:frontier_risk_intro}).}
\label{fig:acc_fair_frontier_intro}
\end{wrapfigure}


==> introspective ensemble/figures/cv_ensemble_introspective_self_play_backup.tex <==
\begin{figure}[ht]
\centering
\begin{subfigure}{.24\textwidth}
\includegraphics[trim=1.5cm 0cm 0cm 0cm, width=\linewidth]{figures/self_play_ensemble.png}
\caption{}
\label{fig:self_play_ensemble}
\end{subfigure}
\qquad
\begin{subfigure}{.7\textwidth}
  \centering
  \includegraphics[trim=0.5cm 16cm 6cm 1cm, width=\columnwidth]{figures/introspective_self_play}
  \caption{}
  \label{fig:introspective_self_play}
\end{subfigure}%
\caption{
(\textbf{Left}) An example of 5-fold cross-validated ensemble. Each ensemble member received $60\%$ of the data (highlighted in orange), and each data split receives 3 in-sample $f_{in,k}$ and 2 out-of-sample predictions $f_{out,k}$.
\textbf{(Right)} An illustration of the two-stage \glsfirst{ISP} model.
}
\vspace{-1.5em}
\end{figure}

==> introspective ensemble/preamble/acronym.tex <==
\newacronym{DNN}{DNN}{deep neural network}

\newacronym{ISP}{\textsc{Isp}}{\textit{Introspective Self-play}}

\newacronym{KKT}{KKT}{Karush–Kuhn–Tucker}

\newacronym{ERM}{ERM}{empirical risk minimization}

\newacronym{JTT}{JTT}{Just Train Twice}

\newacronym{IRM}{IRM}{\textit{Invariant Risk Minimization}}

\newacronym{DRO}{DRO}{Distributionally Robust Optimization}

\newacronym{SSA}{SSA}{Spread Spurious Attribute}

\newacronym{ML}{ML}{machine learning}



\newacronym{MCD}{MCD}{Monte Carlo Dropout}

\newacronym{AL}{AL}{active learning}

\newacronym{DE}{DE}{Deep Ensemble}

\newacronym{GP}{GP}{Gaussian process}

\newacronym{OOD}{OOD}{out-of-domain}

\newacronym{BALD}{BALD}{Bayesian active learning by disagreement}

\newacronym{BADGE}{BADGE}{Batch Active learning by Diverse Gradient Embeddings}

\newacronym{CDF}{CDF}{cumulative distribution function}

\newacronym{GCE}{GCE}{generalized cross entropy}

\newacronym{FL}{FL}{focal loss}


==> introspective ensemble/preamble/definition.tex <==
% \newtheoremstyle{tight}
%   {\topsep}   % ABOVESPACE
%   {\topsep}   % BELOWSPACE
%   {\itshape}  % BODYFONT
%   {0pt}       % INDENT (empty value is the same as 0pt)
%   {\bfseries} % HEADFONT
%   {.}         % HEADPUNCT
%   {5pt plus 1pt minus 1pt} % HEADSPACE
%   {}          % CUSTOM-HEAD-SPEC  
% \theoremstyle{tight}

% for appendix theorems
\newtheorem{theorem_app}{Theorem}[section]

\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}

\newtheorem{assumption}{Assumption}
\newtheorem{proposition}{Proposition}
\newtheorem{corollary}{Corollary}[theorem]
\newtheorem{corollary_prop}{Corollary}[proposition]

\newtheorem{definition}{Definition}

% redefine footnote symbol to avoid confusion in math mode
% \renewcommand\thefootnote{\fnsymbol{footnote}}

\makeatletter
\newcommand*{\addFileDependency}[1]{% argument=file name and extension
  \typeout{(#1)}
  \@addtofilelist{#1}
  \IfFileExists{#1}{}{\typeout{No file #1.}}
}
\makeatother

\newcommand*{\myexternaldocument}[1]{%
    \externaldocument{#1}%
    \addFileDependency{#1.tex}%
    \addFileDependency{#1.aux}%
}

\AtAppendix{\counterwithin{proposition}{section}}

% optimization operator.
\DeclareMathOperator*{\minimize}{minimize}

% Algorithm
\algnewcommand{\LeftComment}[1]{\Statex \(\triangleright\) #1}


\algnewcommand{\Inputs}[1]{%
  \State \textbf{Inputs:} #1
  % \Statex \hspace*{\algorithmicindent}\parbox[t]{.8\linewidth}{\raggedright #1}
}
\algnewcommand{\Output}[1]{%
  \State \textbf{Output:} #1
  % \Statex \hspace*{\algorithmicindent}\parbox[t]{.8\linewidth}{\raggedright #1}
}
\algnewcommand{\Outputs}[1]{%
  \State \textbf{Outputs:} #1
  % \Statex \hspace*{\algorithmicindent}\parbox[t]{.8\linewidth}{\raggedright #1}
}
\algnewcommand{\Compute}[1]{%
  \State \textbf{Compute} #1
  % \Statex \hspace*{\algorithmicindent}\parbox[t]{.8\linewidth}{\raggedright #1}
}
\algnewcommand{\Initialize}[1]{%
  \State \textbf{Initialize:} #1
  % \Statex \hspace*{\algorithmicindent}\parbox[t]{.8\linewidth}{\raggedright #1}
}
\algnewcommand{\OpEstimate}[1]{%
  \State \textbf{(Optional) Estimate:} #1
  % \Statex \hspace*{\algorithmicindent}\parbox[t]{.8\linewidth}{\raggedright #1}
}
\algnewcommand{\Estimate}[1]{%
  \State \textbf{Estimate:} #1
  % \Statex \hspace*{\algorithmicindent}\parbox[t]{.8\linewidth}{\raggedright #1}
}
\algnewcommand{\Infer}[1]{%
  \State \textbf{Infer:} #1
  % \Statex \hspace*{\algorithmicindent}\parbox[t]{.8\linewidth}{\raggedright #1}
}

% Table spacing
\setlength\doublerulesep{0.25em} 


==> introspective ensemble/preamble/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}
\def\valpha{{\bm{\alpha}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> introspective ensemble/preamble/packages.tex <==
\usepackage[acronym,nowarn,section,nonumberlist]{glossaries}
\usepackage{lipsum}  

\usepackage[utf8]{inputenc} % allow utf-8 input
%\usepackage[T1]{fontenc}    % use 8-bit T1 fonts

\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{wrapfig}

% Set space.
\usepackage[nodisplayskipstretch]{setspace}

% Use fancyhdr package
\RequirePackage{multicol}
\RequirePackage{multirow}
\RequirePackage{colortbl}
\RequirePackage{fancyhdr}
\RequirePackage{color}


\RequirePackage{algorithm}
\RequirePackage{algorithmicx}
\usepackage[noend]{algpseudocode}

%\usepackage{algorithm}
%\usepackage{algorithmicx}
%\usepackage{algpseudocode}
\RequirePackage{natbib}
\RequirePackage{eso-pic} % used by \AddToShipoutPicture 
\RequirePackage{forloop}

% Recommended, but optional, packages for figures and better typesetting:
\usepackage{microtype}
\usepackage{graphicx}
\usepackage[export]{adjustbox}

\usepackage[font=scriptsize]{caption}
\usepackage{subcaption}
\usepackage{booktabs} % for professional tables
\usepackage{draftfigure}

\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{mathtools}
\usepackage{amsfonts}
\usepackage{mathptmx}
\usepackage{soul}

%\usepackage{lipsum}

% hyperref makes hyperlinks in the resulting PDF.
% If your build breaks (sometimes temporarily if a hyperlink spans a page)
% please comment out the following usepackage line and replace
% \usepackage{icml2019} with \usepackage[nohyperref]{icml2019} above.
%\usepackage{color}
% \usepackage[dvipsnames,table]{xcolor}
% \definecolor{mydarkblue}{rgb}{0,0.08,0.45}
% \usepackage[colorlinks,citecolor=mydarkblue,urlcolor=mydarkblue,linkcolor=mydarkblue
% ]{hyperref}
%\usepackage{hyperref}
\usepackage{cleveref}
\usepackage{comment}
\usepackage[hang,flushmargin]{footmisc}
      % hyperlinks
\usepackage{url}
% 
\def\UrlBreaks{\do\/\do-}
\usepackage{breakurl}% simple URL typesetting
%

% Attempt to make hyperref and algorithmic work together better:
%\newcommand{\theHalgorithm}{\arabic{algorithm}}

% use glossary
\usepackage
[acronym,nowarn,section,nonumberlist]{glossaries}
\glsdisablehyper{}

% import external document
\usepackage{xr}


% theorem
% adding two lines to avoid conflict in package https://tex.stackexchange.com/questions/43835/conflict-between-amsthm-and-some-other-package
\let\proof\relax
\let\endproof\relax
\usepackage{amsthm}
\usepackage{apptools}

% custom toc
\usepackage[page,header]{appendix}
\usepackage{titletoc}
\usepackage{etoc}

% itemize environment
\usepackage{enumitem}


==> introspective ensemble/proof/lemma_1.tex <==
\begin{lemma}[Optimal Group-size Allocation for Weighted Population Risk]
For an objective function that is the weighted combination of group-specific risk:
$$R_w(\alpha, n)= \sum_{g \in \gG} w_g * R(f_{D_{\alpha,n}}|G=g)$$
where $w=\{w_g\}_{g\in \gG}$ are non-negative weights. 
Furthermore, under Assumption \ref{def:group_scaling_law}, $R_w(\alpha, n)$ is approximated by the weighted sum of approximated group risks $\hat{R}(\alpha, n|G=g)=r(\alpha_g n, n | c_g, \tau_g, \delta_g, p_g, q_g)$:
\begin{align}
\hat{R}_w(\alpha, n)
\coloneqq
\sum_{g \in \gG} w_g * \hat{R}(\alpha, n|G=g)
= \sum_{g \in \gG} w_g * 
\big( c_g * (\alpha_g  n)^{-p_g} + \tau_g * n^{-q_g} + \delta_g \big).
\label{eq:approx_weighted_risk}
\end{align}
Then, 
\begin{itemize}[leftmargin=0.5cm]
\item [(1)] When $p_g = p$ is equal for all groups, the optimal allocation $\alpha^*$ that
minimizes the approximated weighted risk (\ref{eq:approx_weighted_risk}) is:
\begin{align}
\alpha^*_g = 
\frac{(w_g c_g)^{1/(p+1)} }
{\sum_{g\in \gG}(w_g c_g)^{1/(p+1)}}.
\label{eq:simple_allocation_weighted_risk}
\end{align}

\item [(2)] When $p_g$ is allowed to differ by group, the optimal allocation $\alpha^*$ that
minimizes the approximated weighted risk (\ref{eq:approx_weighted_risk}) is:
\begin{align}
\alpha^*_g = 
\frac{(w_g c_g p_g n^{-p_g})^{1/(p_g+1)} }
{\sum_{g\in \gG}(w_g c_g p_g n^{-p_g})^{1/(p_g+1)}}.
\label{eq:general_allocation_weighted_risk}
\end{align}
That is, as $n \rightarrow \infty$, the sample size allocation disproportionally lean towards the group that has the slowest learning rate on the exponential scale (i.e., the group with the smallest $p_g$).
\end{itemize}
\label{thm:allocation_weighted_risk}
\end{lemma}


==> introspective ensemble/proof/lemma_1_proof.tex <==
\begin{proof} The proof is a generalization of Proposition 2 of \citep{rolf2021representation}), where the exponential scaling coefficient $p_g$ is allowed to vary by group, and the weights  $\{w_g\}_{g\in \gG}$ are no longer required to sum to 1. Specifically, note that in (\ref{eq:approx_weighted_risk}), the terms $\tau_g * n^{-q_g} + \delta_g$ does not depend on $\alpha$. Then, restricting $\alpha \in (0, 1)^{|\gG|}$, the optimization problem can be expressed as:
\begin{align*}
\mbox{minimize}_{\alpha} \quad & \sum_{g \in \gG} w_g c_g  (\alpha_g n)^{-p_g}
\\
\mbox{subject to} \quad & \sum_{g \in \gG} \alpha_g = 1.
\end{align*}
Notice that the main objective function is convex in $\alpha=[\alpha_1, \dots, \alpha_{|\gG|}]$. Then, the \gls{KKT} conditions of this constrained optimization problem is:
\begin{align*}
    w_g c_g p_g n^{-p_g} (\alpha_g)^{-(p_g+1)}  &= \lambda 
    \qquad g \in \gG \\
    \sum_{g \in \gG} \alpha_g &= 1.
\end{align*}
Solving the first condition leads to $\alpha_g^* \propto (w_g c_g p_g n^{-p_g})^{1/(p_g+1)}$. This, combined with the second condition, implies that the final solution is of the form (\ref{eq:general_allocation_weighted_risk}):
\begin{align*}
    \alpha^*_g &= \frac{(w_g c_g p_g n^{-p_g})^{1/(p_g+1)} }
    {\sum_{g \in \gG} (w_g c_g p_g n^{-p_g})^{1/(p_g+1)} }.
\end{align*}
Finally,  when $p_g = p$, (\ref{eq:simple_allocation_weighted_risk}) can be derived from (\ref{eq:general_allocation_weighted_risk}) by setting $p_g=p$ and eliminate the multiplicative factor $p_g n^{-p_g}=p n^{-p}$ that is shared by every term in the numerator and the denominator.
\end{proof}


==> introspective ensemble/proof/lemma_2.tex <==
\begin{lemma}[Optimal Group-size Allocation for Worst-case Risk]
For an objective function that is the adversarially-weighted, worst-case risk:
$$R_v(\alpha, n)= \sup_v \sum_{g \in \gG} v_g * R(f_{D_{\alpha,n}}|G=g)$$
where $v=\{v_g\}_{g\in \gG}$ are non-negative weights for group-specific risks that sum to 1. 
Furthermore, under Assumption \ref{def:group_scaling_law}, $R_v(\alpha, n)$ is approximated by the adversarial weighting the the approximated group risks $\hat{R}(\alpha, n|G=g)=r(\alpha_g n, n | c_g, \tau_g, \delta_g, p_g, v_g)$:
\begin{align}
\hat{R}_v(\alpha, n)
\coloneqq
\sup_v \sum_{g \in \gG} v_g * \hat{R}(\alpha, n|G=g)
= \sup_v \sum_{g \in \gG} v_g * 
\big( c_g * (\alpha_g  n)^{-p_g} + \tau_g * n^{-q_g} + \delta_g \big).
\label{eq:approx_worst_risk}
\end{align}
Then, 
\begin{enumerate}[leftmargin=0.5cm]
\item [(1)] When the group-specific risk share the same $p_g=p, q_g=q, \tau_g=\tau, \delta_g=\delta$ across all groups (i.e., the group-specific risks $c_g n_g^{-p} + \tau n^{-q} + \delta$ differ only by the multiplicative scaling coefficient $c_g$), the optimal allocation to minimize the approximated adversarial risk (\ref{eq:approx_worst_risk}) is:
\begin{align}
\alpha^*_g = 
\frac{c_g^{1/p} }
{\sum_{g\in \gG} c_g^{1/p}}; 
% \quad 
% v^*_g=\frac{c_g^{1/p}}{\sum_{g\in \gG} c_g^{1/p}}.
\label{eq:simple_allocation_worst_risk}
\end{align}
% {\color{red} TODO: need to correct: $v_g^*$ solution is not unique when $\alpha=\alpha^*$.}
\item [(2)] When $p_g=p$ are shared by all groups (i.e., the group-specific risks $c_g n_g^{-p} + \tau_g * n^{-q_g} + \delta_g$ share the exponential scaling coefficient $p$), the optimal allocation to minimize the approximated adversarial risk is:
\begin{align}
\alpha^*_g = 
\frac{(c_g l_g)^{1/p} }
{\sum_{g\in \gG} (c_g l_g)^{1/p}}; 
% \quad 
% v^*_g=\frac{c_g^{1/p} \, l_g^{(p+1)/p}}{\sum_{g\in \gG} c_g^{1/p} \, l_g^{(p+1)/p}},
\label{eq:full_allocation_worst_risk}
\end{align}
where $l_g = (\lambda - (\tau_g n^{-q_g} + \delta_g))^{-1}$ is a group-specific non-negative coefficient, in which $\lambda$ is a positive constant that solves the implicit equation $\sum_g (c_g l_g^{p+1})^{1/p} = \Big[ n * \sum_g (c_g l_g)^{1/p} \Big]^{(p+1)/2}$.
\end{enumerate}
\label{thm:allocation_worst_risk}
\end{lemma}


==> introspective ensemble/proof/lemma_2_proof.tex <==
\begin{proof}
Minimizing the approximated worst-group risk (\ref{eq:approx_worst_risk}) is equivalent to solving a minimax problem. Specifically, first write the object function as $$H(\alpha, v) \coloneqq \sum_{g \in \gG} v_g * r(\alpha_g n, n | c_g, \tau_g, \delta_g, p_g, v_g).$$ 
As shown, $H(\alpha, v)$ is a function of both the risk allocation parameter $v$ and the group-size allocation $\alpha$, note that $\hat{R}_v(\alpha, n) = \sup_v H(\alpha, v)$. Also recall that $\alpha \in (0, 1)^{|\gG|}$ and $v_g > 0 \; \forall g$. Then, the optimal value of (\ref{eq:approx_worst_risk}) can be written as:
\begin{align}
    \inf_\alpha \; \hat{R}_v(\alpha, n) = \inf_{\alpha} \sup_v \; H(\alpha, v).
    \label{eq:worst_risk_primal}
\end{align}
Notice that (\ref{eq:worst_risk_primal}) is of a min-max form, this motivates us to derive the dual formulation of the problem, which is often easier to solve. Specifically, notice that the objective function $H(\alpha, v)$ is a convex-concave function which is concave (i.e., linear) in $v$ and convex in $\alpha$ (since $\nabla^2_\alpha H(\alpha, v) =diag_g \big[ p_g (p_g+1) v_g c_g n_g^{-p_g} \alpha_g^{-(p_g+2)} \big] \succeq 0$ is a positive-definite $|\gG| \times |\gG|$ matrix for every $v$). Then, by the max-min equality of the convex-concave function (see, e.g., Exercise 5.25 of \citet{boyd2004convex}, or the Proof of the Proposition 1 of \citet{sagawa2019distributionally}), we have:
\begin{align}
    \inf_{\alpha} \sup_v \; H(\alpha, v) = \sup_v \inf_{\alpha} \; H(\alpha, v),
    \label{eq:worst_risk_dual}
\end{align}
which implies that there exists a saddle point $(\alpha^*, v^*)$ such that $\inf_\alpha \; H(\alpha, v^*) = H(\alpha^*, v^*) = \sup_v \; H(\alpha^*, v)$.

We can now solve (\ref{eq:worst_risk_primal}) by solving the dual problem  (\ref{eq:worst_risk_dual}), i.e., $\sup_v \inf_{\alpha} \; H(\alpha, v)$. First solve the inner problem $\inf_{\alpha} \; H(\alpha, v)$, i.e.,
\begin{align*}
\mbox{minimize}_{\alpha} \quad &  
H(\alpha, v) =\sum_{g \in \gG} v_g c_g  (\alpha_g n)^{-p_g}
\\
\mbox{subject to} \quad & \sum_{g \in \gG} \alpha_g = 1; \quad \alpha_g > 0 \; \forall g \in \gG
\end{align*}
This is equivalent to minimizing a weighted population risk with weights $v=\{v_g\}_{g \in \gG}$. Under the setting $p_g=p$ is equal for all groups, by \Cref{thm:allocation_weighted_risk}, we have that the optimal solution is:
\begin{align}
\alpha^*_g = 
\frac{(v_g c_g)^{1/(p+1)} } {\sum_{g\in \gG}(v_g c_g)^{1/(p+1)}}.
\label{eq:lemma2_inner_problem_sol}
\end{align}

To obtain a concrete expression of $\alpha^*_g$ (i.e., not in terms of the group allocation $v_g$), we need to solve for the for the outer problem $\sup_v H(\alpha^*, v)$ in order to obtain an expression for the group allocation $v^*$. Specifically, under the expression of $\alpha^*$, the optimal risk $\inf_\alpha H(\alpha, v)=H(\alpha^*, v)$ takes the form:
\begin{align}
\nonumber
H(\alpha^*, v) &= 
\sum_{g\in \gG} v_g \Big[  
c_g \big(
\frac{(v_g c_g)^{1/(p+1)}}{\sum_g (v_g c_g)^{1/(p+1)}} n
\big)^{-p} 
+ \tau_g n^{-q_g} + \delta_g
\Big]\\ 
\nonumber
&=
\sum_{g\in \gG} v_g \Big[  
c_g \big(
\frac{(v_g c_g)^{1/(p+1)}}{\sum_g (v_g c_g)^{1/(p+1)}} n
\big)^{-p} 
\Big]
+ 
\sum_{g\in \gG} v_g \Big[  
\tau_g n^{-q_g} + \delta_g
\Big]\\ 
\nonumber
&=
\big[ 
n^{-1} 
\sum_{g\in \gG} (v_g c_g)^{1/(p+1)}
\big]^p
\big[ 
\sum_{g\in \gG} 
(v_g c_g)^{1/(p+1)}
\big]
+ 
\sum_{g\in \gG} v_g \Big[  
\tau_g n^{-q_g} + \delta_g
\Big]\\
&=
n^{-p} 
\Big[ 
\sum_{g\in \gG} (v_g c_g)^{1/(p+1)}
\Big]^{(p+1)}
+ 
\sum_{g\in \gG} v_g \Big[  
\tau_g n^{-q_g} + \delta_g
\Big].
\label{eq:lemma2_outer_problem}
\end{align}
Then, solving for $\inf_v H(\alpha^*, v)$ subject to $\sum_g v_g = 1$ yields the \gls{KKT} conditions:
\begin{align}
n^{-p} \Big[ \sum_{g\in \gG} (v_g c_g)^{1/(p+1)} \Big]^p * c_g^{1/(p+1)}  * v_g^{-p/(p+1)} + (\tau_g n^{-q_g} + \delta_g) = \lambda;
\qquad 
\sum_{g \in \gG} v_g = 1.
\label{eq:lemma2_outer_problem_kkt}
\end{align}
\todo{\color{red} TODO: cover the case $v$ on the edge of the simplex so that $v_g=0$.}

Now denote $l_g = (\lambda - (\tau_g n^{-q_g} + \delta_g))^{-1}$, a simple rearrangement of terms in (\ref{eq:lemma2_outer_problem_kkt}) reveals that:
\begin{align}
\nonumber
v_g 
&= 
\Big[ n^{-1} \sum_{g\in \gG} (v_g c_g)^{1/(p+1)} \Big]^{p+1} *
\Big[ \frac{c_g^{1/p}}{(\lambda - (\tau_g n^{-q_g} + \delta_g))^{(p+1)/p}} \Big] 
\\
&= 
\Big[ n^{-1} \sum_{g\in \gG} (v_g c_g)^{1/(p+1)} \Big]^{p+1} *
\Big[ c_g^{1/p} * l_g^{(p+1)/p} \Big]
\label{eq:lemma2_outer_problem_sol}
\\ \nonumber
&\propto 
c_g^{1/p} l_g^{(p+1)/p},
\end{align}
which combined with the condition $\sum_{g \in \gG} v_g = 1$ implies $v^*_g = \frac{c_g^{1/p} l_g^{(p+1)/p}}{\sum_{g\in \gG c_g^{1/p} l_g^{(p+1)/p}}}$. 

Now, since (\ref{eq:lemma2_inner_problem_sol})-(\ref{eq:lemma2_outer_problem_sol}) are derived under the condition $p_g=p \; \forall g$, we are ready to obtain the expression of $\alpha^*$ for the second part of \Cref{thm:allocation_worst_risk} (i.e., \Cref{eq:full_allocation_worst_risk}). Specifically, obtain the expression for $\alpha^*$ by plugging the expression of $v^*_g$ into (\ref{eq:lemma2_inner_problem_sol}):
\begin{align}
\alpha^*_g 
= 
\frac{(v_g c_g)^{1/(p+1)} } {\sum_{g\in \gG}(v_g c_g)^{1/(p+1)}}
=
\frac{(c_g l_g)^{1/p} } {\sum_{g\in \gG}(c_g l_g)^{1/p}}.
\label{eq:full_allocation_worst_risk_proof}
\end{align}
Furthermore, (\ref{eq:lemma2_outer_problem_sol}) combined with $\sum_g v_g = 1$ and the expression $v^*_g = \frac{c_g^{1/p} l_g^{(p+1)/p}}{\sum_{g\in \gG} c_g^{1/p} l_g^{(p+1)/p}}$ implies that
\begin{align*}
\sum_{g \in \gG} c_g^{1/p} l_g^{(p+1)/p} 
= \Big[ n^{-1} \sum_{g\in \gG} (v_g c_g)^{1/(p+1)} \Big]^{-(p+1)} 
= \Big[n * \sum_{g\in \gG} (v_g c_g)^{1/(p+1)} \Big]^{p+1} 
= \frac{1}{\sum_{g\in \gG} c_g^{1/p} l_g^{(p+1)/p}} * 
\Big[ n \sum_{g \in \gG}
(c_g l_g)^{1/p}
\Big]^{p+1},
\end{align*}
which implies:
\begin{align*}
\sum_{g \in \gG} (c_g l_g^{(p+1)})^{1/p} &= \Big[ n \sum_{g \in \gG}
(c_g l_g)^{1/p}
\Big]^{(p+1)/2}.
\end{align*}

Finally, we derive the first part of \Cref{thm:allocation_worst_risk}, which is a special case. Notice that under the condition that $(p_g=p, q_g=q, \tau_g=\tau, \delta_g=\delta)$ is the same across groups, $l_g = (\lambda - (\tau_g n^{-q_g} + \delta_g))^{-1}$ are also the same across all groups, and can be cancelled out from the nominator and the denominator of (\ref{eq:full_allocation_worst_risk_proof}), which leads to the expressions in (\ref{eq:simple_allocation_worst_risk}), i.e., $\alpha^*_g = \frac{(c_g)^{1/p} } {\sum_{g\in \gG}(c_g)^{1/p}}$ and $v^*_g = \frac{(c_g)^{1/p} } {\sum_{g\in \gG}(c_g)^{1/p}}$.
\end{proof}


==> introspective ensemble/proof/prop_app_1.tex <==
\begin{proposition}[Optimal Allocation for the Accuracy-Fairness Frontier]

Given a data distribution $\gD$ with prevalence of each group as $\{\gamma_g\}_{g \in \gG}$. Recall $D_{\alpha, n}$ is a size-$n$ dataset with group size allocation $\alpha=\{\alpha_g\}_{g \in \gG}$, $\hat{f}_{D_{\alpha, n}}$ is a model trained on $D_{\alpha, n}$. Finally, denote the population-level risk of $\hat{f}_{D_{\alpha, n}}$ when evaluated on $\gD$ as: 
$$R(\alpha, n) = \sum_{g\in \gG} \gamma_g E[R(\hat{f}_{D_{\alpha, n}} | G=g)].$$
where the expectation is over the randomness in $g \in \gG$. Recall that the accuracy-fairness frontier risk can be expressed as:
$$F_{\omega}(\alpha, n) \coloneqq 
\omega * R(\alpha, n) + \omega_2 * (\alpha, n),$$


\begin{comment}
where $\omega =[\omega_1, \omega_2] > \mathbf{0}$ are finite positive constants. $R_{fair}$ is a \textit{``fairness" risk} which can be the average-group risk 
$$\bar{R}(\alpha, n) \coloneqq \frac{1}{|\gG|} \sum_{g\in \gG} R(f_{D_{\alpha, n}}|G=g)$$ or the worst-case risk 
$$\tilde{R}(\alpha, n) \coloneqq \sup_v \sum_{g\in \gG} [ v_g R(f_{D_{\alpha, n}}|G=g)].$$ 
Assuming the group-specific generalization-error scaling laws (Definition \ref{def:group_scaling_law}) share the same exponential scaling coefficient $p_g=p$, we have:
\begin{itemize}[leftmargin=0.5cm]
\item [(1)] \textbf{(Average-group Risk)} Let $R_{fair}$ be the average-group risk $\bar{R}(\alpha, n)$. Also denote the approximated average-case risk as
$\hat{\bar{R}}(\alpha, n) = \frac{1}{|\gG|} \sum_{g\in \gG} \hat{R}(\alpha, n|G=g)$.
Then, to minimizes the approximated accuracy-fairness frontier under the average-group risk
\begin{align}
\hat{F}_{\omega}(\alpha, n)=\omega_1 \hat{R}(\alpha, n) + \omega_2 \hat{\bar{R}}(\alpha, n),
\label{eq:approx_average_group_frontier}
\end{align}
the optimal training-set group allocation $\alpha$ is:
\begin{align*}
\alpha^*_g = 
\frac{[\omega_1  \gamma_g c_g + \omega_2  \frac{1}{|\gG|} c_g]^{1/(p+1)}}
{\sum_{g\in \gG}
[\omega_1 \gamma_g c_g + \omega_2 \frac{1}{|\gG|} c_g]^{1/(p+1)}
}.
\end{align*}
\item [(2)] \textbf{(Worst-case Risk)} Let $R_{fair}$ be the worst-case risk 
$\tilde{R}(\alpha, n)$, where $\sum_g v_g = 1$ and $v_g > 0 \; \forall g \in \gG$. 
Also denote the approximated worst-case risk $\hat{\tilde{R}}(\alpha, n) \coloneqq \sup_v \sum_{g\in \gG} [ v_g \hat{R}(\alpha, n|G=g)]$.
Then, to minimizes the approximated accuracy-fairness frontier under the worst-case risk
\begin{align}
\hat{F}_{\omega}(\alpha, n)=\omega_1 \hat{R}(\alpha, n) + \omega_2 \hat{\tilde{R}}(\alpha, n).
\label{eq:approx_worst_case_frontier}
\end{align}
The optimal training-set group allocation $\alpha$ should satisfy:
\begin{align*}
\alpha^*_g = \frac{(r_g c_g)^{1/(p+1)}}{\sum_{g\in \gG} (r_g c_g)^{1/(p+1)}}, 
\quad \mbox{where} \quad
r_g = \max\Big[
\gamma_g, \;\;
\Big(\frac{\omega_2 + \omega_1\sum_{g \in \gB} \gamma_{g}}
{\omega_1} \Big)\Big( \frac{c_g^{1/p} l_{g,\omega}^{(p+1)/p}}{\sum_{g \in \gB} c_g^{1/p} l_{g,\omega}^{(p+1)/p}}\Big) \Big].
\end{align*}
Here, $l_{g,\omega}=(\lambda - \omega_2(\tau_g n^{-q_g} + \delta_g)))^{-1}$, where $\lambda$ is a large positive constant that solves $\sum_{g \in \gG} 
\max\Big(
0, \;
\omega_2^{1/p}
\big[ n^{-1} \sum_{g\in \gG} (\eta_g c_g)^{1/(p+1)} \big]^{p+1}
 \, c_g^{1/p} l_{g,\omega}^{(p+1)/p}
- 
\frac{\omega_1}{\omega_2}
\gamma_g
\Big)=1$. Finally, $\gB \subseteq \gG$ is the set of under-represented groups that needs to be upsampled in the training data to minimize the accuracy-fairness frontier $F_\omega$. Specifically, for every $g \in \gB$, its population prevalence $\gamma_g$ is bounded by 
\begin{align}
\gamma_g < ( \frac{\omega_2}{\omega_1} + \sum_{g \in \gB} \gamma_g) * 
\frac{c_g^{1/p} l_{g,\omega}^{(p+1)/p}}{\sum_{g \in \gB} c_g^{1/p} l_{g,\omega}^{(p+1)/p}}.
\label{eq:minority_group_criteria}
\end{align}
\end{itemize}
\end{comment}

\label{thm:optimal_allocation_frontier_full}
\end{proposition}



==> introspective ensemble/proof/prop_app_1_proof.tex <==
\begin{proof} First prove (1) (\textbf{Averge-group Risk}). 

First notice that the empirical population risk can be expressed as $\hat{R}(\alpha, n)=\sum_g \gamma_g \hat{R}(\alpha, n | G=g)$, where $\gamma_g=E_{\gD}(G=g)$ is the population prevalence of each group under the empirical distribution. Then, the fairness-accuracy frontier under the approximated average-group risk (\ref{eq:approx_average_group_frontier}) can be expressed as a weighted sum of group-specific risks:
\begin{align*}
\hat{\bar{R}}(\alpha, n) = \sum_{g\in \gG} w_g \hat{R}(\alpha, n|G=g)   
\quad \mbox{where} \quad 
w_g = \omega_1 \gamma_g + \omega_2 \frac{1}{|\gG|}.
\end{align*}
Then, by \Cref{thm:allocation_weighted_risk}, the optimal training-set allocation $\alpha^*$ that minimizes the approximated average-group risk is:
\begin{align*}
\alpha^*_g = 
\frac{(w_g c_g)^{1/(p+1)} }
{\sum_{g\in \gG}(w_g c_g)^{1/(p+1)}}
\quad \mbox{where} \quad 
w_g = \omega_1 \gamma_g + \omega_2 \frac{1}{|\gG|},
\end{align*}
which concludes the proof.



Now prove (2) (\textbf{Worst-case Risk}). 

Notice that the fairness-accuracy frontier under the approximated worst-case risk (\ref{eq:approx_worst_case_frontier}) can be expressed as the adversarial weighting of group-specific risks $\hat{R}(\alpha, n|G=g)$ under a simplex constraint:
\begin{align*}
\hat{\tilde{R}}(\alpha, n) = \sup_v \sum_{g\in \gG} (\omega_1 \gamma_g + \omega_2 v_g ) * \hat{R}(\alpha, n|G=g)   
\quad \mbox{where} \quad 
v \geq \mathbf{0}, \; \sum_g v_g = 0 \; \forall g.
\end{align*}
Consequently, analogous to \Cref{thm:allocation_worst_risk}, finding the optimal allocation $\alpha$ for $\hat{\tilde{R}}(\alpha, n)$ is equivalent to solving a minimax problem $\inf_{\alpha} \sup_v H(\alpha, v)$ with respect to the objective function 
$$H(\alpha, v) = (\omega_1 \gamma_g + \omega_2 v_g ) * \hat{R}(\alpha, n|G=g).$$
Notice that $H(\alpha, v)$ is a convex-concave function that is convex in $\alpha=[\alpha_1, \dots, \alpha_{|\gG|}]$ (since it is a linear sum of $\hat{R}(\alpha, n|G=g)=c_g * (\alpha_g  n)^{-p} + \tau_g * n^{-q_g} + \delta_g$ which is a convex function of $\alpha_g$ for every $g$) and concave (linear) in $v=[v_1, \dots, v_{|\gG|}]$. By the max-min equality of the convex-concave function (see, e.g., Exercise 5.25 of \citet{boyd2004convex}, or the Proof of the Proposition 1 of \citet{sagawa2019distributionally}), we have:
\begin{align}
    \inf_{\alpha} \sup_v \; H(\alpha, v) = \sup_v \inf_{\alpha} \; H(\alpha, v),
    \label{eq:worst_risk_frontier_dual}
\end{align}
which implies that there exists a saddle point $(\alpha^*, v^*)$ such that $\inf_\alpha \; H(\alpha, v^*) = H(\alpha^*, v^*) = \sup_v \; H(\alpha^*, v)$.

Consequently, we can find $\alpha^*$ by solving the dual problem on the right-hand side of (\ref{eq:worst_risk_frontier_dual}). First solve the inner problem $\inf_{\alpha} H(\alpha, v)$, which is equivalent to solving:
\begin{align*}
\mbox{minimize}_{\alpha} \quad &  
H(\alpha, v) =\sum_{g \in \gG} (\omega_1 \gamma_g + \omega_2 v_g ) c_g  (\alpha_g n)^{-p} + const.
\\
\mbox{subject to} \quad & \sum_{g \in \gG} \alpha_g = 1; \quad \alpha_g > 0 \; \forall g \in \gG
\end{align*}
where we have ignored the additive constant terms that do not involve $\alpha$. This is equivalent to minimizing a weighted population risk with weights $\eta_g= \omega_1 \gamma_g + \omega_2 v_g$. Under the setting where $p_g=p$ is equal for all groups, by \Cref{thm:allocation_weighted_risk}, the optimal solution of $\alpha$ is:
\begin{align}
\alpha^*_g = 
\frac{(\eta_g c_g)^{1/(p+1)} } {\sum_{g\in \gG}(\eta_g c_g)^{1/(p+1)}},
\quad \mbox{where} \quad
\eta_g= \omega_1 \gamma_g + \omega_2 v_g.
\label{eq:prop_inner_problem_sol}
\end{align}
This allows us to derive the expression for $\inf_\alpha H(\alpha, v)=H(\alpha^*, v)$, i.e.:
\begin{align*}
    H(\alpha^*, v) &= \sum_{g \in \gG} \eta_g \big[ 
    c_g  (\alpha_g^* n)^{-p}  + \tau_g * n^{-q_g} + \delta_g \big] 
    \\
    &= \sum_{g \in \gG} \eta_g \big[ c_g  (\alpha_g^* n)^{-p}  \big] + 
    \sum_{g \in \gG} \eta_g  \big[ \tau_g * n^{-q_g} + \delta_g \big]
    \\
    &= \sum_{g \in \gG} \eta_g \big[ 
    c_g  (\frac{(\eta_g c_g)^{1/(p+1)} } {\sum_{g\in \gG}(\eta_g c_g)^{1/(p+1)}} n)^{-p}  
    \big] + 
    \sum_{g \in \gG} \eta_g  \big[ \tau_g * n^{-q_g} + \delta_g \big]
    \\
    &=  n^{-p} \Big[\sum_{g\in \gG}(\eta_g c_g)^{1/(p+1)} \Big]^{p+1}
     + 
    \sum_{g \in \gG} \eta_g  \big[ \tau_g * n^{-q_g} + \delta_g \big],
\end{align*}
with derivative (recall $\eta_g= \omega_1 \gamma_g + \omega_2 v_g$):
\begin{align}
\nonumber
\frac{\partial}{\partial v_g} 
H(\alpha^*, v)
&= 
n^{-p} *
\frac{\partial}{\partial v} \Big[
\sum_{g\in \gG}(\eta_g c_g)^{1/(p+1)} \Big]^{p+1} + 
\sum_{g \in \gG} \frac{\partial}{\partial v}  \eta_g  \big[ \tau_g * n^{-q_g} + \delta_g \big]
\\
&=
\omega_2 \, n^{-p}
\Big[ \sum_{g\in \gG} (\eta_g c_g)^{1/(p+1)} \Big]^p * c_g^{1/(p+1)} \eta_g^{-p/(p+1)} + 
\omega_2 \, (\tau_g n^{-q_g} + \delta_g)
.
\label{eq:H_deriv}
\end{align}

Now, we are ready to solve the outer problem $\sup_v H(\alpha^*, v)$ of the dual problem in (\ref{eq:worst_risk_frontier_dual}), which is equivalent to solving:
\begin{align*}
\mbox{maximize}_{v} \quad &  
H(\alpha^*, v) = 
\Big[ n^{-1} \sum_{g\in \gG}(\eta_g c_g)^{1/(p+1)} \Big]^p
\Big[ \sum_{g \in \gG} (\eta_g c_g)^{1/(p+1)} \Big] + 
\sum_{g \in \gG} \eta_g  \big[ \tau_g * n^{-q_g} + \delta_g \big]
\\
\mbox{subject to} \quad & \sum_{g \in \gG} v_g = 1; \quad v_g > 0 \; \forall g \in \gG
\end{align*}
where $\eta_g = \omega_1 \gamma_g + \omega_2 v_g$. Solve this constrained optimization problem by writing down its KKT conditions (see, e.g., Chapter 5.5 of \citet{boyd2004convex}) with respect to the Lagrangian form $-H(\alpha^*, v) + \lambda (\sum_g v_g - 1) - u_g \sum_g v_g $, i.e., for every $g$:
\begin{align*}
    \frac{\partial}{\partial v_g} \big[ -H(\alpha^*, v) + \lambda (\sum_g v_g - 1) - u_g \sum_g v_g \big] = 0; 
    \qquad 
    \sum_{g} v_g = 1; \qquad u_g * v_g = 0;
    \qquad 
    u_g \geq 0, \; v_g &\geq 0.
\end{align*}
Simplifying the first derivative equation in the above, we arrive at the full set of KKT condition:
\begin{alignat*}{2}
&-\frac{\partial}{\partial v_g} H(\alpha^*, v) + \lambda - u_g = 0; 
\quad && \mbox{(Stationarity Condition)}
\\ 
&\sum_{g} v_g = 1; \quad v_g \geq 0; && \mbox{(Primal feasibility)}\\
&u_g \geq 0; && \mbox{(Dual Feasibility)}\\
& u_g * v_g = 0.  && \mbox{(Complementary Slackness)}
\end{alignat*}
Rearranging the terms, we get for every $g$:
\begin{align}
u_g &=-\frac{\partial}{\partial v_g} H(\alpha^*, v) + \lambda;
\label{eq:kkt_stat_cond}
\\
& u_g * v_g = 0; \quad u_g \geq 0; \quad  v_g \geq 0.
\label{eq:kkt_comp_slack}
\\ 
&\sum_{g} v_g = 1;
\label{eq:kkt_simplex_cond}
\end{align}
and our goal is to identify $v^*=\{v^*_g\}_{g\in \gG}$ which satisfy all the above conditions.

First notice (\ref{eq:kkt_stat_cond}) implies that $u_g \geq 0$ if and only if:
\begin{alignat*}{2}
0 
&\geq \frac{\partial}{\partial v_g} H(\alpha^*, v) - \lambda 
\stackrel{By (\ref{eq:H_deriv})}{=}
\Big[ \omega_2^{1/p} n^{-1} \sum_{g\in \gG} (\eta_g c_g)^{1/(p+1)} \Big]^p 
* 
c_g^{1/(p+1)} \eta_g^{-p/(p+1)} + 
[ \omega_2 \, (\tau_g n^{-q_g} + \delta_g)-\lambda ]
\end{alignat*}
Denoting $l_{g,\omega}=(\lambda - \omega_2(\tau_g n^{-q_g} + \delta_g)))^{-1}$ and $Z_\omega =\Big[ \omega_2^{1/p} n^{-1} \sum_{g\in \gG} (\eta_g c_g)^{1/(p+1)} \Big]^{p+1} $, then the above is equivalent to stating:
\begin{align*}
\omega_1 \gamma_g + \omega_2 v_g
&= 
\eta_g \geq
Z_\omega \,
c_g^{1/p} l_{g,\omega}^{(p+1)/p}
\quad \mbox{or equivalently,}
\quad
v_g \geq \frac{\omega_1}{\omega_2}
\Big[ 
\frac{1}{\omega_1} 
Z_\omega \,
c_g^{1/p} l_{g,\omega}^{(p+1)/p}
- \gamma_g
\Big],
\end{align*}
if and only if $u_g \geq 0$ (due to (\ref{eq:kkt_stat_cond})). More specifically, this means:
\begin{align}
\mbox{if} \quad u_g > 0, \qquad &
v_g > \frac{\omega_1}{\omega_2}
\big[ 
\frac{1}{\omega_1} 
Z_\omega \,
c_g^{1/p} l_{g,\omega}^{(p+1)/p}
- \gamma_g
\big],
\; \mbox{or equivalently,} \;\; 
\gamma_g > 
\frac{1}{\omega_1} Z_\omega \,
c_g^{1/p} l_{g,\omega}^{(p+1)/p} - 
\frac{\omega_2}{\omega_1} v_g;
\label{eq:kkt_iff_u_pos}
\\
\mbox{if} \quad u_g = 0, \qquad &
v_g = \frac{\omega_1}{\omega_2}
\Big[ 
\frac{1}{\omega_1} 
Z_\omega \,
c_g^{1/p} l_{g,\omega}^{(p+1)/p}
- \gamma_g
\Big].
\label{eq:kkt_iff_u_zero}
\end{align}

Now use (\ref{eq:kkt_iff_u_pos})-(\ref{eq:kkt_iff_u_zero}) to analyze the second condition (\ref{eq:kkt_comp_slack}) (i.e., complementary slackness). Specifically, (\ref{eq:kkt_comp_slack}) states that $v_g = 0$ if $u_g > 0$, and $v_g \geq 0$ if $u_g = 0$. Under (\ref{eq:kkt_iff_u_pos})-(\ref{eq:kkt_iff_u_zero}), this implies
\begin{align*}
v_g = 
\begin{cases}
0 
&  \mbox{if} \quad u_g>0, 
\; \mbox{or equivalently,} \;
\Big[ 
\frac{1}{\omega_1} 
Z_\omega \,
c_g^{1/p} l_{g,\omega}^{(p+1)/p}
- \gamma_g
\Big] < 0
;
\\
\frac{\omega_1}{\omega_2}
\Big[ 
\frac{1}{\omega_1} 
Z_\omega \,
c_g^{1/p} l_{g,\omega}^{(p+1)/p}
- \gamma_g
\Big]
&  \mbox{if} \quad u_g=0.
\end{cases}
\end{align*}
The above can be expressed succinctly as:
\begin{align}
v_g = \max\Big(
0, \;
\frac{\omega_1}{\omega_2}
\big[ 
\frac{1}{\omega_1} 
Z_\omega \, c_g^{1/p} l_{g,\omega}^{(p+1)/p}
- \gamma_g \big]
\Big).
\label{eq:v_g_interm_expr}
\end{align}
As a result, $\eta_g=\omega_1 \gamma_g + \omega_2 v_g$ can be expressed as:
\begin{align}
\eta_g = \max\Big(
\omega_1 \gamma_g, \;
Z_\omega \, c_g^{1/p} l_{g,\omega}^{(p+1)/p}
\Big).
\label{eq:eta_g_interm_expr}
\end{align}

To obtain a more succinct expression of $\eta_g$, now derive an expression of $Z_\omega$ using the the third and final condition (\ref{eq:kkt_simplex_cond}). Notice that in (\ref{eq:v_g_interm_expr}),
$v_g  > 0$ if and only if $\gamma_g <
\frac{1}{\omega_1} Z_\omega \,
c_g^{1/p} l_{g,\omega}^{(p+1)/p}$ (due to (\ref{eq:kkt_iff_u_pos})), which implies that $v_g > 0$ if and only if the empirical prevalence $\gamma_g$ of group $g$ is low. To this end, let $\gB =\Big\{ g \Big| \gamma_g \leq
\frac{1}{\omega_1} Z_\omega \,
c_g^{1/p} l_{g,\omega}^{(p+1)/p} \Big\} \subseteq \gG$ be the indices  of the low-prevalence, under-represented groups, so that $v_g>0$ if and only if $g \in \gB$. Then, (\ref{eq:kkt_simplex_cond}) implies:
\begin{align}
1 = \sum_{g\in \gG} v_g &= \sum_{g \in \gB} v_g
= 
\sum_{g \in \gB}
\frac{\omega_1}{\omega_2}
\big[ 
\frac{1}{\omega_1} 
Z_\omega \, c_g^{1/p} l_{g,\omega}^{(p+1)/p}
- \gamma_g \big], 
\;\; \mbox{or equivalently,} \;\;
Z_{\omega} = 
\frac{\omega_2 + \omega_1 * \sum_{g \in \gB} \gamma_g}
{\sum_{g \in \gB} c_g^{1/p} l_{g,\omega}^{(p+1)/p}}.
\label{eq:Z_omega_expr}
\end{align}

We are now ready to derive the final expressions of $\eta^*_g$ and $\alpha^*$. Specifically, plugging (\ref{eq:Z_omega_expr}) into (\ref{eq:eta_g_interm_expr}), we get:
\begin{align*}
\eta^*_g = \omega_1 * \max\Big[
\gamma_g, \;
\big(
\frac{\omega_2 + \omega_1 * \sum_{g \in \gB} \gamma_g}{\omega_1} 
\big)\big(
\frac{c_g^{1/p} l_{g,\omega}^{(p+1)/p}}{\sum_{g \in \gB} c_g^{1/p} l_{g,\omega}^{(p+1)/p}}
\big)
\Big].
%\label{eq:eta_g_final_expr}
\end{align*}
Then, (\ref{eq:prop_inner_problem_sol}) implies that the optimal allocation $\alpha^*$ is
\begin{align*}
\alpha^*_g = 
\frac{(r_g c_g)^{1/(p+1)} } {\sum_{g\in \gG}(r_g c_g)^{1/(p+1)}},
\quad \mbox{where} \quad
r_g = \frac{\eta^*_g}{\omega_1}=
\max\Big[
\gamma_g, \;
\big(
\frac{\omega_2 + \omega_1 * \sum_{g \in \gB} \gamma_g}{\omega_1} 
\big)\big(
\frac{c_g^{1/p} l_{g,\omega}^{(p+1)/p}}{\sum_{g \in \gB} c_g^{1/p} l_{g,\omega}^{(p+1)/p}}
\big)
\Big].
\end{align*}

Furthermore, the definition of the under-represented groups $\gB \subseteq \gG$ can be expressed as:
\begin{align*}
\gB =
\bigg\{ g
\Big|
\gamma_g \leq 
\big(
\frac{\omega_2 + \omega_1 * \sum_{g \in \gB} \gamma_g}{\omega_1} 
\big)\big(
\frac{c_g^{1/p} l_{g,\omega}^{(p+1)/p}}{\sum_{g \in \gB} c_g^{1/p} l_{g,\omega}^{(p+1)/p}}
\big)
\bigg\}.
\end{align*}
Finally, notice that (\ref{eq:kkt_simplex_cond}) also implies the $\lambda$ in $l_{g,\omega}=(\lambda - \omega_2(\tau_g n^{-q_g} + \delta_g)))^{-1}$ is the solution to 
% (recall $Z_\omega =\Big[ \omega_2^{1/p} n^{-1} \sum_{g\in \gG} (\eta_g c_g)^{1/(p+1)} \Big]^{p+1}$)
:
\begin{align*}
1 
= \sum_{g \in \gG} v_g 
&= 
\sum_{g \in \gG} 
\max\Big(
0, \;
\frac{1}{\omega_2}
Z_\omega \, c_g^{1/p} l_{g,\omega}^{(p+1)/p}
- 
\frac{\omega_1}{\omega_2}
\gamma_g
\Big)
% \\
% &= 
% \sum_{g \in \gG} 
% \max\Big(
% 0, \;
% \omega_2^{1/p}
% \big[ n^{-1} \sum_{g\in \gG} (\eta_g c_g)^{1/(p+1)} \big]^{p+1}
%  \, c_g^{1/p} l_{g,\omega}^{(p+1)/p}
% - 
% \frac{\omega_1}{\omega_2}
% \gamma_g
% \Big)
,
\end{align*}
so that $\exists g$ such that $v_g>0$ and that $\gB$ is non-empty.

% Notice that the similarity between structure of this solution and that of the \textit{water-filling problem} (see, e.g., Example 5.2 of \citet{boyd2004convex}). 
\end{proof}


==> introspective ensemble/sections/abstract_old_versions.tex <==
\jereliu{original version}
Uncertainty-based active learning (AL) is a promising approach to mitigate dataset bias and improve model fairness. By diversely sampling from the under-represented tail groups, AL is expected to improve the distributional balance in the training data and the so-called \textit{accuracy-fairness frontier} in the trained model. \dvij{I think active learning is broader and goal is data efficient learning more generally. Perhaps we want to discuss fairness aware active learning more specifically?}
However, the quality of uncertainty estimates from modern deep-learning model are typically worse in the presence of spurious correlations and dataset bias,  
so the improvements from AL on tail groups may be limited even though AL can improve overall accuracy. 
In this work, we propose \textit{\gls{ISP}}, a simple approach to improve the uncertainty estimation of a deep neural network under dataset bias. 
ISP adds an auxiliary \textit{introspection} task to model training, asking the model to predict whether an example belongs to an under-represented group.
We show that ISP provably improves the bias-awareness of the model representations and the resulting uncertainty estimates, and can be readily adapted to the setting where group annotation is not available via a cross-validation procedure.
On challenging tabular and language tasks with dataset bias and label noise, ISP consistently improves both the tail-group sampling rate and hence the accuracy-fairness tradeoff frontier of the final model, strongly outperforming the popular alternatives.

\dvij{Alternative abstract}:
Deep learning has been shown to suffer from spurious correlations and systematic bias, particularly when datasets deep networks are trained on are themselves biased. Further, this bias may not be easy to measure when details of the data generation process are not available. In this work, we develop a new technique, \gls{ISP} that learns to estimate per-datapoint bias and uses the learned bias predictions to preferentially sample datapoints in an active learning setting to mitigate the impact of this bias. Unlike prior work, our technique does not require subgroup information. We analyze our approach theoretically and demonstrate that, under standard assumptions used in the fairness literature, our technique correctly estimates dataset bias \dvij{Jeremiah please check or refine this.}. Further, we demonstrate empirically that on datasets with systematic bias, our technique correctly identifies under-represented groups on which the model performance is low and up-samples these in an active learning setting. \dvij{Provide some concrete numbers on empirical improvements}

\balaji{Alternative abstract}:
Uncertainty-based active learning (AL) is a promising approach to mitigate dataset bias and improve model fairness. By diversely sampling from the under-represented tail groups, AL is expected to improve the distributional balance in the training data and improve the so-called \textit{accuracy-fairness frontier} in the trained model. 
A key ingredient for such AL approaches is an accurate estimate of the model bias and uncertainty. However, the quality of uncertainty estimates from modern deep-learning model are typically worse in the presence of spurious correlations, and furthermore, the bias may not be easy to measure when details of the data generation process are not available. Hence, existing approaches do not significantly improve the performance on tail groups, leading to sub-optimal solutions in the accuracy-fairness frontier.   %even though they may improve overall accuracy. 
In this work, we propose \textit{\gls{ISP}}, a simple approach to improve the uncertainty estimation of a deep neural network under dataset bias. ISP adds an auxiliary \textit{introspection} task to model training, asking the model to predict whether an example belongs to an under-represented group.
We show that ISP provably improves the bias-awareness of the model representations and the resulting uncertainty estimates, and can be readily adapted to the setting where group annotation is not available via a cross-validation procedure.
On challenging tabular and language tasks with dataset bias and label noise, we demonstrate that ISP correctly identifies tail groups on which the model performance is low and up-samples these in an active learning setting, thus achieving sate-of-the-art on the accuracy-fairness frontier.


==> introspective ensemble/sections/app_optimal_allocation.tex <==
\section{Optimal Group-size Allocation: Full Theoretical Results}
{\color{red} Note: Hide from main submission}

Denote $D_{\alpha,n}$ as a dataset with sample size $n$ and group allocation $\alpha=\{\alpha_g\}_{g\in \gG}$, $f_{D_{\alpha,n}}$ is a model trained on $D_{\alpha,n}$, and $R(f|G=g)=E_{D_g}(L(y, f))$ is the group-specific risk for a model $f$. 

\subsection{Key Technical Lemmas}
\label{sec:lemma}

\input{proof/lemma_1}
{\proof See \Cref{sec:allocation_weighted_risk_proof}.}\\

\input{proof/lemma_2}
{\proof See \Cref{sec:allocation_worst_risk_proof}.}\\


\subsection{Key Technical Propositions}
\input{proof/prop_app_1}

{\proof See \Cref{sec:optimal_allocation_frontier_full_proof}.}\\

\subsection{Corollaries}

\begin{corollary_prop}[Sufficient Conditions of the Underrepresented Group $\gB$]
Under the assumption of \ref{thm:optimal_allocation_frontier_full} (i.e., the group-specific scaling laws share the same $p_g=p \;\forall g$). Recall that the definition of underrepresented group $\gB$ is:
\begin{align*}
\gB \coloneqq 
\Bigg\{ g \Big|
\gamma_g < ( \frac{\omega_2}{\omega_1} + \sum_{g \in \gB} \gamma_g) * 
\frac{c_g^{1/p} l_{g,\omega}^{(p+1)/p}}{\sum_{g \in \gB} c_g^{1/p} l_{g,\omega}^{(p+1)/p}}
\Bigg\}.
\end{align*}
Then a group $g \in \gG$ belongs to the underrepresented group $\gB$ if its population prevalence satisfies:
\begin{align}
\gamma_g < \frac{\omega_2}{\omega_1}  * 
\frac{c_g^{1/p} l_{g,\omega}^{(p+1)/p}}{\sum_{g \in \gG} c_g^{1/p} l_{g,\omega}^{(p+1)/p}}.
\label{eq:minority_criteria_full}
\end{align}

\label{thm:minority_group_criteria_full}
\end{corollary_prop}

\begin{proof}
Notice that the right-hand side of (\ref{eq:minority_criteria_full}) is an lower bound of the condition in $\gB$. Specifically,
\begin{alignat*}{2}
&
( \frac{\omega_2}{\omega_1} + \sum_{g \in \gB} \gamma_g) * 
\frac{c_g^{1/p} l_{g,\omega}^{(p+1)/p}}{\sum_{g \in \gB} c_g^{1/p} l_{g,\omega}^{(p+1)/p}} \\
\geq \; & 
( \frac{\omega_2}{\omega_1}) * 
\frac{c_g^{1/p} l_{g,\omega}^{(p+1)/p}}{\sum_{g \in \gB} c_g^{1/p} l_{g,\omega}^{(p+1)/p}} 
&& \mbox{(Since $\sum_{g \in \gB} \gamma_g \geq 0$)} \\
\geq \; & 
( \frac{\omega_2}{\omega_1}) * 
\frac{c_g^{1/p} l_{g,\omega}^{(p+1)/p}}{\sum_{g \in \gG} c_g^{1/p} l_{g,\omega}^{(p+1)/p}} 
&& \mbox{(Since $\gB \subseteq \gG$ and $c_g, l_{g,\omega}$ are non-negative)}.
\end{alignat*}
Therefore, if (\ref{eq:minority_criteria_full}) holds, we have:
\begin{align*}
\gamma_g 
<  
( \frac{\omega_2}{\omega_1}) * 
\frac{c_g^{1/p} l_{g,\omega}^{(p+1)/p}}{\sum_{g \in \gG} c_g^{1/p} l_{g,\omega}^{(p+1)/p}} 
\leq 
( \frac{\omega_2}{\omega_1} + \sum_{g \in \gB} \gamma_g) * 
\frac{c_g^{1/p} l_{g,\omega}^{(p+1)/p}}{\sum_{g \in \gB} c_g^{1/p} l_{g,\omega}^{(p+1)/p}},
\end{align*}
which implies $\gamma_g \in \gB$.
\end{proof}

\begin{corollary_prop}[Generalization Error-based Sampling Selects Underrepresented Group]
Assuming the group-specific scaling laws share the same $p_g=p, q_g=q, \tau_g=\tau, \delta_g=\delta \;\forall g$. Then the definition of underrepresented group $\gB$ is:
\begin{align*}
\gB \coloneqq 
\Bigg\{ g \Big|
\gamma_g < ( \frac{\omega_2}{\omega_1} + \sum_{g \in \gB} \gamma_g) * 
\frac{c_g^{1/p}}{\sum_{g \in \gB} c_g^{1/p}}
\Bigg\}.
\end{align*}
Notice that the criteria for underrepresented groups remains the same even when $n \rightarrow \infty$.

Recall that under the empirical distribution $\gD$, by Assumption \ref{def:group_scaling_law}, the generalization error for a group $g$ is $e_g \coloneqq c_g n_g^{-p} + \tau n^{-q} + \delta$. Then, under a
generalization-error based active sampling policy $I(e_g > t_n)$ with threshold $t_n$, i.e., an example is selected if its generalization exceeds $t_n$. There exists a optimal threshold $t_n$ such that a group will be selected if and only if it belongs to $\gB$.
\label{thm:optimality_cv_active_sampling}
\end{corollary_prop}

\begin{proof}
Under the empirical distribution, the size of each group can be expressed as $n_g = \gamma_g n$. Then, the threshold-based sampling policy implies:
\begin{alignat*}{2}
t_n &< c_g (\gamma_g n)^{-p} + \tau n^{-q} + \delta,
&& \mbox{which implies}
\\
(\gamma_g n)^{p}  &< c_g (t_n - \tau n^{-q} - \delta)^{-1}, 
&& \mbox{which implies}
\\
\gamma_g  &< n^{-1} c_g^{1/p} (t_n - \tau n^{-q} - \delta)^{-1/p}.
\end{alignat*}
Then, equating the last expression with the criteria for the underrepresented group $\gB$, we have:
\begin{align*}
n^{-1} c_g^{1/p} (t_n - \tau n^{-q} - \delta)^{-1/p} &=  ( \frac{\omega_2}{\omega_1} + \sum_{g \in \gB} \gamma_g) * 
\frac{c_g^{1/p}}{\sum_{g \in \gB} c_g^{1/p}}
&& \mbox{which implies}
\\
t_n &=  
C n^{-p} + \tau n^{-q} + \delta,
\end{align*}
where $C=\big[ ( \frac{\omega_2}{\omega_1} + \sum_{g \in \gB} \gamma_g) / 
(\sum_{g \in \gB} c_g^{1/p}) \big]^{-p}$ is a constant that does not depend on $n$. 
Consequently, there exists a threshold $t_n=C * n^{-p} + \tau n^{-q} + \delta$ such that it selects a group $g$ if and only if it belongs to the underrepresented group $\gB$.
\end{proof}


%\newpage
\section{Proof of Propositions}
\subsection{Proof of \Cref{thm:optimal_allocation_frontier_full}}
\label{sec:optimal_allocation_frontier_full_proof}
\input{proof/prop_app_1_proof}


%\newpage
\section{Proof of Lemmas}
\label{eq:lemma_proof}

\subsection{Proof of \Cref{thm:allocation_weighted_risk}}
\label{sec:allocation_weighted_risk_proof}
\input{proof/lemma_1_proof}


\subsection{Proof of \Cref{thm:allocation_worst_risk}}
\label{sec:allocation_worst_risk_proof}
\input{proof/lemma_2_proof}

%\newpage

\begin{assumption}[Group-specific generalization error  \citep{rolf2021representation}]
The group-specific generalization error $R(f_{D}|G=g)=E_{D_g}(L(y, f_D))$ can be approximated by a scaling function of the group sample size $n_g$ and the total sample size $n$. That is, $\exists \, M_g >0$ and  constants $c_g, \tau_g, \delta_g \geq 0$, $p_g, q_g > 0$ such that for a dataset $D_{\alpha, n}$ with sample size $n$ and group allocation $\alpha=\{\alpha_g\}_{g\in \gG}$, and $f_{D_{\alpha, n}}$ the model trained $D$ with a particular algorithm, the generalization error $R(f_{D_{\alpha, n}}|G=g)$ can be approximated as:
\begin{align}
%\nonumber
R(f_{D_{\alpha, n}}|G=g) &\approx 
r(n_g, n | c_g, \tau_g, \delta_g, p_g, q_g) 
= c_g * n_g^{-p_g} + \tau_g * n^{-q_g} + \delta_g.
\label{eq:group_scaling_law}
\end{align}
The above is assumed to hold for any $\alpha \in \Delta^{|\gG|}$ and any $n$ such that $n_g = \lfloor \alpha_g n \rfloor \geq M_g$.
\vspace{-0.5em}
\label{def:group_scaling_law}
\end{assumption}
Assumption \ref{def:group_scaling_law} essentially states that each group has an unique learning rate $o(c_g n^{-p_g} + \tau_g n^{-q_g})$, which includes a $\tau_g n^{-q_g}$ term to allow the overall data size to influence the risk of group $g$. The scaling coefficients $(c_g, \tau_g, p_g, q_g)$ describes the difficulty of the learning problem.
%, where higher values of $(c_g, \tau_g)$ and lower values of $(p_g, q_g)$ indicate that the group $g$ is more difficult to learn (i.e., the generalization error decreases slower with respect to sample size). Note that for common choices of loss function, we expect $p_g, q_g$ to be bounded in a small range (e.g.,  $p_g, q_g  < 1$ for squared loss, since the optimal parametric learning rate is $n^{-1}$ \citep{bach2017breaking}). It should be acknowledged that the Assumption \ref{def:group_scaling_law} is simplistic, as it assumes that the scaling coefficients $(c_g, \tau_g, p_g, q_g)$ are not impacted by the group composition of the training data $\alpha$. However, 
\citet{rolf2021representation} shows that (\ref{eq:group_scaling_law}) holds exactly in classic settings such as linear regression, and verified that it approximated holds empirically in, e.g., image classification tasks using ResNet models.


==> introspective ensemble/sections/background_backup.tex <==
Given a dataset $D \sim \gD$ and a loss function $L$ , we consider learning the prediction function 
\[f_D = \argmin_{f \in \gF} L(f, y|D), \text{ where } L(y, f|D)=\sum_{\{\rvx_i, y_i\}\in D} L(y_i, f(\rvx_i)).\] Following the previous work \citep{pfau2013generalized}, we denote the \textit{ensemble predictor}:
\[\bar{f} = \argmin_{f\in \gF} E_{D\sim\gD}(L(f_D, f))\]
over ensemble members $f_D$'s, where each $f_D$ is trained on a random draw of training dataset $D \sim \gD$. 
% We also denote $f^*=\argmin_{f \in \gF} E_{D^*}L(f, y|D^*)$ the \textit{oracle predictor} that is learned from the infinitely-large and perfectly-balanced oracle training set $D^*$. Note that $f^*$ is deterministic due to the infinitely large size of $D^*$.
For test example $\{y_i, \rvx_i\}$, we can decompose the predictive error of a trained model $f_D(\rvx)$ using a generalized bias-variance decomposition for Bregman divergence:
\begin{proposition}[Noise-Bias-Variance Decomposition under Bregman divergence \citep{domingos2000unified, pfau2013generalized}] 
Given a loss function of the Bregman divergence family, for a test example $\{y, \rvx\}$ the expected prediction loss $L(y, f_D(\rvx))$ of an empirical predictor $f_D$ can be decomposed as:
\begin{align}
E_D \big[ L(y, f_D(\rvx)) \big]
&= 
\underbrace{E_{D} \big[ L(y, \tilde{y}(\rvx)) \big]}_\text{{\color{OliveGreen} Noise}}
+ \quad
\underbrace{L(\tilde{y}(\rvx), \bar{f}(\rvx))}_\text{{\color{Maroon} Bias}}
\quad + \quad
\underbrace{E_{D} \big[ L(\bar{f}(\rvx), f_D(\rvx)) \big]}_\text{{\color{RoyalBlue} Uncertainty}}
\label{eq:error_decomposition}
\end{align}
\vspace{-1.5em}
\label{thm:error_decomposition_app}
\end{proposition}
%Proof is in \Cref{sec:error_decomposition_proof}. \Cref{thm:error_decomposition} is a generalization of the classic noise-bias-variance decomposition result \citep{domingos2000unified} to account for the model mis-specification error in $\gF$. This is achieved by defining $f^*=\argmin_{f \in \gF} E_{D^*}L(f, y|D^*)$ as the best-achievable function within the model class $\gF$, rather than the Bayes optimal predictor $f^{opt}(\rvx_i) = \argmin_{y'} E_{y\sim P(y|\rvx_i, g_i)}L(y, y')$. 
We now interpret each of the terms defined above: \\
\emph{\bf Noise:} Given a fixed data distribution $\gD$, the first term {\color{OliveGreen} $E_{D} \big[ L(y, f^*(\rvx)) \big]$} quantifies the {\color{OliveGreen} \textit{irreducible noise}} that is due to the stochasticity in the noisy observation $y$. \\%or the mis-specification in the model class $\gF$. 
\emph{\bf Uncertainty:} The third term {\color{RoyalBlue} $E_{D} \big[ L(\bar{f}(\rvx), f_D(\rvx)) \big]$} quantifies the {\color{RoyalBlue} \textit{model uncertainty}} in the prediction, which can be due to variations in the finite-size data $D$, the stochasticity in the randomized learning algorithm $\gF \times D \rightarrow f_D$, or the randomness in the initialization of an  overparameterized model \citep{adlam2020understanding}. \\
\emph{\bf Bias:} Finally, the middle term {\color{Maroon} $L(\tilde{y}(\rvx), \bar{f}(\rvx))$} quantifies the gap between  $\tilde{y}(\rvx)$ (i.e., the ``true label") and the ensemble predictor $\bar{f}$ learned from the empirical data $D \sim \gD$. For the examples $\rvx$ coming from the under-represented groups with $\gamma_g \ll \frac{1}{|\gG|}$, the bias term can be further decomposed into:
\begin{align}
L(\tilde{y}(\rvx), \bar{f}(\rvx))
&= 
\underbrace{L(\tilde{y}(\rvx), \bar{f}^*(\rvx))}_\text{{\color{Maroon} \textit{Bias, Model}}}
+
\underbrace{\gE(\bar{f}^*(\rvx), \bar{f}(\rvx))}_\text{{\color{Maroon} \textit{Excess Bias, Data}}},
\label{eq:bias_decomposition}
\end{align}
where $\bar{f}^\ast = \argmin_{f\in \gF} E_{D^\ast \sim \gD^\ast}(L(f_{D^\ast}, f))$ is the optimal ensemble predictor based on size-$n$ datasets $D^\ast$ sampled from the optimal distribution $\gD^\ast$ where all groups have equal representation. Here, $L(\tilde{y}(\rvx), \bar{f}^*(\rvx))$ is the bias inherent to the model class and cannot be eliminated by ensembling. It can be caused by model misspecification, missing features, or regularization. On the other hand, $\gE(\bar{f}^*(\rvx), \bar{f}(\rvx)) = L(\tilde{y}(\rvx), \bar{f}(\rvx)) - L(\tilde{y}(\rvx), \bar{f}^*(\rvx))$ indicates the ``excess bias" for the under-represented groups caused by the imbalance in the group distribution $P(G)$ in the data-generation distribution $\gD$. 

To make the idea concrete, consider a simple example where we fit a ridge regression model $f(\rvx_i)=\beta^\top \rvx_i$ to the Gaussian observation data $y_i=\theta^{\top} \rvx_i + \epsilon, \epsilon \sim N(0, \sigma^2)$ under an imbalanced experiment design, where we have $|\gG|$ treatment groups and $n_g$ observations in each group. Here, $\rvx_i = [1_{g_i = 1}, ..., 1_{g_i = |\gG|}]$ is a $|\gG| \times 1$ one-hot indicator of the membership of $g_i$ for each group in $\gG$, and $\theta=[\theta_1, \dots, \theta_{|\gG|}]$ is the true effect for each group. Then, under ridge regression, the noise-bias-variance decomposition for group $g$ is $E_D(L(y, f_D))={\color{OliveGreen} \sigma^2} + {\color{Maroon} \frac{(\lambda\theta_g)^{ 2}}{(n_g + \lambda)^2}} + {\color{RoyalBlue} \frac{\sigma^2 n_g}{(n_g + \lambda)^2}}$, where the regularization parameter $\lambda$  modulates a trade-off between the {\color{Maroon} \textit{bias}} and {\color{RoyalBlue} \textit{uncertainty}} terms 
(\Cref{sec:error_decomposition_ridge}). Consequently, for an underrepresented group with small size $\gamma_g \ll \frac{1}{|\gG|}$, its predictive bias ${\color{Maroon} \frac{(\lambda\theta_g)^{\ast 2}}{(n_g + \lambda)^2}}$ is exacerbated due to lacking sufficient statistical information to counter the regularization bias, incuring an excessive bias of $\gE(\bar{f}^*(\rvx), \bar{f}(\rvx))\approx \frac{\lambda \theta_g}{n \gamma^\ast_g \gamma_g}(\gamma^\ast_g - \gamma_g)$ when compared to an optimal ensemble predictor $\bar{f}^*$ trained from a perfectly balanced size-$n$ datasets with $\gamma^\ast_g=1/|\gG|$.

Finally, note that in \Cref{eq:error_decomposition}, the first two terms combined constitute the traditional bias term $E_D[L(y, \bar{f})]=E_{D} \big[ L(y, f^*(\rvx)) \big] + L(f^*(\rvx), \bar{f}(\rvx))$ in the classic bias-variance decomposition. To this end, the conceptual significance of Equations (\ref{eq:error_decomposition})-(\ref{eq:bias_decomposition}) is to isolate data imbalance as a distinct source of systematic error (i.e., that is different from those due to label noise or model misspecification), motivating us to explore the practical approximation of $\gE(\bar{f}^*(\rvx), \bar{f}(\rvx))$ for improving model performance under dataset bias (\Cref{sec:bias_estimation}).

As an aside, when the predictive model $f_D$ is probabilistic (e.g., the model generates a posterior predictive distribution $P(f|D)$ rather than a point estimate $f$), the {\color{RoyalBlue} \textit{model uncertainty}} in \Cref{eq:error_decomposition} is further decomposed as:
\begin{align}
E_D \big[ L(\bar{f}(\rvx), f_D(\rvx)) \big]= 
\underbrace{ E_D \big[ L(\bar{f}(\rvx), \mu_D(\rvx))  \big]}_\text{
{\color{RoyalBlue}\textit{Ensemble Diversity}}} + 
\underbrace{E_D E_{f \sim P(f|D)} \big[ L(\mu_D(\rvx), f(\rvx)) \big] }_\text{
{\color{RoyalBlue}\textit{Posterior Variance}}}
\end{align}
where $\mu_D(\rvx)=E_{f\sim P(f|D)}[f(\rvx)]$ is the posterior mean. As shown, comparing to an ensemble of deterministic models, the ensemble of probabilistic models provides additional flexibility in quantifying model uncertainty via the extra term of expected posterior variance.


==> introspective ensemble/sections/intro_backup.tex <==
\input{figures/acc_fair_intro}

The modern \glsfirst{DNN} models are commonly trained on the large-scale, in-the-wild datasets \citep{deng2009imagenet}.
These data often exhibits an imbalanced long-tail distribution with many small population subgroups, reflecting the nature of the physical and social processes underlying the data distribution 
\citep{zhu2014capturing, feldman2020neural%yang2020rethinking,
}. 
This imbalance in training data distribution, i.e., \textbf{\textit{dataset bias}}, has prevented the \gls{DNN} models from generalizing equitably to the under-represented population groups
\citep{hasnain2007disparities%, ekstrand2018all, hofmanninger2020automatic
}. {\color{red} mention spurious correlation}

\textbf{Accuracy-Fairness Frontier:} In response, the existing bias mitigation literature has focused on improving the training procedure under a fixed and imbalanced training dataset, striving to produce a balanced performance between model accuracy and fairness (e.g., the average-case v.s. worst-group performance)
\citep{agarwal2018reductions, martinez2020minimax, martinez2021blind}%, sagawa2020investigation, liu2021just}
. Formally, this goal corresponds to identifying a optimal model $f \in \gF$ that attains the \textit{Pareto efficiency frontier} of the accuracy-fairness trade-off (e.g., see \Cref{fig:acc_fair_frontier_intro}), so that under the same training data $D=\{y_i, \rvx_i\}_{i=1}^n$, we cannot find another model $f' \in \gF$ that outperforms $f$ in both accuracy and  fairness. In the literature, this \textit{accuracy-fairness frontier} is often characterized by a trade-off objective \citep{martinez2021blind}:
\begin{align}
    f_\lambda = \argmin_{f\in \gF} F_{\lambda}(f|D); 
    \qquad
    F_{\lambda}(f|D) \coloneqq R_{acc}(f|D) + \lambda R_{fair}(f|D),
    \label{eq:frontier_risk_intro}
\end{align}
\vspace{-1.5em}

where $R_{acc}$ and $R_{fair}$ are risk functions for a model's accuracy and fairness, and $\lambda > 0$ a trade-off parameter.
Then, $f_\lambda$ cannot be outperformed by any another $f'$ at the trade-off level $\lambda$.
The entire frontier under a dataset $D$ can then be characterized by finding $f_\lambda$ that minimizes the fairness-accuracy objective (\ref{eq:frontier_risk_intro}) at every trade-off level $\lambda$, and tracing out their $(R_{acc},  R_{fair})$ performances
%on a 2D plane 
(\Cref{fig:acc_fair_frontier_intro}).

\textbf{Goal:} However, bias-robust learning under a fixed and imbalanced dataset comes with inherent challenges.
The limited size of the tail-group examples restricts the \gls{DNN} model's worst-group performance, leading to a compromised accuracy-fairness frontier 
% (i.e., a high value in the $min_{f \in \gF} F_\lambda(f|D)$)
\citep{zhao2019inherent, dutta2020there%vzliobaite2015relation, menon2018cost
}. 
Recognizing this inherent limitation brought by the dataset distribution, we ask: 

\textit{Under a fixed learning algorithm, can we meaningfully push the model's accuracy-fairness frontier by improving the training data distribution using active learning?} 

That is, denoting $D_{\alpha, n}=\{(y_i, \rvx_i)\}_{i=1}^n$ a training dataset with $K$ subgroups and the group size distribution $\alpha = [\alpha_1, \dots, \alpha_K]$, we study that if a model's accuracy-fairness performance $F_\lambda$ can be improved by improving the group distribution of the training data $\alpha$, i.e., we seek to optimize an outer problem:
\begin{align}
% F_\lambda^* = 
{\color{Maroon} \minimize_{\alpha \in \Delta^{|\gG|}}}
\Big[ \min_{f \in \gF} F_{\lambda}(f|D_{{\color{Maroon}\alpha},n}) \Big],
\label{eq:al_objective_intro}
\end{align}
where $\Delta^K$ is the simplex of all possible group distributions \citep{rolf2021representation}. In practice, the uncertainty-based \gls{AL} holds promise to achieve this exact objective: given a sampling model with \textit{well-calibrated} uncertainty (i.e., the model uncertainty is well-correlated with generalization error), \gls{AL} can pro-actively identify the unlabelled examples from the under-represented subgroups, and add them to the training data to reach a more balanced data distribution \citep{branchaud2021can}. 
% This this undoubtly appealing
% This helps the model to improve its worst-group performance without significantly sacrificing accuracy, thereby breaking the accuracy-fairness frontier otherwise ``locked" by an imbalanced data distribution \citep{idrissi2022simple} (\Cref{fig:acc_fair_frontier_intro}).

\textbf{Challenges with DNN Uncertainty under Bias:} However, the recent work suggest that the \gls{DNN} model's uncertainty estimate is less trust-worthy under spurious correlations and distributional shift, potentially compromising the \gls{AL} performance under dataset bias.
For example, \citet{ovadia2019can} shows that the \gls{DNN}'s expected calibration error rises as the testing data distribution deviates from the training data distribution, and \citet{ming2022impact} shows that \gls{DNN}'s ability in detecting out-of-distribution examples is significantly hampered by the spurious patterns. Looking deeper, \citet{liu2022simple, ming2022impact, van2020uncertainty} suggests that this failure mode in \gls{DNN} uncertainty can be caused by an issue in representation learning known as \textit{feature collapse}, where the model over-focused on correlational features that helps to distinguish between the output classes on the training data, but ignored the non-predictive but still semantically meaningful input features that are important for uncertainty quantification (\Cref{fig:2d_example}). In this work, we show that this failure mode can be provably mitigated by a training procedure we term \textit{introspective training}(\Cref{sec:method}). Briefly
introspective training adds an auxiliary \textit{introspection} task to model training, asking the model to predict whether an example belongs to the under-represented groups. 
It comes with a guanrantee in injecting \textit{bias-awareness} into model representation (\Cref{thm:bias_awareness}), encouraging it to learn diverse hidden features that distinguishes the minority-group examples from the majority group, even if these features are not correlated with the target labels on the training dataset. As a result, introspective training helps the model to circumvent the well-known pathology of \textit{feature collapse} under spurious correlation, leading to improved uncertainty quality for the tail groups (\Cref{fig:2d_example}). 

\textbf{Contributions:} In this work, we study the problem of improving a \gls{DNN} model's fairness-accuracy frontier by improving the training data distribution using active learning 
(\Cref{eq:al_objective_intro}).
%\vspace{-1em}
\begin{itemize}[noitemsep,topsep=0pt,leftmargin=0.5cm]
    \item We first introduce \textbf{\gls{ISP}}, a simple training approach to improve a \gls{DNN} model's uncertainty quality for the under-represented groups (\Cref{sec:method}). Using group annotations from the training data, \gls{ISP} conducts \textit{introspective training} to provably improves a \gls{DNN}'s representation and uncertainty quality for the tail groups. When the group annotation is not available, \gls{ISP} additionally estimates it using a cross-validation-based procedure that conducts a noise-bias-variance decomposition of model's generalization error \citep{domingos2000unified}.
    \item \textbf{Theoretical Analysis.} Complementing the method development, we conduct a initial theoretical analysis the optimization problem (\ref{eq:al_objective_intro}) under a group-specific learning rate model \citep{rolf2021representation} (\Cref{sec:theory}). Our result elucidates the role of training data distribution $\alpha$ in the model’s best-attainable accuracy-fairness frontier $F_\lambda$. In particular, it confirms the theoretical necessity of up-sampling the under-represented groups for obtaining the optimal accuracy-fairness frontier, and revealed an non-obvious fact that the notion of \textit{under-representation} is in fact a interplay of the subgroup's learning difficulty and its population prevalence.
    \item \textbf{Empirical Effectiveness.} Under two challenging real-world tasks (census income prediction and toxic comment detection), we empirically validate the effectiveness of \gls{ISP} training in improving a \gls{DNN} model's active learning performance under dataset bias. \gls{ISP} helped uncertainty-based \gls{AL} methods to achieve much improved tail-group sampling rate, meaningfully pushing the accuracy-fairness frontier of the final model.
\end{itemize}

==> introspective ensemble/sections/intro_bullet.tex <==
\jereliu{logic flow: accuracy-fairness frontier $\rightarrow$ importance of data distribution $\rightarrow$ active learning $\rightarrow$ caveat of deep learning uncertainty $\rightarrow$ ISP}
\balaji{Sycned with Jeremiah: these bullet points will eventually go away}

% Background:
% \begin{itemize}
% \item The modern \gls{DNN} models are commonly trained on the large-scale, in-the-wild datasets. \citep{deng2009imagenet}
% \item These data tend to exhibit an imbalanced long-tail distribution with many small population subgroups, reflecting the natural or societal mechanisms underlying the data generation process \citep{zhu2014capturing, yang2020rethinking, feldman2020neural}. 
% \item This imbalance in training data distribution (i.e., \textit{dataset bias}) has prevented the \gls{ML} models from generalizing equitably to the underrepresented population groups. \citep{hasnain2007disparities, ekstrand2018all, hofmanninger2020automatic}.
% \item In response, many spurious correlation and fairness research has focused on improving model training under a fixed and imbalanced training dataset, striving towards a balanced model performance that offers competitive utility (average-case performance) while ensuring fairness (e.g., worst-case performance) \citep{martinez2021blind, martinez2020minimax, agarwal2018reductions, sagawa2020investigation, liu2021just} (see \Cref{sec:related_debiasing_supervised} for a review).
% \item Formally, developing models with balanced accuracy-fairness tradeoff. Measured by accuracy-fairness frontier \citep{martinez2020minimax, martinez2021blind, agarwal2018reductions, little2022fairness}.
% \end{itemize}

% Goal:
% \begin{itemize}
% \item 
% However, fairness learning under a fixed dataset comes with inherent challenges.
% The limited size of the tail groups invariably restricts the model's worst-group performance, leading to a compromised frontier in the accuracy-fairness tradeoff  (i.e., a high value in the $min_{f \in \gF} F_\lambda(f|D)$)
% \citep{zhao2019inherent, dutta2020there%vzliobaite2015relation, menon2018cost
% }. 
% \item In this work, recognizing this inherent limitation brought by this imbalanced distribution, we ask an orthogonal question: \textit{under a fixed learning algorithm, can we ``break" the accuracy-fairness frontier of the model by improving the distribution of the training data?} That is, for example, given a fixed model class $\gF$ and denote $D_{\alpha, n}$ a size-$n$ training dataset with group-size allocation $\alpha = [\alpha_g]_{g \in \gG}$, we study that if we can improve the accuracy-fairness frontier $F_\lambda(f|D_{\lambda, n})$ by studying the outer optimization problem \citep{rolf2021representation}:
% \begin{align}
% F_\lambda^* = 
% {\color{Maroon} \min_{\alpha \in \Delta^{|\gG|}} }
% \Big[ \min_{f \in \gF} F_{\lambda}(f|D_{{\color{Maroon}\alpha},n}) \Big],
% \label{eq:al_objective_intro}
% \end{align}
% where $\Delta^{|\gG|}$ is the simplex of all possible group size allocations. 
% \item Concretely, we study uncertainty-based \glsfirst{AL} as an approach to optimize the above objective in practice. 
% We expect this direction to be fruitful: 
% By diversely sampling from the under-represented tail groups, \gls{AL} is expected to attain a well-balanced dataset that offers richer sets of examples from the tail population, helping the model $f \in \gF$ to naturally achieve a better performance for the worst-case group, and thereby ``breaking" the accuracy-fairness frontier otherwise ``locked" by an imbalanced data distribution without needing additional modeling change
% \citep{rolf2021representation, chen2018my, idrissi2022simple, branchaud2021can}.
% \end{itemize}

% Challenges:
% \begin{itemize}
%     \item (Caveat in Deep Uncertainty) 
%     However, \gls{DNN} models exhibits failure modes in the presence of spurious correlation and subpopulation shifts 
%     \citep{sagawa2020investigation}
%     \citep{tran2022plex}. Can be traced to issue in the embedding space \citep{liu2022simple}. 
%     \item (Unknown bias) There exists many situations where the sources of biases are unknown or hidden, where it is infeasible to manually categorize or annotate all sources of the underlying data biases due to its enormous size or the external regulatory constraints \citep{ekstrand2018all, veale2017fairer, holstein2019improving}.
%     \item (Secondary, Label Noise) Furthermore, labeling noise is known to be pervasive in real-world data curation process and annotation pipelines (more so for tail groups), creating additional challenges for bias estimation techniques  \citep{li2022more, northcutt2021pervasive}.
% \end{itemize}

% \vspace{5em}

Contribution I: Method
\begin{itemize}
    \item We propose \textit{\glsfirst{ISP}}, a simple approach to improve the uncertainty quality of a deep neural network under dataset bias. ISP adds an auxiliary \textit{introspection} task to model training, asking the model to predict whether an example belongs to an under-represented group. {\color{red} (mention representation learning guanrantee).}
    \item In the situation of unknown bias, \gls{ISP} estimates the bias label using a cross-validation-based \textit{self-play} procedure. It answers the aforementioned challenges by estimating bias label using noise-bias-variance decomposition \citep{domingos2000unified}
    .
\end{itemize}
\Cref{sec:related_work} surveys related work.

Contribution II: Theory
\begin{itemize}
    \item Complementing the method development, we also conduct an initial theoretical investigation to elucidate the role of training data distribution in the model's ability in obtaining the optimal accuracy-fairness frontier.
    \item Specifically, under a group-specific learning rate model \citep{chen2018my, rolf2021representation}, we derive the optimal group distribution $\alpha^*$ that minimizes the frontier risk (\ref{eq:frontier_risk}), analyzing how it interacts with both the empirical prevalence and the inherent learning difficulty of each group (\Cref{thm:optimal_allocation_frontier_main}).
    \item Our result reveals two simple yet non-obvious insights: 
    \begin{itemize}
        \item to attain optimal worst-group accuracy (i.e., the minimax group fairness \citep{rawls2001justice, lahoti2020fairness, martinez2020minimax, gil2022minimax}), the group distribution should be primarily informed by the relative learning difficulty of each group, rather than their existing prevalence in the data \citep{nam2020learning}.
        \item Furthermore, it confirms that to attain an optimal fairness-accuracy performance, a group needs to be upsampled only if their existing prevalence doesn't justify their learning accuracy. i.e., the definition of ``under-represented groups" is a joint property of the group's empirical prevalence and its learning difficulty.
    \end{itemize}
    \item Further justifying active sampling policy informed by model's  generalization error.
\end{itemize}

We conclude the paper with an empirical investigation.
Contribution III: Experiments



==> introspective ensemble/sections/related_work.tex <==
\subsection{Supervised and semi-supervised learning under dataset bias}
\label{sec:related_debiasing_supervised}

In recent years, there has been significant interest in studying robust generalization for long-tail population subgroups under dataset bias. The literature is vast and encompasses topics including fairness, debiasing, long-tail recognition, spurious correlation, distributional (i.e., domain or subpopulation) shift, etc. In the following, we focus on notable and recent work that is highly relevant to the \gls{ISP} approach, and refer to works such as \citet{caton2020fairness,mehrabi2021survey,hort2022bia} for an exhaustive survey.

Majority of the fairness and debiasing work focuses on the supervised learning setting, where the model only have access to a fixed and imbalanced dataset. Among them, the earlier work operated under the assumption that the source of dataset bias is completely known, and the group annotation is available for every training example. Then these group information is use to train a robust model by modify components of the training pipeline (e.g., training objective, regularization method, or composition of training data). For example, \citet{levy2020large, sagawa2019distributionally, zhang2020coping} proposes minimizing the worst-group loss via \glsfirst{DRO}, which is shown to be equivalent to ERM training on a well-curated training set in some settings \citep{slowik2022distributionally}; 
{\color{black} \gls{IRM} \citep{arjovsky2019invariant} proposes 
learning a classifier that is simultaneously optimal for all groups by learning a invariant representation.}
\citet{teney2021unshuffling, idrissi2022simple, byrd2019effect, xu2021understanding} studies the effect of group-weighted loss in model's fairness-accuracy performance, and REx \citep{krueger2021out} minimizes a combination of group-balanced and worst-case loss. Further, the recent literature has also seen sophisticated neural-network loss that modifies gradient for the tail-group examples. For example, LDAM \citep{cao2019learning} proposes to modify group-specific logits by an offset factor that is associated with group size, and equalization loss \citep{tan2020equalization} uses a instance-specific mask to suppress the ``discouraging gradients" from majority groups to the rare groups. 
On the regularization front, the examples include 
{\color{black} IRM$\_$v1  \citep{arjovsky2019invariant} that proposed to approximate the original \gls{IRM} objective through gradient penalty.
% appends a group-balanced loss with a gradient norm penalty.
} \textit{Heteroskedastic Adaptive Regularization} (HAR) \citep{cao2020heteroskedastic} imposes Lipschitz regularization in the neighborhood of tail-group examples. There also exists a large collection of work imposing other types of fairness constraints. 
% \todo{{\color{red} cite}} 
Finally, the third class of methods modifies the composition of the training data by enriching the number of obsevations in the tail groups, this includes \citet{sagawa2020investigation, idrissi2022simple} that study the impact of resampling to the worst-group performance, and \citet{goel2020model} that generates synthetic examples for the minority groups.
In the setting where the group information is available, our work proposes a novel approach (introspective training) that has both a theoretical guarantee and is empirically competitive than reweighted training.
% \todo{{\color{red} data augmentation \citep{mroueh2021fair}}}
% \todo{{\color{red} how does our method compares / fits in?}}

On the other hand, there exist a separate stream of work that allows for partial group annotation, i.e., the types of bias underlying a dataset is still completely known, but the group annotation is only available for a subset of the data. Most work along this direction employs semi-supervised learning techniques (e.g, confidence-threshold-based pseudo labeling), with examples include \gls{SSA} \citep{nam2020learning}, BARACK \citep{sohoni2021barack} and Fair-PG \citep{jung2022learning}. This setting can be considered as a special case of \gls{ISP} where we use group information as the underrepresentation label to train the $p(b|\rvx)$ predictor. However, our goal is distinct that we study the efficacy of this signal as an active learning policy, and also investigate its extension in the case where the label information is completely unobserved in the experiments \Cref{sec:exp_ablation}.
% \todo{{\color{red} how does our method compares / fits in?}}

% \todo{{\color{red} multi-task learning works on fairness?\citep{wang2021understanding}}}

\subsection{Estimating dataset bias for model debiasing} 
\label{sec:related_bias_estimation}
In the situation where the source of dataset bias is not known and the group annotation is unavailable, several techniques has been proposed to estimate proxy bias labels for the downstream debiasing procedures. These methods roughly fall into three camps: clustering, adversarial search, and using the generalization error from a biased model. 

For clustering, GEORGE \citep{sohoni2020no} and CNC \citep{zhang2021correct} proposed estimating group memberships of examples based on clustering the last hidden-layer output. For adversarial search, REPAIR \citep{li2019repair}, ARL \citep{lahoti2020fairness}, EIIL \citep{creager2021environment}, BPF \citep{martinez2021blind}, FAIR \citep{petrovic2022fair}, Prepend \citep{tosh2022simple} 
infers the group assignments by finding the worst-case group assignments that maximize certain objective function. {\color{black} For example, \textit{Environment Inference for Invariant Learning} (EIIL) \citep{creager2021environment} infer the group membership by maximizing the gradient-based regularizer from IRM$\_$v1.}

Estimating bias label using the error from a biased model is by far the most popular technique. These include \textit{forgettable examples} \citep{yaghoobzadeh2021increasing}, \textit{Product of Experts} (PoE) \citep{clark2019don, sanh2020learning}, DRiFt \citep{he2019unlearn} and \textit{Confidence Regularization} (CR) \citep{utama2020towards, utama2020mind} that uses errors from a separate class of weak models that is different from the main model; \textit{Neutralization for Fairness} (RNF) \citep{du2021fairness} and \textit{Learning from Failure} (LfF) that trains a bias-amplified model of the same architecture using generalized cross entropy (GCE); and\textit{ \glsfirst{JTT}} that directly uses the error from a standard model trained from cross entropy loss. 

Notably, there also exists several work that estimates bias label using ensemble techniques, this includes \textit{Gradient Alignment} (GA) \citep{zhao2021learning} that identifies the tail-group (i.e., bias-conflicting)  examples based on the agreement between two sets of epoch ensembles, \textit{Bias-conflicting Detection} (BCD) \citep{lee2022biasensemble} that uses the testing error of a biased deep ensemble trained with GCE, and \textit{Learning with Biased Committee} (LWBC) uses the testing error of a bootstrap ensemble.

To this end, our work proposes a novel \textit{self-play estimator} (\Cref{eq:bias_estimator}) that uses bootstrap ensembles to estimate the \textit{generalization gap} due to dataset bias. \textit{self-play estimator} has the appealing property of better controlling for label noise while more stably estimating model variance, addressing two weaknesses of the naive predictive error estimator used in the previous works.

% Finally, \citet{khan2019striking} uses the class-level and instance-level uncertainty to automatically reweight group-specific (i.e., class-specific) loss during training.

\subsection{Representation learning under dataset bias}

Originated from the fairness literature, 
{\color{black} the earlier work in debiased representation learning has focused on identifying a representation that improves a model's fairness properties, as measured by notions such as demographic parity (DP), equalized odds (EO), or sufficiency
\citep{arjovsky2019invariant, arjovsky2020out, creager2021environment, shui2022fair}. This is commonly achieved by striving to learn a representation that is invariant with respect to the group information.
% To this end, the earlier work in debiased representation learning has focused on techniques to eliminate the information of spurious features (e.g., protected attributes) from the model representation. 
Such methods are commonly characterized as \textit{in-processing methods} in the existing survey of the fairness literature
\citep{caton2020fairness, hort2022bia}, and was categorized into classes of approaches
}
including adversarial training \citep{beutel2017data, kim2019learning, ragonesi2021learning, zhu2021learning, madras2018learning}, regularization \citep{bahng2020learning, tartaglione2021end, arjovsky2019invariant}, contrastive learning \citep{shen2021contrastive, park2022fair, cheng2020fairfil} and its conditional variants \citep{gupta2021controllable, tsai2021conditionala, tsai2021conditionalb, chi2022conditional}, 
{\color{black} or explicit solutions to a bi-level optimization problem \citep{shui2022fair}. (Please see \citet{caton2020fairness, hort2022bia} for a complete survey).}
However, some later works questions the necessity and the sufficiency of such approaches. For example, some work shows that careful training of the output head along is sufficient to yield improved performance in fairness and bias mitigation \citep{kang2019decoupling, du2021fairness, kirichenko2022last}, and \citet{cherepanova2021technical} shows that models with fair feature representations do not necessarily yield fair model behavior.

At the meantime, a separate stream of work explores the opposite direction of encouraging the model to learn diverse hidden features. For example, \citet{locatello2019challenging, locatello2019fairness} establish a connection between the notion of feature disentanglement and fairness criteria, showing that feature disentanglement techniques may be
a useful property to encourage model fairness when sensitive variables are not observed. However, such techniques often involves specialized models (e.g., VAE) which restricts the broad applicability of such approaches. Some other work explores feature augmentation techniques to learn both invariant and spurious attributes, and use them to debias the output head \citep{lee2021learning}. Finally, a promising line of research has been focusing on using self-supervised learning to help the model avoid using spurious features in model predictions \citep{chen2020self, xie2020n, cai2021theory, hamidieh2022evaluating}. Our work follows this latter line of work by proposing novel techniques to encourage model to learn diverse features that is \textit{bias-aware}, but with a distinct purpose of better uncertainty quantification.

% \begin{itemize}
%     \item debiasing by suppressing learning spurious features \\
%     \begin{itemize}
%         \item adversarial training \citep{beutel2017data, kim2019learning, ragonesi2021learning, zhu2021learning}; 
%         \item regularization \citep{bahng2020learning, tartaglione2021end}
%         \item contrastive learning: \citep{shen2021contrastive, park2022fair, cheng2020fairfil} remove sensitive attribute information using  contrastive learning to maximising the similarities of instance pairs which share a main task label and minimising the similarities of such pairs from the protected attribute perspective .
%         \item conditional contrastive learning: Fair contrastive learning constructs positive and negative pairs with similiar attributes, fixing the outcome of the sensitive variable prevents the model from using the sensitive information to distinguish positive pairs from negative pairs. conditional sampling: CCL-K \citep{tsai2021conditionala},  Fair-InfoNCE \citep{tsai2021conditionalb} CS-InfoNCE\citep{chi2022conditional} \citep{gupta2021controllable}  minimizes the mutual information between representations and protected attributes.
%         \item Other techniques: removing the class-specific features of a random class to allow the model to learn de-correlated representations for each class, i.e., DropClass \citep{chu2021learning}.
%     \end{itemize}
%     \item yields questions:
%     \begin{itemize}
%         \item representation learned from biased data itself is fine. \\
%         \citep{kang2019decoupling, du2021fairness, kirichenko2022last}
%         \item Fair Feature Representations Do Not Yield Fair Model Behavior. \\
%         \citep{cherepanova2021technical}
%     \end{itemize}
%     \item learning diverse features \\
%     \begin{itemize}
%         \item Disentangled Feature Augmentation \citep{lee2021learning} (learn diverse feature by varying loss function and additional augmentation via feature permutation.
%         need knowledge of biased features, complicated procedure requiring scheduling augmentation.)
%         \item self-supervised learning \\
%         \citep{chen2020self, xie2020n, cai2021theory}
%         % \citep{kumar2022calibrated}
%         \citep{hamidieh2022evaluating}
%     \end{itemize}
% \end{itemize}

\subsection{Active learning under dataset bias}

In recent years, the role of training data in ensuring the model's fairness and bias-mitigation performance has been increasing noticed. Notably, \citep{chen2018my} presented some of the earlier theoretical and empirical evidence that increasing training set size along is already effective in mitigating model unfairness. Correspondingly, under the assumption that the \textit{group information in the unlabelled set is fully known}, there has been several works that studies group-based sampling strategies and their impact on model behavior. For example, \citet{rai2010domain, wang2014active} shows group-based active sampling strategy improves model performance under domain and distributional shifts, and \citet{abernethy22active} proves a guarantee for a worst-group active sampling strategy's ability in helping the SGD-trained model to convergence to a solution that attains min-max fairness.
A second line of research focuses on designing better active learning objectives that incorporates fairness constraints, e.g., \textit{Fair Active Learning (FAL)} \citep{anahideh2022fair} and \textit{PANDA} \citep{sharaf2022promoting}. \citet{agarwal2022does} introduce a data repair algorithm using the coefficient of variation to curate fair and contextually balanced data for a protected class(es).
Furthermore, there exists few active learning works formulating the objective of their method as optimizing a fairness-aware objective. For example, \textit{Slice Tuner} \citep{tae2021slice} proposes adaptive sampling strategy based on per-group learning curve to minimize fairness tradeoff, performs numeric optimization. \citet{cai2022adaptive} which formalized the fairness learning problem as an min-max optimization objective, however their did not conduct further theoretical analysis of their objective, but instead proposed a per-group sampling algorithm based predicted model error using linear regression. 
{\color{black}
Finally, a recent line of active learning work has been well-developed to formulate active learning from the perspective of distributional matching between labeled and unlabeled datasets. \citep{shui2020deep, de2021discrepancy, mahmood2021low, xie2022active}. These approaches are well-equipped to hand distributional shift, but often comes with the cost of assuming knowledge of the test feature distribution at the training time \citep{shui2020deep, de2021discrepancy, mahmood2021low, xie2022active}.} 
In comparison, our work conducts theoretical analysis of the optimization problem \Cref{sec:theory}, and our proposed method (\gls{ISP}) does not require a priori knowledge (e.g., group information) from the unlabelled set.

On the other hand, there exists active re-sampling methods that do not require the knowledge of group information in the unlabelled set. For example, \citet{amini2019uncovering} learns the data distribution using a VAE model under additional supervision of class / attribute labels, and then perform IPW sampling with respect to learned model. REPAIR \citep{li2019repair} that estimates dataset bias using prediction error of a weak model, and then re-train model via e.g., sample re-weighting based on the estimated bias. The bias estimation method used in this work is analogous to that of the \gls{JTT}, which we compare with in our work. A work close to our direction is \citet{branchaud2021can}, which shows \gls{DNN} uncertainty (i.e., BatchBALD with Monte Carlo Dropout \citep{kirsch2019batchbald}) helps the model to achieve fairness objectives in active learning on a synthetic vision problem. Our empirical result confirms the finding of \citet{branchaud2021can} on realistic datasets, and we further propose techniques to improve the vanilla \gls{DNN} uncertainty estimators for more effective active learning under dataset bias.

As an aside, a recent work \citet{farquhar2020statistical} studies the statistical bias in the estimation of active learning objectives due to the non-i.i.d. nature of active sampling. This is separate from the issue of dataset bias (i.e., imbalance in data group distribution) which we focus on in this work.

% \begin{itemize}
%     \item Simply increasing training set size without changing data distribution can already decrease unfairness \citep{chen2018my}
%     \item known group information
%     \begin{itemize}
%         \item re-sampling: group-balanced sampling strategy  \citep{rai2010domain, wang2014active}
%         \item Theory: \citep{abernethy22active} proves an guarantee for gradient descent model trained under a worst-group active sampling strategy convergence to a min-max fair solution.
%         \item \gls{AL} objective design: Fair Active Learning (FAL) \citep{anahideh2022fair} and PANDA \citep{sharaf2022promoting} incorporate group-based fairness constraint into objective, which needs complete group information. \citet{agarwal2022does} introduce a data repair algorithm using the coefficient of variation to curate fair and contextually balanced data for a protected class(es).
%         \item Related work by solving fairness objectives:
%         \begin{itemize}
%             \item \citep{cai2022adaptive} formalized the fairness learning problem as an min-max optimization objective, did not conduct theoretical analysis. proposed a per-group sampling algorithm based predicted model error using linear regression.
%             \item Slice Tuner \citep{tae2021slice} proposes adaptive sampling strategy based on per-group learning curve to minimize fairness tradeoff, performs numeric optimization.
%         \end{itemize}
%         \item \citep{li2022more} studies active learning under fairness constraints in the Presence of Label Bias, emphasizing the importance of explicitly differentiating between the types of bias that fairness-aware algorithms aim to address, and highlighting the risks of neglecting label error during data collection. Our work as an initial attempt to address this challenge, where we control for the impact of label noise in a model's sampling policy via noise-bias-variance decomposition in the bias signal estimation.
%     \end{itemize}
%     \item unknown group information
%     \begin{itemize}
%         \item bias estimation (using weak model error / VAE / clustering) then re-sampling:
%         \begin{itemize}
%             \item REPAIR \citep{li2019repair} (quantify bias using prediction error of a weak model, then re-train model via bias-based sample reweighting.)
%             \item \citep{amini2019uncovering} (use generative model (VAE) to learn data distribution (there's additional supervision of encoder via known class / attribute labels), then perform IPW sampling with respect to learned model).
%         \end{itemize}
%         \item uncertainty
%         \begin{itemize}
%             \item MCD+BALD \citep{branchaud2021can}
%         \end{itemize}
%     \end{itemize}
%     \item different notion of bias: \citep{farquhar2020statistical}
% \end{itemize}

\subsection{Uncertainty estimation with \gls{DNN}s} 

In recent years, the probabilistic \gls{ML} literature has seen a plethora of work that study enabling calibrated predictive uncertainty in \glspl{DNN}s. Given a model $f$, the probabilistic \gls{DNN} model aims to learn a predictive distribution for the model function $f$, such that given training data $D=\{(y_i, \rvx_i)\}_{i=1}^n$ and a testing point $\rvx_{test}$, the model outputs a predictive distribution $f(\rvx_{test}) \sim P(f|\rvx_{test}, D)$ rather than a simple point prediction. To this end, the key challenge is to learn a predictive distribution (implicitly or explicitly) during the SGD-based training process of \gls{DNN}, generating calibrated predictive uncertainty without significantly impacting the accuracy or latency when compared to a deterministic \gls{DNN}.

To this end, the classic works focus on the study of Bayesian neural networks (BNNs) \citep{neal2012bayesian}, which took a full Bayesian approach by \textit{explicitly} placing priors to the hidden weights of the neural network, and performance MCMC or variance inference during learning. Although theoretically sound, BNN are delicate to apply in practice, with its performance highly dependent on prior choice and inference algorithm, and are observed to lead to suboptimal predictive accuracy or even poor uncertainty performance (e.g., under distributional distribution shift) \citep{wenzel2020good, izmailov2021bayesian}. Although there exists ongoing works that actively advancing the BNN practice (e.g., \cite{dusenberry2020efficient}). On the other hand, some recent work studies computationally more approaches that \textit{implicitly} learn a predictive distribution as part of deterministic SGD training. Notable examples include Monte Carlo Dropout \citep{gal2016dropout} which generates predictive distribution by enabling the random Dropout mask during inference, and ensemble approaches such as Deep Ensemble \citep{lakshminarayanan2017simple} and their later variants \citep{maddox2019simple,wenzel2020hyperparameter,havasi2020training} that trains multiple randomly-initialized networks to learn the  modes of the posterior distribution of the neural network weights \citep{wilson2020bayesian}. Although generally regarded as the state-of-the-art in deep uncertainty quantification, these methods are still computationally expensive, requiring multiple \gls{DNN} forward passes at the inference time.

At the meantime, a more recent line of research avoids probabilistic inference for the hidden weights altogether, focusing on learning a scalable probabilistic model (e.g., Gaussian process) to replace the last dense layer of the neural network \citep{van2020uncertainty,van2021feature,liu2022simple,collier2021correlated}. A key important observation in this line of work is the role of hidden representation quality in a model's ability in obtaining high-quality predictive uncertainty. In particular, \citet{liu2022simple, van2020uncertainty} suggests that this failure mode in \gls{DNN} uncertainty can be caused by an issue in representation learning known as \textit{feature collapse}, where the \gls{DNN} over-focuses on correlational features that help to distinguish between output classes on the training data, but ignore the non-predictive but semantically meaningful input features that are important for uncertainty quantification. \citep{ming2022impact} also observed that \gls{DNN} exhibits particular modes of failure in \gls{OOD} detection in the presence of dataset bias. Later, \citet{tran2022plex, minderer2021revisiting} suggests that this issue can be partially mitigated by large-scale pre-traininig with large \gls{DNN}s, where larger pre-trained \gls{DNN}'s tend to exhibit stronger uncertainty performance even under spurious correlation and subpopulational shift. In this work, we confirm this observation in the setting of dataset bias in \Cref{fig:2d_example}), and propose simple procedures to mitigate this failure mode in representation learning without needing any change to the \gls{DNN} model, and illustrates improvement even on top of large-scale pre-trained \gls{DNN}s (BERT).

% \citep{collier2021correlated}

% \citet{setlur2022adversarial} improves model uncertainty in out-of-domain situations by training the model to be less confident on adversarial examples.\\

\textbf{Deep uncertainty methods in active learning.} Active learning with \gls{DNN}s is an active field with numerous theoretical and applied works, we refer to \citet{matsushita2018deep, ren2021survey} for comprehensive survey, and only mention here few notable methods that involves \gls{DNN} uncertainty estimation techniques. Under a classification model, the most classic approach to uncertainty-based active learning is to use the predictive distribution's entropy, confidence or margin as the acquisition policy \citep{settles1994active}. Notice that in the binary classification setting, these three acquisition policy are rank-equivalent since they are monotonic to the distance between $max[p(\rvx), 1-p(\rvx)]$ and the null probability value of 0.5. On the other hand, \textit{\gls{BADGE}} \citep{ash2019deep} proposes to blend diversity-based acquisition policy into uncertainty-based active learning, by applying k-means++ algorithm to the gradient embedding of the class-specific logits (which quantifies uncertainty). As a result, \textit{\gls{BADGE}} may also suffer from the pathology in model representation under dataset bias, which this work is attempt to address. 

Finally, \cite{houlsby2011bayesian} has proposed a information-theoretic policy \gls{BALD}, which measures the mutual information between data points and model parameters and is adopted in the deep uncertainty literature \citep{gal2017deep, kirsch2019batchbald, kothawade2022clinical}. However, stable estimation of mutual information can be delicate in practice, and we leave the investigation of these advanced acquisition policies under dataset bias for future work.

% Survey \citep{ren2021survey}

% \paragraph{Bias-variance decomposition in machine learning}

% \paragraph{Pareto frontier of accuracy-fairness tradeoff}
% \citep{martinez2021blind}


==> introspective ensemble/sections/theory_long.tex <==

Given a dataset $D_{\alpha,n}$ with sample size $n$ and group allocation $\alpha=\{\alpha_g\}_{g\in \gG}$, we denote $f_D$ the model learned from $D$. We also denote the group-specific distribution as $D_g=P(y, \rvx|G=g)$, and the group-specific generalization error of a given model $f$ is $R(f|G=g)=E_{D_g} \big[ L(y, f|D_g) \big]$. Finally, denote $\Delta^K$ the space of $K$-simplex so that $\forall \alpha=[\alpha_1, \dots, \alpha_K] \in \Delta^K$, it satisfies $\sum_k \alpha_k = 1$ and $\alpha_k > 0 \, \forall k$. 

We consider the below notion of accuracy-fairness frontier:
\begin{definition}[Accuracy-fairness Frontier Risk] Given a predictive function $f$, let $R(f|\alpha, n)\coloneqq \sum_{g\in \gG} \gamma_g R(f|G=g)$ be the standard empirical risk, and $\tilde{R}(f|\alpha, n)$ be the \textit{``fairness" risk} which is the worst-case risk among the groups $g\in \gG$:
$$\tilde{R}(f|\alpha, n) \coloneqq \sup_v \sum_{g\in \gG} [ v_g R(f|G=g)],$$ 
\vspace{-1.5em}

where $v \in \Delta^{|\gG|}$. Then, for non-negative weighting coefficients $\omega=\{\omega_1, \omega_2\}$, the accuracy-fairness frontier risk is defined as:
\begin{align}
F_{\omega}(f|\alpha, n) \coloneqq 
\omega_1 * R(f|\alpha, n) + \omega_2 * \tilde{R}(f|\alpha, n).    
\label{eq:frontier_risk}
\end{align}
\vspace{-2em}
\label{def:fairness_accuracy_frontier}
\end{definition}
% related work \citep{zhao2019inherent, menon2018cost, little2022fairness}

The form of the frontier risk in \Cref{def:fairness_accuracy_frontier} is common among objective functions in fairness literature, i.e., $F_\omega \propto R + \frac{\omega_2}{\omega_1} \tilde{R}$, where the standard risk $R$ is combined with a ``fairness constraint" $\tilde{R}$ under a trade-off parameter $\frac{\omega_2}{\omega_1}$. Then, for a fixed dataset, a point $(\tilde{r}, r^*)$ on the accuracy-fairness frontier can be identified by fitting a sequence of candidate models under different degrees of fairness-accuracy trade-off $\frac{\omega_2}{\omega_1}$, and then identify the best-achievable accuracy risk  $r^*$ among the models whose accuracy risk $\tilde{R}$ is less than $\tilde{r}$ \citep{little2022fairness}. Clearly, due to the Lagrangian form of \Cref{eq:frontier_risk}, a lower value of $F_\omega$ indicates a better accuracy-fairness tradeoff.

% In practice, a common goal is to search along the frontier to identify a model $f$ that attains the lowest fairness risk $\tilde{R}$ under the condition that its utility is above certain threshold (i.e., the standard risk $R > \lambda$). As we will show, this is equivalent to searching for a $f$ that minimizes \cref{eq:frontier_risk} under a particular value of $\frac{\omega_2}{\omega_1}$.

% When $\frac{\omega_2}{\omega_1}=1$, the frontier risk $F_{\omega}(f|\alpha, n)$ has a geometric interpretation as the perimeter of the rectangle defined by a point on the accuracy v.s. fairness trade-off curve (up to a scaling constant). 
% Given a trade-off level $\frac{\omega_2}{\omega_1}$, a model $f$ that attains a lower $F_\omega$ effectively attains a more advanced accuracy - fairness performance. 

To date, most of the prior work have focused on improving model performance by studying algorithms that better solve $\min_{f \in \gF} F_{\omega}(f|\alpha=\gamma, n)$ under a fixed (imbalanced) dataset \citep{martinez2020minimax, sagawa2019distributionally}, where $\gamma=\{\gamma_g\}_{g\in \gG}$ is the imbalanced group prevalences in the population. 

In this work, recognizing that the data imbalance can impose an inherent limitation on model performance 
%\citep{zhao2019inherent}
(i.e., \cref{eq:error_decomposition})
, we ask an orthogonal question: \textit{under a fixed learning algorithm, can we ``break" the accuracy-fairness frontier of the method by improving the distribution of the training data?} That is, we study the outer problem of the below optimization objective:
$$\alpha^* = 
{\color{Maroon} \argmin_{\alpha \in \Delta^{|\gG|}} }
\Big[ \min_{f \in \gF} F_{\omega}(f|\alpha, n) \Big]$$
where $\alpha \in \Delta^{|\gG|}$ is the allocation of group sizes in the training data. This question is of particular importance in active learning, {\color{red} because...}

In this section, our goal is to obtain an initial understanding of the potential impact of training data's group distribution in the resulting model's accuracy-fairness performance. Specifically, we would like to understand if and how a data group's population prevalence $\gamma_g$ and learning difficulty (in terms of finite-sample learning rate $o(c_g n^{-p_g})$) plays a role in the optimal distribution $\alpha^*$ that minimizes different fairness-relevant risk objectives. 

To maintain mathematical tractability in this initial analysis, we follow the previous literature to consider the below simple theoretical model for group-specific scaling laws for generalization error \citep{chen2018my, rolf2021representation}:

\begin{assumption}[Group-specific generalization error  \citep{rolf2021representation}]
The group-specific generalization error $R(f_{D}|G=g)=E_{D_g}(L(y, f_D))$ can be approximated by a scaling function of the group sample size $n_g$ and the total sample size $n$. That is, $\exists \, M_g >0$ and  constants $c_g, \tau_g, \delta_g \geq 0$, $p_g, q_g > 0$ such that for a dataset $D_{\alpha, n}$ with sample size $n$ and group allocation $\alpha=\{\alpha_g\}_{g\in \gG}$, and $f_{D_{\alpha, n}}$ the model trained $D$ with a particular algorithm, the generalization error $R(f_{D_{\alpha, n}}|G=g)$ can be approximated as:
\begin{align}
%\nonumber
R(f_{D_{\alpha, n}}|G=g) &\approx 
r(n_g, n | c_g, \tau_g, \delta_g, p_g, q_g) 
= c_g * n_g^{-p_g} + \tau_g * n^{-q_g} + \delta_g.
\label{eq:group_scaling_law}
\end{align}
The above is assumed to hold for any $\alpha \in \Delta^{|\gG|}$ and any $n$ such that $n_g = \lfloor \alpha_g n \rfloor \geq M_g$.
\vspace{-0.5em}
\label{def:group_scaling_law}
\end{assumption}
Assumption \ref{def:group_scaling_law} essentially states that each group has an unique learning rate $o(c_g n^{-p_g} + \tau_g n^{-q_g})$, which includes a $\tau_g n^{-q_g}$ term to allow data from other groups to influence the risk of group $g$. The scaling coefficients $(c_g, \tau_g, p_g, q_g)$ describes the difficulty of the learning problem, where higher values of $(c_g, \tau_g)$ and lower values of $(p_g, q_g)$ indicate that the group $g$ is more difficult to learn (i.e., the generalization error decreases slower with respect to sample size). Note that for common choices of loss function, we expect $p_g, q_g$ to be bounded in a small range (e.g.,  $p_g, q_g  < 1$ for squared loss, since the optimal parametric learning rate is $n^{-1}$ \citep{bach2017breaking}). It should be acknowledged that the Assumption \ref{def:group_scaling_law} is simplistic, as it assumes that the scaling coefficients $(c_g, \tau_g, p_g, q_g)$ are not impacted by the group composition of the training data $\alpha$. However, \citet{rolf2021representation} shows that it is indeed true in classic settings such as linear regression with group-specific intercepts {\color{red} (add more detail)}, and empirically verified that \cref{eq:group_scaling_law} approximated holds in, e.g., image classification tasks using ResNet models.

To this end, the below theorem 
% elucidates the importance of the training data's group-size allocation on the resulting model's fairness - accuracy performance. Importantly, \Cref{thm:optimal_allocation_frontier_main} theoretically
confirms that a model's fairness-accuracy frontier can be improved by careful design of the training data (i.e., by sufficiently representing data groups that are under-represented in the population). 
%This necessity notably does not vanish even under extremely large $n$, thereby highlighting the fact that the {\color{Maroon} \textit{data bias}} error in (\ref{eq:error_decomposition}) persists even in the asymptotics. 
Interestingly, it also provides a mathematical characterization for the heuristic notion of ``under-represented group" in the fairness literature (i.e., \cref{eq:minority_group_criteria_main}), in terms of whether a group's population prevalence $\gamma_g$ is comparable to its relative learning difficulty (as characterized by learning rate coefficients $c_g$, $p_g$ (\cref{eq:group_scaling_law})) when compared to the rest of the groups.

\begin{theorem}[Optimal Group-size Allocation for Fairness-Accuracy Frontier]
Assuming the group-specific scaling laws (Definition \ref{def:group_scaling_law}) differ only by the multiplicative coefficient $c_g$, so that the approximated group-specific risk is $\hat{R}(f_{D_{\alpha, n}}|G=g) \coloneqq c_g n^{-p} + \tau n^{-q} + \delta$. Denote the approximate population risk as $\hat{R}(\alpha, n) = \sum_g \gamma_g \hat{R}(f_{D_{\alpha, n}}|G=g)$ and the approximated worst-case risk as $\hat{\tilde{R}}(\alpha, n) = \sup_v \sum_{g\in \gG} [ v_g \hat{R}(f_{D_{\alpha, n}}|G=g)]$. Then:
\begin{itemize}[leftmargin=0.5cm]
\item [(I)] \textbf{(Population Risk},  \citet{rolf2021representation})  If  $F_{\omega=\{1,0\}}(\alpha, n)=R(\alpha, n)$ is the standard population risk. The optimal training-data group distribution $\alpha^*$ that minimizes $\hat{R}(\alpha, n)$ is
$\alpha^*_g = 
\frac{(\gamma_g c_g)^{1/(p+1)} }
{\sum_{g\in \gG}(\gamma_g c_g)^{1/(p+1)}}.$
\item [(II)] \textbf{(Worst-case Risk)} If  $F_{\omega=\{0, 1\}}(\alpha, n)=\tilde{R}(\alpha, n)$ is the worst-case risk. The optimal 
training-data group distribution $\tilde{\alpha}^*$ that minimizes $\hat{\tilde{R}}(\alpha, n)$ is
$\tilde{\alpha}^*_{g} = 
\frac{(c_g)^{1/p} }
{\sum_{g\in \gG}(c_g)^{1/p}}$, i.e., the relative learning difficulty of group $g$.
% \item [(III)] \textbf{(Fairness-Accuracy Frontier, Average-group Risk)} 
% Let $R_{fair}$ be the average-group risk $\bar{R}(\alpha, n)$ so that
% $F_{\omega}(\alpha, n) \coloneqq 
% \omega_1 * R(\alpha, n) + \omega_2 * \bar{R}(\alpha, n)$.
% The optimal training-set group-size allocation $\alpha^*$ that minimizes the approximated accuracy-fairness frontier $\hat{F}_\omega(\alpha, n)$ is: 
% \begin{align*}
% \alpha^*_g = \frac{(r_g c_g)^{1/(p+1)}}{\sum_{g\in \gG} (r_g c_g)^{1/(p+1)}}, 
% \quad \mbox{where} \quad
% r_g = \omega_1  \gamma_g + \omega_2 \frac{1}{|\gG|}.
% \end{align*}
\item [(III)] \textbf{(Fairness-Accuracy Frontier Risk)} 
For general $\omega>\mathbf{0}$, the optimal training-set group distribution $\alpha^*$ that minimizes the  $\hat{F}_\omega(\alpha, n) \coloneqq 
\omega_1 \hat{R}(\alpha, n) + \omega_2 \hat{\tilde{R}}(\alpha, n)$ is: 
\begin{align}
\alpha^*_g = \frac{(r_g c_g)^{1/(p+1)}}{\sum_{g\in \gG} (r_g c_g)^{1/(p+1)}}, 
\quad \mbox{where} \quad
r_g = \max\Big[
\gamma_g, \;\;
\Big(\frac{\omega_2}{\omega_1} + \sum_{g \in \gB} \gamma_{g} \Big)\Big( \frac{c_g^{1/p}}{\sum_{g \in \gB} c_g^{1/p}} \Big) \Big].
\label{eq:optimal_sampling}
\end{align}
Here $\gB \subseteq \gG$ is the set of under-represented groups whose population prevalence $\gamma_g$ satisfy:
\begin{align}
\gB \coloneqq 
\Bigg\{ g \Big|
\gamma_g \leq 
\Big(\frac{\omega_2}{\omega_1} + \sum_{g \in \gB} \gamma_{g} \Big)\Big( \frac{c_g^{1/p}}{\sum_{g \in \gB} c_g^{1/p}} \Big)
\Bigg\}.
\label{eq:minority_group_criteria_main}
\end{align}
Furthermore, a sufficient condition for $g \in \gB$ is
$\gamma_g 
< 
\frac{\omega_2}{\omega_1} * (\frac{c_g^{1/p}}{\sum_{g \in \gG} c_g^{1/p}})$, where
$\frac{c_g^{1/p}}{\sum_{g \in \gG} c_g^{1/p}}$ is the relative learning difficulty of group $g$, and $\frac{\omega_2}{\omega_1}$ the relative weights of the worst-case and population risks.
\end{itemize}
\label{thm:optimal_allocation_frontier_main}
\end{theorem}
Proof is in \Cref{sec:optimal_allocation_frontier_proof}. In the above, Part (I) (Population Risk) is due to \citet{rolf2021representation}, it shows a striking fact that the optimal group sizes $\alpha^*$ minimizing the approximated empirical risk is \textit{not} the empirical distribution $\gamma=\{ \gamma_g \}_{g \in \gG}$, thereby highlighting the importance of training data design in achieving optimality in even the standard generalization performance\footnote{In \Cref{thm:allocation_weighted_risk} 
(\Cref{sec:lemma}), we go beyond the previous work to show that in a more general setting where the group-specific scaling coefficient $p_g$ is not equal, the optimal sampling allocation $\alpha^*$ in fact disproportionally favors the more difficult-to-learn groups as $n \rightarrow \infty$.}. Parts (II)-(III) are new to this work. Specifically, (II) highlights that to optimize the model's fairness performance (as measured by worst-case risk $\tilde{R}$), the group sizes in the training data should be proportional to the group's inherent learning difficulty (as characterized by $c_g^{1/p}$), \textit{irrespective} to the prevalence of these groups in the population $\gamma_g$. Finally, (III) highlights that the accuracy-fairness trade-off under a fixed learning algorithm can be improved by properly sample the data groups.
%should be sampled according to whether it is \textit{under-represented}, i.e., if its population prevalence $\gamma_g$ does not sufficiently reflect its relative learning difficulty  {\scriptsize $c_g^{1/p}/(\sum_g c_g^{1/p})$} (\cref{eq:minority_group_criteria_main}).
In particular, under the assumption that we have oracle knowledge of the scaling laws $c_g n_g^{-p} + \tau n^{-1} + \delta$, Part (III) hints at a sampling procedure that guarantees optimality: Given a data group $g \in \gG$, if $g$ doesn't belong to the under-represented group $\gB$, sample it  according to a likelihood function that is proportional to population prevalence $\gamma_g$, otherwise sample it according to a likelihood function (\cref{eq:optimal_sampling}) that is lower bounded by the group's relative learning difficulty $c_g^{1/p}/(\sum_g c_g^{1/p})$ scaled by the relative weight of the fairness and accuracy risks $\omega_2 / \omega_1$. 

{\color{red} Outline for transitioning paragraph below:}

{\color{red}
Begs the question.
\begin{enumerate}
    \item how to sample when group membership / group-specific scaling law are not known? Answer: use generalization error. empirically verified by \citep{liu2021just}.
    \item how to sample in active learning. where the generalization error is not known for sampling candidates? Answer: introspective training. Importantly, not only provides an estimate of generalization error, but also a guanrantee in bias-awareness.
    Improve uncertainty-sampling performance.
\end{enumerate}
}
 
{(Introduce Introspective Self-play)

Intuition: predict under-represented group / generalization error.

Deep implication in uncertainty-awre active learning under dataset bias: 
\begin{itemize}
    \item Injects bias-awareness into model representation.
    \item Improves bias-awareness in uncertainty quantification.
\end{itemize}
Improved model uncertainty under dataset bias / spurious correlation.
}

==> preamble/packages.tex <==
\usepackage[acronym,nowarn,section,nonumberlist]{glossaries}
\usepackage{lipsum}  

\usepackage[utf8]{inputenc} % allow utf-8 input
%\usepackage[T1]{fontenc}    % use 8-bit T1 fonts

\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{wrapfig}

% Set space.
\usepackage[nodisplayskipstretch]{setspace}

% Use fancyhdr package
\RequirePackage{multicol}
\RequirePackage{multirow}
\RequirePackage{colortbl}
\RequirePackage{fancyhdr}
\RequirePackage{color}


\RequirePackage{algorithm}
\RequirePackage{algorithmicx}
\usepackage[noend]{algpseudocode}

%\usepackage{algorithm}
%\usepackage{algorithmicx}
%\usepackage{algpseudocode}
\RequirePackage{natbib}
\RequirePackage{eso-pic} % used by \AddToShipoutPicture 
\RequirePackage{forloop}

% Recommended, but optional, packages for figures and better typesetting:
\usepackage{microtype}
\usepackage{graphicx}
\usepackage[export]{adjustbox}

\usepackage[font=scriptsize]{caption}
\usepackage{subcaption}
\usepackage{booktabs} % for professional tables
\usepackage{draftfigure}

\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{mathtools}
\usepackage{amsfonts}
\usepackage{mathptmx}
\usepackage{soul}

%\usepackage{lipsum}

% hyperref makes hyperlinks in the resulting PDF.
% If your build breaks (sometimes temporarily if a hyperlink spans a page)
% please comment out the following usepackage line and replace
% \usepackage{icml2019} with \usepackage[nohyperref]{icml2019} above.
%\usepackage{color}
% \usepackage[dvipsnames,table]{xcolor}
% \definecolor{mydarkblue}{rgb}{0,0.08,0.45}
% \usepackage[colorlinks,citecolor=mydarkblue,urlcolor=mydarkblue,linkcolor=mydarkblue
% ]{hyperref}
%\usepackage{hyperref}
\usepackage{cleveref}
\usepackage{comment}
\usepackage[hang,flushmargin]{footmisc}
      % hyperlinks
\usepackage{url}
% 
\def\UrlBreaks{\do\/\do-}
\usepackage{breakurl}% simple URL typesetting
%

% Attempt to make hyperref and algorithmic work together better:
%\newcommand{\theHalgorithm}{\arabic{algorithm}}

% use glossary
\usepackage
[acronym,nowarn,section,nonumberlist]{glossaries}
\glsdisablehyper{}

% import external document
\usepackage{xr}


% theorem
% adding two lines to avoid conflict in package https://tex.stackexchange.com/questions/43835/conflict-between-amsthm-and-some-other-package
\let\proof\relax
\let\endproof\relax
\usepackage{amsthm}
\usepackage{apptools}

% custom toc
\usepackage[page,header]{appendix}
\usepackage{titletoc}
\usepackage{etoc}

% itemize environment
\usepackage{enumitem}


==> proof/group_detection.tex <==
\subsection{Proof for Theorem \ref{thm:group_detect_guanrantee_app}}

\begin{proof}
By Bayes' rule, we have:
\begin{align}
P(g=1|F(l)>q) &= P(F(l)>q|g=1) * \frac{P(g=1)}{P(F(l)>q)}
\label{eq:detection_precision_0}
\end{align}

\underline{Expression for $P(g=1)$ and $P(F(l)>q)$}

Notice that $P(g=1)=1-\gamma_0$, and $P(F(l)>q)=P(U>q)=1-q$ for $U \sim Unif(0, 1)$. Here we used the fact that $F(l) \sim Unif(0, 1)$ when $F$ is the \gls{CDF} for the distribution of the random variable $l$ \citep{blitzstein2015introduction}. 

\underline{Expression for $P(F(l)>q|g=1)$}

Notice $P(F(l)>q|g=1)=P(F(l_1) > q)$, where $l_1=L(\tilde{y}_1, f_y(\rvx_1)), (\tilde{y}_1, \rvx_1)\sim P_1$ is the random variable for the minority-group loss.
Also notice that $F(l_1)=P(l' < l_1)$ where $l'=L(y', f_y(\rvx'))$ for $(y', \rvx', g')\sim P$ is the non-group-specific loss.  Then a conditional decomposition of $P(F(l_1)>q)$ reveals :
\begin{align*}
%P(F(l)>q|g=1) &= 
P(F(l_1)>q) &= P[P(l' < l_1)>q]\\
&= P \big[P(l' < l_1)>q | g'=0 \big]P(g'=0) + 
P\big[P(l' < l_1)>q| g'=1 \big]P(g'=1) \\
&= P \big( F_0(l_1)>q \big)\gamma_0 + (1-q)(1-\gamma_0),
\end{align*}
where the last equality follows since $P(g'=0)=\gamma_0, P(g'=1)=1-\gamma_0$ and $P\big[P(l' < l_1)>q \big]=P\big[F_1(l_1)>q \big]=P(U > q)=1-q$ for $U\sim Unif(0, 1)$. Here we again used the fact that $F_1(l_1) \sim Unif(0, 1)$ when $F_1$ is the \gls{CDF} for the distribution of $l_1$ \citep{blitzstein2015introduction}. 

\underline{Lower bound for $P \big( F_0(l_1)>q \big)$}

Lower bound $P \big( F_0(l_1)>q \big)$ by deriving a Cantelli-type inequality using the second moment method \citep{lyons2017probability}. Specifically, for a random variable $R$ with $E(R) \geq 0$, we have:
\begin{align*}
E(R)^2 \leq E(R * 1_{R>0})^2 &\leq E(R^2) P(R>0) 
\quad \mbox{which implies} \quad
\frac{P(R>0)}{1-P(R>0)} \geq \frac{E(R)^2}{Var(R)}.
\end{align*}
Setting $R=F_0(l_1) - q$, we have:
\begin{align*}
\frac{P \big( F_0(l_1)>q \big)}{1-P(F_0(l_1)>q)} &\geq \frac{(E(F_0(l_1))-q)^2}{Var(F_0(l_1))} = z^2, 
\quad \mbox{which implies} \quad 
P(F_0(l_1)>q) \geq \frac{z^2}{1 + z^2}
\end{align*}

\underline{Derive the final bound}

Finally, using the above three facts, we can express \Cref{eq:detection_precision_0} as:
\begin{align*}
P(g=1|F(l)>q) 
&= P(F(l)>q|g=1) * \frac{P(g=1)}{P(F(l_1)>q)} 
% \\
= P(F(l)>q|g=1) * \frac{1-\gamma_0}{1-q} 
% \\
% &= \Big( P \big( F_0(l_1)>q \big)\gamma_0 + (1-q)(1-\gamma_0) \Big) * \frac{1-\gamma_0}{1-q} \\
% &\geq  \Big( \frac{z^2}{1 + z^2} * \gamma_0 + (1-q)(1-\gamma_0) \Big) * \frac{1-\gamma_0}{1-q} \\
% &= (1-\gamma_0)^2 + \gamma_0 * \frac{1-\gamma_0}{1-q} *  \frac{z^2}{1 + z^2},
% \label{eq:detection_precision_1}
\end{align*}
which further leads to:
\begin{alignat*}{2}
P(g=1|F(l)>q) 
&=      \Big( (1-q)(1-\gamma_0) + P \big( F_0(l_1)>q \big)  \gamma_0  \Big) * \frac{1-\gamma_0}{1-q} 
% \\
&\geq   \Big( (1-q)(1-\gamma_0) + \frac{z^2}{1 + z^2} * \gamma_0 \Big) * \frac{1-\gamma_0}{1-q},
% \\
% = (1-\gamma_0)^2 + \gamma_0 * \frac{1-\gamma_0}{1-q} *  \frac{z^2}{1 + z^2},
% \label{eq:detection_precision_1}
\end{alignat*}
yielding the final bound $P(g=1|F(l)>q) \geq (1-\gamma_0)^2 + \gamma_0 * \frac{1-\gamma_0}{1-q} *  \frac{z^2}{1 + z^2}$ as in \Cref{eq:rank_estimator_lower_bound_app}.
\end{proof}

\subsection{Proof for Theorem \ref{thm:standardized_likelihood_guanrantee_app}}

\begin{proof}
For $F_0(l_1)$, recall $F_0$ is the \gls{CDF} of $l_0=L(\tilde{y}_0, f_y(\rvx_0))$ where $(\tilde{y}_0, \rvx_0) \sim P_0$ and  $l_1=L(\tilde{y}_1, f_y(\rvx_1))$ is the random variable of minority-group loss with  $(\tilde{y}_1, \rvx_1) \sim P_1$.

To derive lower bound for $z=\frac{E(F_0(l_1))-q}{Var(F_0(l_1))}$, first derive bounds on $E(F_0(l_1))$ and $Var(F_0(l_1))$:

\underline{Lower bound for $E(F_0(l_1))$}

Recall $P(F(l)|g=1) = P(F(l_1))$, where $l_1=L(\tilde{y}_1, f_y(\rvx_1))$ is the random variable for minority-group error with $(\tilde{y}_1, f_y(\rvx_1)) \sim P_1$. Then:
\begin{align*}
    E(F_0(l_1))  = E(F_0(l) | g = 1) = P(l_0 \leq l_1) = P(l_1 - l_0 \geq 0).
\end{align*}
By the second moment method inequality \citep{lyons2017probability}, we have:
\begin{align}
P(l_1 - l_0 \geq 0) 
&\geq \frac{E[l_1 - l_0]^2}{E[(l_1 - l_0)^2]} 
= \frac{E[l_1 - l_0]^2}{Var(l_1 - l_0) + E[l_1 - l_0]^2}
\nonumber\\
&\geq \frac{E[l_1 - l_0]^2}{Var(l_1) + Var(l_0) + E[l_1 - l_0]^2}
\nonumber\\
&= \frac{d^2}{(\sigma_0^2 + \sigma_1^2) + d^2}.
\label{eq:mean_loss_diff_bound}
\end{align}

\underline{Upper bound for $Var(F_0(l_1))$}

Recall that $Var(F(l))=E\Big[(F(l)-E(F(l)))^2\Big]$. Using the iterative expectation formula, we split the variance computation for $F_0(l_1)$ into two regions of $l_1$ depending on whether the minority-group loss of $l_1 \geq \mu_1 - \lambda \sigma_1$: 
\begin{align*}
    Var(F_0(l_1)) 
    = 
    & Var(F_0(l_1) | l_1 \leq \mu_1 - \lambda \sigma_1)
    P(l_1 \leq \mu_1 - \lambda \sigma_1)
    + 
    \nonumber  \\
    & Var(F_0(l_1) | l_1 > \mu_1 - \lambda \sigma_1)
    P(l_1 > \mu_1 - \lambda \sigma_1),
    %\label{eq:var_F0_iterated_expectation}
\end{align*}
which holds for any positive multiplier $\lambda > 0$. 

Notice that in the above,  $P(l_1 < \mu_1 - \lambda \sigma_1)$ in the second line describes the tail probability of the loss distribution of $l_1$, for suitably large $\lambda$, $P(l_1 < \mu_1 - \lambda \sigma_1)$ should be small. On the other hand, $Var(F_0(l_1) | l_1 \geq \mu_1 - \lambda \sigma_1)$ in the second line describes the variance of $F_0(l_1)$ in the region where $l_1$ is large. When the distribution of $l_0$ and $l_1$ is well separated (i.e., $\mu_1-\mu_0 = d > 0$), for suitable value of $\lambda$, we expect the value of $F_0(l_1=F_0( \mu_1 - \lambda \sigma_1))$ to be high and close to 1, and as a result the $Var(F_0(l_1)|l_1 \geq \mu_1 - \lambda \sigma_1)$ will be low since $F_0(l_1)$ is bounded within a small range $[F_0( \mu_1 - \lambda \sigma_1), 1]$. Consequently, to obtain a tight upper bound of $Var(F(l))$, it is sufficient to identify a suitable value of $\lambda$ such that both $Var(F_0(l_1) | l_1 \geq \mu_1 - \lambda \sigma_1)$ and $P(l_1 < \mu_1 - \lambda \sigma_1)$ are low.

To identify a suitable value of $\lambda$, first derive an upper bound of $Var(F_0(l_1))$ in terms of $\lambda$. Notice below two facts:
\begin{itemize}
\item By Cantelli's inequality:
$$P(l_1 \leq \mu_1 - \lambda \sigma_1) \leq \frac{1}{\lambda^2 + 1}.$$ 
\item By the inequality for variance of the bounded variables:
$$Var(F_0(l_1)|l_1 \leq \mu_1 - \lambda \sigma_1) \leq \frac{1}{4} F_0(\mu_1 - \lambda \sigma_1)^2,$$
where the first inequality follows by the fact that for a random variable $R$ bounded between $[a, b]$ (in this case between $[F(\mu_1 - \lambda \sigma_1), 1]$), its variance is bounded by $Var(R) \leq (b-E(R))(E(R)-a) \leq \frac{1}{4}(b-a)^2$.

\item By Markov's inequality, $F_0(l_1) = P(l_1 \leq l_1) \geq \mu_0/l_1$, which implies:
$$Var(F_0(l_1)|l_1 \geq \mu_1 - \lambda \sigma_1) 
\leq 
\frac{1}{4} (1-F_0(\mu_1 - \lambda \sigma_1))^2
\leq 
\frac{1}{4} (1-\frac{\mu_0}{\mu_1 - \lambda \sigma_1})^2,$$
where the first inequality also follows by the variance inequality of the bounded variables.
\end{itemize}
Using the above two facts, we can bound $Var(F_0(l_1))$ as:

\begin{align}
Var(F_0(l_1)) 
&= 
 Var(F_0(l_1) | l_1 \leq \mu_1 - \lambda \sigma_1) * 
P(l_1 \leq \mu_1 - \lambda \sigma_1) + 
 Var(F_0(l_1) | l_1 > \mu_1 - \lambda \sigma_1) * 
P(l_1 \geq \mu_1 - \lambda \sigma_1) 
\nonumber\\
&\leq 
Var(F_0(l_1) | l_1 \leq \mu_1 - \lambda \sigma_1) * 
\frac{1}{\lambda^2 + 1} + 
Var(F_0(l_1) | l_1 > \mu_1 - \lambda \sigma_1) * 
\frac{\lambda^2}{\lambda^2 + 1} 
\nonumber\\
&\leq 
\frac{1}{4} F_0(\mu_1 - \lambda \sigma_1)^2 * 
\frac{1}{\lambda^2 + 1} + 
\frac{1}{4} (1-\frac{\mu_0}{\mu_1 - \lambda \sigma_1})^2 * 
\frac{\lambda^2}{\lambda^2 + 1}.
\label{eq:var_F0_iterated_expectation}
\end{align}
where the first inequality holds since the first conditional variance term $Var(F_0(l_1) | l_1 \leq \mu_1 - \lambda \sigma_1)$ (i.e., variance in the majority bulk) is expected to be much larger than the second term $Var(F_0(l_1) | l_1 > \mu_1 - \lambda \sigma_1)$ (i.e., variance in the far tail), therefore assigning the highest possible probability weight $P(l_1 \leq \mu_1 - \lambda \sigma_1)$ to the larger variance term $Var(F_0(l_1) | l_1 \leq \mu_1 - \lambda \sigma_1)$ leads to an upper bound for $Var(F_0(l_1))$.

Further simplifying \Cref{eq:var_F0_iterated_expectation}, we arrive at:
\begin{align*}
Var(F_0(l_1)) 
&\leq 
\frac{1}{4} F_0(\mu_1 - \lambda \sigma_1)^2 * 
\frac{1}{\lambda^2 + 1} + 
\frac{1}{4} (1-\frac{\mu_0}{\mu_1 - \lambda \sigma_1})^2 * 
\frac{\lambda^2}{\lambda^2 + 1}\\
&= \frac{1}{4} * \frac{1}{\lambda^2 + 1} * 
\Big(
F_0(\mu_1 - \lambda \sigma_1)^2 + 
\frac{\lambda^2}{4} (1-\frac{\mu_0}{\mu_1 - \lambda \sigma_1})^2 
\Big) \\
&= \frac{1}{4} * \frac{1}{\lambda^2 + 1} * 
\Big(
F_0(\mu_1 - \lambda \sigma_1)^2 + 
\frac{\lambda^2}{4} (\frac{d - \lambda \sigma_1}{\mu_1 - \lambda \sigma_1})^2 
\Big)
\end{align*}
where recall $d=\mu_1 - \mu_0$ is the expected error gap between the majority and the minority groups. Setting $\lambda = \frac{d}{\sigma_1}$, we have:
\begin{align}
Var(F_0(l_1)) 
&\leq 
\frac{1}{4} * F_0(\mu_0)^2 * \frac{1}{\lambda^2 + 1}
=
\frac{F_0(\mu_0)^2}{4} * \frac{\sigma_1^2}{d^2 + \sigma_1^2}.
\label{eq:var_loss_diff_bound}
\end{align}

\underline{Lower bound for $z$}

Finally, plugging the bounds for $E(F_0(l_1))$ and $Var(F_0(l_1))$ from \Cref{eq:mean_loss_diff_bound} and \ref{eq:var_loss_diff_bound} into $z=\frac{E[F_0(l_1)] - q}{\sqrt{Var[F_0(l_1)]}}$ yields the final lower bound in \Cref{eq:standardized_likelihood_lower_bound_app}, i.e.,
\begin{align*}
z=\frac{E[F_0(l_1)] - q}{\sqrt{Var[F_0(l_1)]}} 
&\geq 
(\frac{d^2}{(\sigma_1^2 + \sigma_2^2) + d^2} - q) \Big/
\sqrt{\frac{F_0(\mu_0)^2}{4} * \frac{\sigma_1^2}{d^2 + \sigma_1^2}}
\\
&=
\frac{2}{F_0(\mu_0)}
* \sqrt{\frac{\sigma_1^2 + d^2}{\sigma_1^2}} * (\frac{d^2}{(\sigma_1^2 + \sigma_2^2) + d^2} - q).
\end{align*}


\end{proof}

==> proof/lemma_1.tex <==
\begin{lemma}[Optimal Group-size Allocation for Weighted Population Risk]
For an objective function that is the weighted combination of group-specific risk:
$$R_w(\alpha, n)= \sum_{g \in \gG} w_g * R(f_{D_{\alpha,n}}|G=g)$$
where $w=\{w_g\}_{g\in \gG}$ are non-negative weights. 
Furthermore, under Assumption \ref{def:group_scaling_law}, $R_w(\alpha, n)$ is approximated by the weighted sum of approximated group risks $\hat{R}(\alpha, n|G=g)=r(\alpha_g n, n | c_g, \tau_g, \delta_g, p_g, q_g)$:
\begin{align}
\hat{R}_w(\alpha, n)
\coloneqq
\sum_{g \in \gG} w_g * \hat{R}(\alpha, n|G=g)
= \sum_{g \in \gG} w_g * 
\big( c_g * (\alpha_g  n)^{-p_g} + \tau_g * n^{-q_g} + \delta_g \big).
\label{eq:approx_weighted_risk}
\end{align}
Then, 
\begin{itemize}[leftmargin=0.5cm]
\item [(1)] When $p_g = p$ is equal for all groups, the optimal allocation $\alpha^*$ that
minimizes the approximated weighted risk (\ref{eq:approx_weighted_risk}) is:
\begin{align}
\alpha^*_g = 
\frac{(w_g c_g)^{1/(p+1)} }
{\sum_{g\in \gG}(w_g c_g)^{1/(p+1)}}.
\label{eq:simple_allocation_weighted_risk}
\end{align}

\item [(2)] When $p_g$ is allowed to differ by group, the optimal allocation $\alpha^*$ that
minimizes the approximated weighted risk (\ref{eq:approx_weighted_risk}) is:
\begin{align}
\alpha^*_g = 
\frac{(w_g c_g p_g n^{-p_g})^{1/(p_g+1)} }
{\sum_{g\in \gG}(w_g c_g p_g n^{-p_g})^{1/(p_g+1)}}.
\label{eq:general_allocation_weighted_risk}
\end{align}
That is, as $n \rightarrow \infty$, the sample size allocation disproportionally lean towards the group that has the slowest learning rate on the exponential scale (i.e., the group with the smallest $p_g$).
\end{itemize}
\label{thm:allocation_weighted_risk}
\end{lemma}


==> proof/lemma_1_proof.tex <==
\begin{proof} The proof is a generalization of Proposition 2 of \citep{rolf2021representation}), where the exponential scaling coefficient $p_g$ is allowed to vary by group, and the weights  $\{w_g\}_{g\in \gG}$ are no longer required to sum to 1. Specifically, note that in (\ref{eq:approx_weighted_risk}), the terms $\tau_g * n^{-q_g} + \delta_g$ does not depend on $\alpha$. Then, restricting $\alpha \in (0, 1)^{|\gG|}$, the optimization problem can be expressed as:
\begin{align*}
\mbox{minimize}_{\alpha} \quad & \sum_{g \in \gG} w_g c_g  (\alpha_g n)^{-p_g}
\\
\mbox{subject to} \quad & \sum_{g \in \gG} \alpha_g = 1.
\end{align*}
Notice that the main objective function is convex in $\alpha=[\alpha_1, \dots, \alpha_{|\gG|}]$. Then, the \gls{KKT} conditions of this constrained optimization problem is:
\begin{align*}
    w_g c_g p_g n^{-p_g} (\alpha_g)^{-(p_g+1)}  &= \lambda 
    \qquad g \in \gG \\
    \sum_{g \in \gG} \alpha_g &= 1.
\end{align*}
Solving the first condition leads to $\alpha_g^* \propto (w_g c_g p_g n^{-p_g})^{1/(p_g+1)}$. This, combined with the second condition, implies that the final solution is of the form (\ref{eq:general_allocation_weighted_risk}):
\begin{align*}
    \alpha^*_g &= \frac{(w_g c_g p_g n^{-p_g})^{1/(p_g+1)} }
    {\sum_{g \in \gG} (w_g c_g p_g n^{-p_g})^{1/(p_g+1)} }.
\end{align*}
Finally,  when $p_g = p$, (\ref{eq:simple_allocation_weighted_risk}) can be derived from (\ref{eq:general_allocation_weighted_risk}) by setting $p_g=p$ and eliminate the multiplicative factor $p_g n^{-p_g}=p n^{-p}$ that is shared by every term in the numerator and the denominator.
\end{proof}


==> proof/lemma_2.tex <==
\begin{lemma}[Optimal Group-size Allocation for Worst-case Risk]
For an objective function that is the adversarially-weighted, worst-case risk:
$$R_v(\alpha, n)= \sup_v \sum_{g \in \gG} v_g * R(f_{D_{\alpha,n}}|G=g)$$
where $v=\{v_g\}_{g\in \gG}$ are non-negative weights for group-specific risks that sum to 1. 
Furthermore, under Assumption \ref{def:group_scaling_law}, $R_v(\alpha, n)$ is approximated by the adversarial weighting the the approximated group risks $\hat{R}(\alpha, n|G=g)=r(\alpha_g n, n | c_g, \tau_g, \delta_g, p_g, v_g)$:
\begin{align}
\hat{R}_v(\alpha, n)
\coloneqq
\sup_v \sum_{g \in \gG} v_g * \hat{R}(\alpha, n|G=g)
= \sup_v \sum_{g \in \gG} v_g * 
\big( c_g * (\alpha_g  n)^{-p_g} + \tau_g * n^{-q_g} + \delta_g \big).
\label{eq:approx_worst_risk}
\end{align}
Then, 
\begin{enumerate}[leftmargin=0.5cm]
\item [(1)] When the group-specific risk share the same $p_g=p, q_g=q, \tau_g=\tau, \delta_g=\delta$ across all groups (i.e., the group-specific risks $c_g n_g^{-p} + \tau n^{-q} + \delta$ differ only by the multiplicative scaling coefficient $c_g$), the optimal allocation to minimize the approximated adversarial risk (\ref{eq:approx_worst_risk}) is:
\begin{align}
\alpha^*_g = 
\frac{c_g^{1/p} }
{\sum_{g\in \gG} c_g^{1/p}}; 
% \quad 
% v^*_g=\frac{c_g^{1/p}}{\sum_{g\in \gG} c_g^{1/p}}.
\label{eq:simple_allocation_worst_risk}
\end{align}
% {\color{red} TODO: need to correct: $v_g^*$ solution is not unique when $\alpha=\alpha^*$.}
\item [(2)] When $p_g=p$ are shared by all groups (i.e., the group-specific risks $c_g n_g^{-p} + \tau_g * n^{-q_g} + \delta_g$ share the exponential scaling coefficient $p$), the optimal allocation to minimize the approximated adversarial risk is:
\begin{align}
\alpha^*_g = 
\frac{(c_g l_g)^{1/p} }
{\sum_{g\in \gG} (c_g l_g)^{1/p}}; 
% \quad 
% v^*_g=\frac{c_g^{1/p} \, l_g^{(p+1)/p}}{\sum_{g\in \gG} c_g^{1/p} \, l_g^{(p+1)/p}},
\label{eq:full_allocation_worst_risk}
\end{align}
where $l_g = (\lambda - (\tau_g n^{-q_g} + \delta_g))^{-1}$ is a group-specific non-negative coefficient, in which $\lambda$ is a positive constant that solves the implicit equation $\sum_g (c_g l_g^{p+1})^{1/p} = \Big[ n * \sum_g (c_g l_g)^{1/p} \Big]^{(p+1)/2}$.
\end{enumerate}
\label{thm:allocation_worst_risk}
\end{lemma}


==> proof/lemma_2_proof.tex <==
\begin{proof}
Minimizing the approximated worst-group risk (\ref{eq:approx_worst_risk}) is equivalent to solving a minimax problem. Specifically, first write the object function as $$H(\alpha, v) \coloneqq \sum_{g \in \gG} v_g * r(\alpha_g n, n | c_g, \tau_g, \delta_g, p_g, v_g).$$ 
As shown, $H(\alpha, v)$ is a function of both the risk allocation parameter $v$ and the group-size allocation $\alpha$, note that $\hat{R}_v(\alpha, n) = \sup_v H(\alpha, v)$. Also recall that $\alpha \in (0, 1)^{|\gG|}$ and $v_g > 0 \; \forall g$. Then, the optimal value of (\ref{eq:approx_worst_risk}) can be written as:
\begin{align}
    \inf_\alpha \; \hat{R}_v(\alpha, n) = \inf_{\alpha} \sup_v \; H(\alpha, v).
    \label{eq:worst_risk_primal}
\end{align}
Notice that (\ref{eq:worst_risk_primal}) is of a min-max form, this motivates us to derive the dual formulation of the problem, which is often easier to solve. Specifically, notice that the objective function $H(\alpha, v)$ is a convex-concave function which is concave (i.e., linear) in $v$ and convex in $\alpha$ (since $\nabla^2_\alpha H(\alpha, v) =diag_g \big[ p_g (p_g+1) v_g c_g n_g^{-p_g} \alpha_g^{-(p_g+2)} \big] \succeq 0$ is a positive-definite $|\gG| \times |\gG|$ matrix for every $v$). Then, by the max-min equality of the convex-concave function (see, e.g., Exercise 5.25 of \citet{boyd2004convex}, or the Proof of the Proposition 1 of \citet{sagawa2019distributionally}), we have:
\begin{align}
    \inf_{\alpha} \sup_v \; H(\alpha, v) = \sup_v \inf_{\alpha} \; H(\alpha, v),
    \label{eq:worst_risk_dual}
\end{align}
which implies that there exists a saddle point $(\alpha^*, v^*)$ such that $\inf_\alpha \; H(\alpha, v^*) = H(\alpha^*, v^*) = \sup_v \; H(\alpha^*, v)$.

We can now solve (\ref{eq:worst_risk_primal}) by solving the dual problem  (\ref{eq:worst_risk_dual}), i.e., $\sup_v \inf_{\alpha} \; H(\alpha, v)$. First solve the inner problem $\inf_{\alpha} \; H(\alpha, v)$, i.e.,
\begin{align*}
\mbox{minimize}_{\alpha} \quad &  
H(\alpha, v) =\sum_{g \in \gG} v_g c_g  (\alpha_g n)^{-p_g}
\\
\mbox{subject to} \quad & \sum_{g \in \gG} \alpha_g = 1; \quad \alpha_g > 0 \; \forall g \in \gG
\end{align*}
This is equivalent to minimizing a weighted population risk with weights $v=\{v_g\}_{g \in \gG}$. Under the setting $p_g=p$ is equal for all groups, by \Cref{thm:allocation_weighted_risk}, we have that the optimal solution is:
\begin{align}
\alpha^*_g = 
\frac{(v_g c_g)^{1/(p+1)} } {\sum_{g\in \gG}(v_g c_g)^{1/(p+1)}}.
\label{eq:lemma2_inner_problem_sol}
\end{align}

To obtain a concrete expression of $\alpha^*_g$ (i.e., not in terms of the group allocation $v_g$), we need to solve for the for the outer problem $\sup_v H(\alpha^*, v)$ in order to obtain an expression for the group allocation $v^*$. Specifically, under the expression of $\alpha^*$, the optimal risk $\inf_\alpha H(\alpha, v)=H(\alpha^*, v)$ takes the form:
\begin{align}
\nonumber
H(\alpha^*, v) &= 
\sum_{g\in \gG} v_g \Big[  
c_g \big(
\frac{(v_g c_g)^{1/(p+1)}}{\sum_g (v_g c_g)^{1/(p+1)}} n
\big)^{-p} 
+ \tau_g n^{-q_g} + \delta_g
\Big]\\ 
\nonumber
&=
\sum_{g\in \gG} v_g \Big[  
c_g \big(
\frac{(v_g c_g)^{1/(p+1)}}{\sum_g (v_g c_g)^{1/(p+1)}} n
\big)^{-p} 
\Big]
+ 
\sum_{g\in \gG} v_g \Big[  
\tau_g n^{-q_g} + \delta_g
\Big]\\ 
\nonumber
&=
\big[ 
n^{-1} 
\sum_{g\in \gG} (v_g c_g)^{1/(p+1)}
\big]^p
\big[ 
\sum_{g\in \gG} 
(v_g c_g)^{1/(p+1)}
\big]
+ 
\sum_{g\in \gG} v_g \Big[  
\tau_g n^{-q_g} + \delta_g
\Big]\\
&=
n^{-p} 
\Big[ 
\sum_{g\in \gG} (v_g c_g)^{1/(p+1)}
\Big]^{(p+1)}
+ 
\sum_{g\in \gG} v_g \Big[  
\tau_g n^{-q_g} + \delta_g
\Big].
\label{eq:lemma2_outer_problem}
\end{align}
Then, solving for $\inf_v H(\alpha^*, v)$ subject to $\sum_g v_g = 1$ yields the \gls{KKT} conditions:
\begin{align}
n^{-p} \Big[ \sum_{g\in \gG} (v_g c_g)^{1/(p+1)} \Big]^p * c_g^{1/(p+1)}  * v_g^{-p/(p+1)} + (\tau_g n^{-q_g} + \delta_g) = \lambda;
\qquad 
\sum_{g \in \gG} v_g = 1.
\label{eq:lemma2_outer_problem_kkt}
\end{align}
\todo{\color{red} TODO: cover the case $v$ on the edge of the simplex so that $v_g=0$.}

Now denote $l_g = (\lambda - (\tau_g n^{-q_g} + \delta_g))^{-1}$, a simple rearrangement of terms in (\ref{eq:lemma2_outer_problem_kkt}) reveals that:
\begin{align}
\nonumber
v_g 
&= 
\Big[ n^{-1} \sum_{g\in \gG} (v_g c_g)^{1/(p+1)} \Big]^{p+1} *
\Big[ \frac{c_g^{1/p}}{(\lambda - (\tau_g n^{-q_g} + \delta_g))^{(p+1)/p}} \Big] 
\\
&= 
\Big[ n^{-1} \sum_{g\in \gG} (v_g c_g)^{1/(p+1)} \Big]^{p+1} *
\Big[ c_g^{1/p} * l_g^{(p+1)/p} \Big]
\label{eq:lemma2_outer_problem_sol}
\\ \nonumber
&\propto 
c_g^{1/p} l_g^{(p+1)/p},
\end{align}
which combined with the condition $\sum_{g \in \gG} v_g = 1$ implies $v^*_g = \frac{c_g^{1/p} l_g^{(p+1)/p}}{\sum_{g\in \gG c_g^{1/p} l_g^{(p+1)/p}}}$. 

Now, since (\ref{eq:lemma2_inner_problem_sol})-(\ref{eq:lemma2_outer_problem_sol}) are derived under the condition $p_g=p \; \forall g$, we are ready to obtain the expression of $\alpha^*$ for the second part of \Cref{thm:allocation_worst_risk} (i.e., \Cref{eq:full_allocation_worst_risk}). Specifically, obtain the expression for $\alpha^*$ by plugging the expression of $v^*_g$ into (\ref{eq:lemma2_inner_problem_sol}):
\begin{align}
\alpha^*_g 
= 
\frac{(v_g c_g)^{1/(p+1)} } {\sum_{g\in \gG}(v_g c_g)^{1/(p+1)}}
=
\frac{(c_g l_g)^{1/p} } {\sum_{g\in \gG}(c_g l_g)^{1/p}}.
\label{eq:full_allocation_worst_risk_proof}
\end{align}
Furthermore, (\ref{eq:lemma2_outer_problem_sol}) combined with $\sum_g v_g = 1$ and the expression $v^*_g = \frac{c_g^{1/p} l_g^{(p+1)/p}}{\sum_{g\in \gG} c_g^{1/p} l_g^{(p+1)/p}}$ implies that
\begin{align*}
\sum_{g \in \gG} c_g^{1/p} l_g^{(p+1)/p} 
= \Big[ n^{-1} \sum_{g\in \gG} (v_g c_g)^{1/(p+1)} \Big]^{-(p+1)} 
= \Big[n * \sum_{g\in \gG} (v_g c_g)^{1/(p+1)} \Big]^{p+1} 
= \frac{1}{\sum_{g\in \gG} c_g^{1/p} l_g^{(p+1)/p}} * 
\Big[ n \sum_{g \in \gG}
(c_g l_g)^{1/p}
\Big]^{p+1},
\end{align*}
which implies:
\begin{align*}
\sum_{g \in \gG} (c_g l_g^{(p+1)})^{1/p} &= \Big[ n \sum_{g \in \gG}
(c_g l_g)^{1/p}
\Big]^{(p+1)/2}.
\end{align*}

Finally, we derive the first part of \Cref{thm:allocation_worst_risk}, which is a special case. Notice that under the condition that $(p_g=p, q_g=q, \tau_g=\tau, \delta_g=\delta)$ is the same across groups, $l_g = (\lambda - (\tau_g n^{-q_g} + \delta_g))^{-1}$ are also the same across all groups, and can be cancelled out from the nominator and the denominator of (\ref{eq:full_allocation_worst_risk_proof}), which leads to the expressions in (\ref{eq:simple_allocation_worst_risk}), i.e., $\alpha^*_g = \frac{(c_g)^{1/p} } {\sum_{g\in \gG}(c_g)^{1/p}}$ and $v^*_g = \frac{(c_g)^{1/p} } {\sum_{g\in \gG}(c_g)^{1/p}}$.
\end{proof}


==> proof/prop_app_1.tex <==
\begin{proposition}[Optimal Allocation for the Accuracy-Fairness Frontier]

Given a data distribution $\gD$ with prevalence of each group as $\{\gamma_g\}_{g \in \gG}$. Recall $D_{\alpha, n}$ is a size-$n$ dataset with group size allocation $\alpha=\{\alpha_g\}_{g \in \gG}$, $\hat{f}_{D_{\alpha, n}}$ is a model trained on $D_{\alpha, n}$. Finally, denote the population-level risk of $\hat{f}_{D_{\alpha, n}}$ when evaluated on $\gD$ as: 
$$R(\alpha, n) = \sum_{g\in \gG} \gamma_g E[R(\hat{f}_{D_{\alpha, n}} | G=g)].$$
where the expectation is over the randomness in $g \in \gG$. Recall that the accuracy-fairness frontier risk can be expressed as:
$$F_{\omega}(\alpha, n) \coloneqq 
\omega * R(\alpha, n) + \omega_2 * (\alpha, n),$$


\begin{comment}
where $\omega =[\omega_1, \omega_2] > \mathbf{0}$ are finite positive constants. $R_{fair}$ is a \textit{``fairness" risk} which can be the average-group risk 
$$\bar{R}(\alpha, n) \coloneqq \frac{1}{|\gG|} \sum_{g\in \gG} R(f_{D_{\alpha, n}}|G=g)$$ or the worst-case risk 
$$\tilde{R}(\alpha, n) \coloneqq \sup_v \sum_{g\in \gG} [ v_g R(f_{D_{\alpha, n}}|G=g)].$$ 
Assuming the group-specific generalization-error scaling laws (Definition \ref{def:group_scaling_law}) share the same exponential scaling coefficient $p_g=p$, we have:
\begin{itemize}[leftmargin=0.5cm]
\item [(1)] \textbf{(Average-group Risk)} Let $R_{fair}$ be the average-group risk $\bar{R}(\alpha, n)$. Also denote the approximated average-case risk as
$\hat{\bar{R}}(\alpha, n) = \frac{1}{|\gG|} \sum_{g\in \gG} \hat{R}(\alpha, n|G=g)$.
Then, to minimizes the approximated accuracy-fairness frontier under the average-group risk
\begin{align}
\hat{F}_{\omega}(\alpha, n)=\omega_1 \hat{R}(\alpha, n) + \omega_2 \hat{\bar{R}}(\alpha, n),
\label{eq:approx_average_group_frontier}
\end{align}
the optimal training-set group allocation $\alpha$ is:
\begin{align*}
\alpha^*_g = 
\frac{[\omega_1  \gamma_g c_g + \omega_2  \frac{1}{|\gG|} c_g]^{1/(p+1)}}
{\sum_{g\in \gG}
[\omega_1 \gamma_g c_g + \omega_2 \frac{1}{|\gG|} c_g]^{1/(p+1)}
}.
\end{align*}
\item [(2)] \textbf{(Worst-case Risk)} Let $R_{fair}$ be the worst-case risk 
$\tilde{R}(\alpha, n)$, where $\sum_g v_g = 1$ and $v_g > 0 \; \forall g \in \gG$. 
Also denote the approximated worst-case risk $\hat{\tilde{R}}(\alpha, n) \coloneqq \sup_v \sum_{g\in \gG} [ v_g \hat{R}(\alpha, n|G=g)]$.
Then, to minimizes the approximated accuracy-fairness frontier under the worst-case risk
\begin{align}
\hat{F}_{\omega}(\alpha, n)=\omega_1 \hat{R}(\alpha, n) + \omega_2 \hat{\tilde{R}}(\alpha, n).
\label{eq:approx_worst_case_frontier}
\end{align}
The optimal training-set group allocation $\alpha$ should satisfy:
\begin{align*}
\alpha^*_g = \frac{(r_g c_g)^{1/(p+1)}}{\sum_{g\in \gG} (r_g c_g)^{1/(p+1)}}, 
\quad \mbox{where} \quad
r_g = \max\Big[
\gamma_g, \;\;
\Big(\frac{\omega_2 + \omega_1\sum_{g \in \gB} \gamma_{g}}
{\omega_1} \Big)\Big( \frac{c_g^{1/p} l_{g,\omega}^{(p+1)/p}}{\sum_{g \in \gB} c_g^{1/p} l_{g,\omega}^{(p+1)/p}}\Big) \Big].
\end{align*}
Here, $l_{g,\omega}=(\lambda - \omega_2(\tau_g n^{-q_g} + \delta_g)))^{-1}$, where $\lambda$ is a large positive constant that solves $\sum_{g \in \gG} 
\max\Big(
0, \;
\omega_2^{1/p}
\big[ n^{-1} \sum_{g\in \gG} (\eta_g c_g)^{1/(p+1)} \big]^{p+1}
 \, c_g^{1/p} l_{g,\omega}^{(p+1)/p}
- 
\frac{\omega_1}{\omega_2}
\gamma_g
\Big)=1$. Finally, $\gB \subseteq \gG$ is the set of under-represented groups that needs to be upsampled in the training data to minimize the accuracy-fairness frontier $F_\omega$. Specifically, for every $g \in \gB$, its population prevalence $\gamma_g$ is bounded by 
\begin{align}
\gamma_g < ( \frac{\omega_2}{\omega_1} + \sum_{g \in \gB} \gamma_g) * 
\frac{c_g^{1/p} l_{g,\omega}^{(p+1)/p}}{\sum_{g \in \gB} c_g^{1/p} l_{g,\omega}^{(p+1)/p}}.
\label{eq:minority_group_criteria}
\end{align}
\end{itemize}
\end{comment}

\label{thm:optimal_allocation_frontier_full}
\end{proposition}



==> proof/prop_app_1_proof.tex <==
\begin{proof} First prove (1) (\textbf{Averge-group Risk}). 

First notice that the empirical population risk can be expressed as $\hat{R}(\alpha, n)=\sum_g \gamma_g \hat{R}(\alpha, n | G=g)$, where $\gamma_g=E_{\gD}(G=g)$ is the population prevalence of each group under the empirical distribution. Then, the fairness-accuracy frontier under the approximated average-group risk (\ref{eq:approx_average_group_frontier}) can be expressed as a weighted sum of group-specific risks:
\begin{align*}
\hat{\bar{R}}(\alpha, n) = \sum_{g\in \gG} w_g \hat{R}(\alpha, n|G=g)   
\quad \mbox{where} \quad 
w_g = \omega_1 \gamma_g + \omega_2 \frac{1}{|\gG|}.
\end{align*}
Then, by \Cref{thm:allocation_weighted_risk}, the optimal training-set allocation $\alpha^*$ that minimizes the approximated average-group risk is:
\begin{align*}
\alpha^*_g = 
\frac{(w_g c_g)^{1/(p+1)} }
{\sum_{g\in \gG}(w_g c_g)^{1/(p+1)}}
\quad \mbox{where} \quad 
w_g = \omega_1 \gamma_g + \omega_2 \frac{1}{|\gG|},
\end{align*}
which concludes the proof.



Now prove (2) (\textbf{Worst-case Risk}). 

Notice that the fairness-accuracy frontier under the approximated worst-case risk (\ref{eq:approx_worst_case_frontier}) can be expressed as the adversarial weighting of group-specific risks $\hat{R}(\alpha, n|G=g)$ under a simplex constraint:
\begin{align*}
\hat{\tilde{R}}(\alpha, n) = \sup_v \sum_{g\in \gG} (\omega_1 \gamma_g + \omega_2 v_g ) * \hat{R}(\alpha, n|G=g)   
\quad \mbox{where} \quad 
v \geq \mathbf{0}, \; \sum_g v_g = 0 \; \forall g.
\end{align*}
Consequently, analogous to \Cref{thm:allocation_worst_risk}, finding the optimal allocation $\alpha$ for $\hat{\tilde{R}}(\alpha, n)$ is equivalent to solving a minimax problem $\inf_{\alpha} \sup_v H(\alpha, v)$ with respect to the objective function 
$$H(\alpha, v) = (\omega_1 \gamma_g + \omega_2 v_g ) * \hat{R}(\alpha, n|G=g).$$
Notice that $H(\alpha, v)$ is a convex-concave function that is convex in $\alpha=[\alpha_1, \dots, \alpha_{|\gG|}]$ (since it is a linear sum of $\hat{R}(\alpha, n|G=g)=c_g * (\alpha_g  n)^{-p} + \tau_g * n^{-q_g} + \delta_g$ which is a convex function of $\alpha_g$ for every $g$) and concave (linear) in $v=[v_1, \dots, v_{|\gG|}]$. By the max-min equality of the convex-concave function (see, e.g., Exercise 5.25 of \citet{boyd2004convex}, or the Proof of the Proposition 1 of \citet{sagawa2019distributionally}), we have:
\begin{align}
    \inf_{\alpha} \sup_v \; H(\alpha, v) = \sup_v \inf_{\alpha} \; H(\alpha, v),
    \label{eq:worst_risk_frontier_dual}
\end{align}
which implies that there exists a saddle point $(\alpha^*, v^*)$ such that $\inf_\alpha \; H(\alpha, v^*) = H(\alpha^*, v^*) = \sup_v \; H(\alpha^*, v)$.

Consequently, we can find $\alpha^*$ by solving the dual problem on the right-hand side of (\ref{eq:worst_risk_frontier_dual}). First solve the inner problem $\inf_{\alpha} H(\alpha, v)$, which is equivalent to solving:
\begin{align*}
\mbox{minimize}_{\alpha} \quad &  
H(\alpha, v) =\sum_{g \in \gG} (\omega_1 \gamma_g + \omega_2 v_g ) c_g  (\alpha_g n)^{-p} + const.
\\
\mbox{subject to} \quad & \sum_{g \in \gG} \alpha_g = 1; \quad \alpha_g > 0 \; \forall g \in \gG
\end{align*}
where we have ignored the additive constant terms that do not involve $\alpha$. This is equivalent to minimizing a weighted population risk with weights $\eta_g= \omega_1 \gamma_g + \omega_2 v_g$. Under the setting where $p_g=p$ is equal for all groups, by \Cref{thm:allocation_weighted_risk}, the optimal solution of $\alpha$ is:
\begin{align}
\alpha^*_g = 
\frac{(\eta_g c_g)^{1/(p+1)} } {\sum_{g\in \gG}(\eta_g c_g)^{1/(p+1)}},
\quad \mbox{where} \quad
\eta_g= \omega_1 \gamma_g + \omega_2 v_g.
\label{eq:prop_inner_problem_sol}
\end{align}
This allows us to derive the expression for $\inf_\alpha H(\alpha, v)=H(\alpha^*, v)$, i.e.:
\begin{align*}
    H(\alpha^*, v) &= \sum_{g \in \gG} \eta_g \big[ 
    c_g  (\alpha_g^* n)^{-p}  + \tau_g * n^{-q_g} + \delta_g \big] 
    \\
    &= \sum_{g \in \gG} \eta_g \big[ c_g  (\alpha_g^* n)^{-p}  \big] + 
    \sum_{g \in \gG} \eta_g  \big[ \tau_g * n^{-q_g} + \delta_g \big]
    \\
    &= \sum_{g \in \gG} \eta_g \big[ 
    c_g  (\frac{(\eta_g c_g)^{1/(p+1)} } {\sum_{g\in \gG}(\eta_g c_g)^{1/(p+1)}} n)^{-p}  
    \big] + 
    \sum_{g \in \gG} \eta_g  \big[ \tau_g * n^{-q_g} + \delta_g \big]
    \\
    &=  n^{-p} \Big[\sum_{g\in \gG}(\eta_g c_g)^{1/(p+1)} \Big]^{p+1}
     + 
    \sum_{g \in \gG} \eta_g  \big[ \tau_g * n^{-q_g} + \delta_g \big],
\end{align*}
with derivative (recall $\eta_g= \omega_1 \gamma_g + \omega_2 v_g$):
\begin{align}
\nonumber
\frac{\partial}{\partial v_g} 
H(\alpha^*, v)
&= 
n^{-p} *
\frac{\partial}{\partial v} \Big[
\sum_{g\in \gG}(\eta_g c_g)^{1/(p+1)} \Big]^{p+1} + 
\sum_{g \in \gG} \frac{\partial}{\partial v}  \eta_g  \big[ \tau_g * n^{-q_g} + \delta_g \big]
\\
&=
\omega_2 \, n^{-p}
\Big[ \sum_{g\in \gG} (\eta_g c_g)^{1/(p+1)} \Big]^p * c_g^{1/(p+1)} \eta_g^{-p/(p+1)} + 
\omega_2 \, (\tau_g n^{-q_g} + \delta_g)
.
\label{eq:H_deriv}
\end{align}

Now, we are ready to solve the outer problem $\sup_v H(\alpha^*, v)$ of the dual problem in (\ref{eq:worst_risk_frontier_dual}), which is equivalent to solving:
\begin{align*}
\mbox{maximize}_{v} \quad &  
H(\alpha^*, v) = 
\Big[ n^{-1} \sum_{g\in \gG}(\eta_g c_g)^{1/(p+1)} \Big]^p
\Big[ \sum_{g \in \gG} (\eta_g c_g)^{1/(p+1)} \Big] + 
\sum_{g \in \gG} \eta_g  \big[ \tau_g * n^{-q_g} + \delta_g \big]
\\
\mbox{subject to} \quad & \sum_{g \in \gG} v_g = 1; \quad v_g > 0 \; \forall g \in \gG
\end{align*}
where $\eta_g = \omega_1 \gamma_g + \omega_2 v_g$. Solve this constrained optimization problem by writing down its KKT conditions (see, e.g., Chapter 5.5 of \citet{boyd2004convex}) with respect to the Lagrangian form $-H(\alpha^*, v) + \lambda (\sum_g v_g - 1) - u_g \sum_g v_g $, i.e., for every $g$:
\begin{align*}
    \frac{\partial}{\partial v_g} \big[ -H(\alpha^*, v) + \lambda (\sum_g v_g - 1) - u_g \sum_g v_g \big] = 0; 
    \qquad 
    \sum_{g} v_g = 1; \qquad u_g * v_g = 0;
    \qquad 
    u_g \geq 0, \; v_g &\geq 0.
\end{align*}
Simplifying the first derivative equation in the above, we arrive at the full set of KKT condition:
\begin{alignat*}{2}
&-\frac{\partial}{\partial v_g} H(\alpha^*, v) + \lambda - u_g = 0; 
\quad && \mbox{(Stationarity Condition)}
\\ 
&\sum_{g} v_g = 1; \quad v_g \geq 0; && \mbox{(Primal feasibility)}\\
&u_g \geq 0; && \mbox{(Dual Feasibility)}\\
& u_g * v_g = 0.  && \mbox{(Complementary Slackness)}
\end{alignat*}
Rearranging the terms, we get for every $g$:
\begin{align}
u_g &=-\frac{\partial}{\partial v_g} H(\alpha^*, v) + \lambda;
\label{eq:kkt_stat_cond}
\\
& u_g * v_g = 0; \quad u_g \geq 0; \quad  v_g \geq 0.
\label{eq:kkt_comp_slack}
\\ 
&\sum_{g} v_g = 1;
\label{eq:kkt_simplex_cond}
\end{align}
and our goal is to identify $v^*=\{v^*_g\}_{g\in \gG}$ which satisfy all the above conditions.

First notice (\ref{eq:kkt_stat_cond}) implies that $u_g \geq 0$ if and only if:
\begin{alignat*}{2}
0 
&\geq \frac{\partial}{\partial v_g} H(\alpha^*, v) - \lambda 
\stackrel{By (\ref{eq:H_deriv})}{=}
\Big[ \omega_2^{1/p} n^{-1} \sum_{g\in \gG} (\eta_g c_g)^{1/(p+1)} \Big]^p 
* 
c_g^{1/(p+1)} \eta_g^{-p/(p+1)} + 
[ \omega_2 \, (\tau_g n^{-q_g} + \delta_g)-\lambda ]
\end{alignat*}
Denoting $l_{g,\omega}=(\lambda - \omega_2(\tau_g n^{-q_g} + \delta_g)))^{-1}$ and $Z_\omega =\Big[ \omega_2^{1/p} n^{-1} \sum_{g\in \gG} (\eta_g c_g)^{1/(p+1)} \Big]^{p+1} $, then the above is equivalent to stating:
\begin{align*}
\omega_1 \gamma_g + \omega_2 v_g
&= 
\eta_g \geq
Z_\omega \,
c_g^{1/p} l_{g,\omega}^{(p+1)/p}
\quad \mbox{or equivalently,}
\quad
v_g \geq \frac{\omega_1}{\omega_2}
\Big[ 
\frac{1}{\omega_1} 
Z_\omega \,
c_g^{1/p} l_{g,\omega}^{(p+1)/p}
- \gamma_g
\Big],
\end{align*}
if and only if $u_g \geq 0$ (due to (\ref{eq:kkt_stat_cond})). More specifically, this means:
\begin{align}
\mbox{if} \quad u_g > 0, \qquad &
v_g > \frac{\omega_1}{\omega_2}
\big[ 
\frac{1}{\omega_1} 
Z_\omega \,
c_g^{1/p} l_{g,\omega}^{(p+1)/p}
- \gamma_g
\big],
\; \mbox{or equivalently,} \;\; 
\gamma_g > 
\frac{1}{\omega_1} Z_\omega \,
c_g^{1/p} l_{g,\omega}^{(p+1)/p} - 
\frac{\omega_2}{\omega_1} v_g;
\label{eq:kkt_iff_u_pos}
\\
\mbox{if} \quad u_g = 0, \qquad &
v_g = \frac{\omega_1}{\omega_2}
\Big[ 
\frac{1}{\omega_1} 
Z_\omega \,
c_g^{1/p} l_{g,\omega}^{(p+1)/p}
- \gamma_g
\Big].
\label{eq:kkt_iff_u_zero}
\end{align}

Now use (\ref{eq:kkt_iff_u_pos})-(\ref{eq:kkt_iff_u_zero}) to analyze the second condition (\ref{eq:kkt_comp_slack}) (i.e., complementary slackness). Specifically, (\ref{eq:kkt_comp_slack}) states that $v_g = 0$ if $u_g > 0$, and $v_g \geq 0$ if $u_g = 0$. Under (\ref{eq:kkt_iff_u_pos})-(\ref{eq:kkt_iff_u_zero}), this implies
\begin{align*}
v_g = 
\begin{cases}
0 
&  \mbox{if} \quad u_g>0, 
\; \mbox{or equivalently,} \;
\Big[ 
\frac{1}{\omega_1} 
Z_\omega \,
c_g^{1/p} l_{g,\omega}^{(p+1)/p}
- \gamma_g
\Big] < 0
;
\\
\frac{\omega_1}{\omega_2}
\Big[ 
\frac{1}{\omega_1} 
Z_\omega \,
c_g^{1/p} l_{g,\omega}^{(p+1)/p}
- \gamma_g
\Big]
&  \mbox{if} \quad u_g=0.
\end{cases}
\end{align*}
The above can be expressed succinctly as:
\begin{align}
v_g = \max\Big(
0, \;
\frac{\omega_1}{\omega_2}
\big[ 
\frac{1}{\omega_1} 
Z_\omega \, c_g^{1/p} l_{g,\omega}^{(p+1)/p}
- \gamma_g \big]
\Big).
\label{eq:v_g_interm_expr}
\end{align}
As a result, $\eta_g=\omega_1 \gamma_g + \omega_2 v_g$ can be expressed as:
\begin{align}
\eta_g = \max\Big(
\omega_1 \gamma_g, \;
Z_\omega \, c_g^{1/p} l_{g,\omega}^{(p+1)/p}
\Big).
\label{eq:eta_g_interm_expr}
\end{align}

To obtain a more succinct expression of $\eta_g$, now derive an expression of $Z_\omega$ using the the third and final condition (\ref{eq:kkt_simplex_cond}). Notice that in (\ref{eq:v_g_interm_expr}),
$v_g  > 0$ if and only if $\gamma_g <
\frac{1}{\omega_1} Z_\omega \,
c_g^{1/p} l_{g,\omega}^{(p+1)/p}$ (due to (\ref{eq:kkt_iff_u_pos})), which implies that $v_g > 0$ if and only if the empirical prevalence $\gamma_g$ of group $g$ is low. To this end, let $\gB =\Big\{ g \Big| \gamma_g \leq
\frac{1}{\omega_1} Z_\omega \,
c_g^{1/p} l_{g,\omega}^{(p+1)/p} \Big\} \subseteq \gG$ be the indices  of the low-prevalence, under-represented groups, so that $v_g>0$ if and only if $g \in \gB$. Then, (\ref{eq:kkt_simplex_cond}) implies:
\begin{align}
1 = \sum_{g\in \gG} v_g &= \sum_{g \in \gB} v_g
= 
\sum_{g \in \gB}
\frac{\omega_1}{\omega_2}
\big[ 
\frac{1}{\omega_1} 
Z_\omega \, c_g^{1/p} l_{g,\omega}^{(p+1)/p}
- \gamma_g \big], 
\;\; \mbox{or equivalently,} \;\;
Z_{\omega} = 
\frac{\omega_2 + \omega_1 * \sum_{g \in \gB} \gamma_g}
{\sum_{g \in \gB} c_g^{1/p} l_{g,\omega}^{(p+1)/p}}.
\label{eq:Z_omega_expr}
\end{align}

We are now ready to derive the final expressions of $\eta^*_g$ and $\alpha^*$. Specifically, plugging (\ref{eq:Z_omega_expr}) into (\ref{eq:eta_g_interm_expr}), we get:
\begin{align*}
\eta^*_g = \omega_1 * \max\Big[
\gamma_g, \;
\big(
\frac{\omega_2 + \omega_1 * \sum_{g \in \gB} \gamma_g}{\omega_1} 
\big)\big(
\frac{c_g^{1/p} l_{g,\omega}^{(p+1)/p}}{\sum_{g \in \gB} c_g^{1/p} l_{g,\omega}^{(p+1)/p}}
\big)
\Big].
%\label{eq:eta_g_final_expr}
\end{align*}
Then, (\ref{eq:prop_inner_problem_sol}) implies that the optimal allocation $\alpha^*$ is
\begin{align*}
\alpha^*_g = 
\frac{(r_g c_g)^{1/(p+1)} } {\sum_{g\in \gG}(r_g c_g)^{1/(p+1)}},
\quad \mbox{where} \quad
r_g = \frac{\eta^*_g}{\omega_1}=
\max\Big[
\gamma_g, \;
\big(
\frac{\omega_2 + \omega_1 * \sum_{g \in \gB} \gamma_g}{\omega_1} 
\big)\big(
\frac{c_g^{1/p} l_{g,\omega}^{(p+1)/p}}{\sum_{g \in \gB} c_g^{1/p} l_{g,\omega}^{(p+1)/p}}
\big)
\Big].
\end{align*}

Furthermore, the definition of the under-represented groups $\gB \subseteq \gG$ can be expressed as:
\begin{align*}
\gB =
\bigg\{ g
\Big|
\gamma_g \leq 
\big(
\frac{\omega_2 + \omega_1 * \sum_{g \in \gB} \gamma_g}{\omega_1} 
\big)\big(
\frac{c_g^{1/p} l_{g,\omega}^{(p+1)/p}}{\sum_{g \in \gB} c_g^{1/p} l_{g,\omega}^{(p+1)/p}}
\big)
\bigg\}.
\end{align*}
Finally, notice that (\ref{eq:kkt_simplex_cond}) also implies the $\lambda$ in $l_{g,\omega}=(\lambda - \omega_2(\tau_g n^{-q_g} + \delta_g)))^{-1}$ is the solution to 
% (recall $Z_\omega =\Big[ \omega_2^{1/p} n^{-1} \sum_{g\in \gG} (\eta_g c_g)^{1/(p+1)} \Big]^{p+1}$)
:
\begin{align*}
1 
= \sum_{g \in \gG} v_g 
&= 
\sum_{g \in \gG} 
\max\Big(
0, \;
\frac{1}{\omega_2}
Z_\omega \, c_g^{1/p} l_{g,\omega}^{(p+1)/p}
- 
\frac{\omega_1}{\omega_2}
\gamma_g
\Big)
% \\
% &= 
% \sum_{g \in \gG} 
% \max\Big(
% 0, \;
% \omega_2^{1/p}
% \big[ n^{-1} \sum_{g\in \gG} (\eta_g c_g)^{1/(p+1)} \big]^{p+1}
%  \, c_g^{1/p} l_{g,\omega}^{(p+1)/p}
% - 
% \frac{\omega_1}{\omega_2}
% \gamma_g
% \Big)
,
\end{align*}
so that $\exists g$ such that $v_g>0$ and that $\gB$ is non-empty.

% Notice that the similarity between structure of this solution and that of the \textit{water-filling problem} (see, e.g., Example 5.2 of \citet{boyd2004convex}). 
\end{proof}


==> sections/abstract_old_versions.tex <==
\jereliu{original version}
Uncertainty-based active learning (AL) is a promising approach to mitigate dataset bias and improve model fairness. By diversely sampling from the under-represented tail groups, AL is expected to improve the distributional balance in the training data and the so-called \textit{accuracy-fairness frontier} in the trained model. \dvij{I think active learning is broader and goal is data efficient learning more generally. Perhaps we want to discuss fairness aware active learning more specifically?}
However, the quality of uncertainty estimates from modern deep-learning model are typically worse in the presence of spurious correlations and dataset bias,  
so the improvements from AL on tail groups may be limited even though AL can improve overall accuracy. 
In this work, we propose \textit{\gls{ISP}}, a simple approach to improve the uncertainty estimation of a deep neural network under dataset bias. 
ISP adds an auxiliary \textit{introspection} task to model training, asking the model to predict whether an example belongs to an under-represented group.
We show that ISP provably improves the bias-awareness of the model representations and the resulting uncertainty estimates, and can be readily adapted to the setting where group annotation is not available via a cross-validation procedure.
On challenging tabular and language tasks with dataset bias and label noise, ISP consistently improves both the tail-group sampling rate and hence the accuracy-fairness tradeoff frontier of the final model, strongly outperforming the popular alternatives.

\dvij{Alternative abstract}:
Deep learning has been shown to suffer from spurious correlations and systematic bias, particularly when datasets deep networks are trained on are themselves biased. Further, this bias may not be easy to measure when details of the data generation process are not available. In this work, we develop a new technique, \gls{ISP} that learns to estimate per-datapoint bias and uses the learned bias predictions to preferentially sample datapoints in an active learning setting to mitigate the impact of this bias. Unlike prior work, our technique does not require subgroup information. We analyze our approach theoretically and demonstrate that, under standard assumptions used in the fairness literature, our technique correctly estimates dataset bias \dvij{Jeremiah please check or refine this.}. Further, we demonstrate empirically that on datasets with systematic bias, our technique correctly identifies under-represented groups on which the model performance is low and up-samples these in an active learning setting. \dvij{Provide some concrete numbers on empirical improvements}

\balaji{Alternative abstract}:
Uncertainty-based active learning (AL) is a promising approach to mitigate dataset bias and improve model fairness. By diversely sampling from the under-represented tail groups, AL is expected to improve the distributional balance in the training data and improve the so-called \textit{accuracy-fairness frontier} in the trained model. 
A key ingredient for such AL approaches is an accurate estimate of the model bias and uncertainty. However, the quality of uncertainty estimates from modern deep-learning model are typically worse in the presence of spurious correlations, and furthermore, the bias may not be easy to measure when details of the data generation process are not available. Hence, existing approaches do not significantly improve the performance on tail groups, leading to sub-optimal solutions in the accuracy-fairness frontier.   %even though they may improve overall accuracy. 
In this work, we propose \textit{\gls{ISP}}, a simple approach to improve the uncertainty estimation of a deep neural network under dataset bias. ISP adds an auxiliary \textit{introspection} task to model training, asking the model to predict whether an example belongs to an under-represented group.
We show that ISP provably improves the bias-awareness of the model representations and the resulting uncertainty estimates, and can be readily adapted to the setting where group annotation is not available via a cross-validation procedure.
On challenging tabular and language tasks with dataset bias and label noise, we demonstrate that ISP correctly identifies tail groups on which the model performance is low and up-samples these in an active learning setting, thus achieving sate-of-the-art on the accuracy-fairness frontier.


==> sections/app_optimal_allocation.tex <==
\section{Optimal Group-size Allocation: Full Theoretical Results}
{\color{red} Note: Hide from main submission}

Denote $D_{\alpha,n}$ as a dataset with sample size $n$ and group allocation $\alpha=\{\alpha_g\}_{g\in \gG}$, $f_{D_{\alpha,n}}$ is a model trained on $D_{\alpha,n}$, and $R(f|G=g)=E_{D_g}(L(y, f))$ is the group-specific risk for a model $f$. 

\subsection{Key Technical Lemmas}
\label{sec:lemma}

\input{proof/lemma_1}
{\proof See \Cref{sec:allocation_weighted_risk_proof}.}\\

\input{proof/lemma_2}
{\proof See \Cref{sec:allocation_worst_risk_proof}.}\\


\subsection{Key Technical Propositions}
\input{proof/prop_app_1}

{\proof See \Cref{sec:optimal_allocation_frontier_full_proof}.}\\

\subsection{Corollaries}

\begin{corollary_prop}[Sufficient Conditions of the Underrepresented Group $\gB$]
Under the assumption of \ref{thm:optimal_allocation_frontier_full} (i.e., the group-specific scaling laws share the same $p_g=p \;\forall g$). Recall that the definition of underrepresented group $\gB$ is:
\begin{align*}
\gB \coloneqq 
\Bigg\{ g \Big|
\gamma_g < ( \frac{\omega_2}{\omega_1} + \sum_{g \in \gB} \gamma_g) * 
\frac{c_g^{1/p} l_{g,\omega}^{(p+1)/p}}{\sum_{g \in \gB} c_g^{1/p} l_{g,\omega}^{(p+1)/p}}
\Bigg\}.
\end{align*}
Then a group $g \in \gG$ belongs to the underrepresented group $\gB$ if its population prevalence satisfies:
\begin{align}
\gamma_g < \frac{\omega_2}{\omega_1}  * 
\frac{c_g^{1/p} l_{g,\omega}^{(p+1)/p}}{\sum_{g \in \gG} c_g^{1/p} l_{g,\omega}^{(p+1)/p}}.
\label{eq:minority_criteria_full}
\end{align}

\label{thm:minority_group_criteria_full}
\end{corollary_prop}

\begin{proof}
Notice that the right-hand side of (\ref{eq:minority_criteria_full}) is an lower bound of the condition in $\gB$. Specifically,
\begin{alignat*}{2}
&
( \frac{\omega_2}{\omega_1} + \sum_{g \in \gB} \gamma_g) * 
\frac{c_g^{1/p} l_{g,\omega}^{(p+1)/p}}{\sum_{g \in \gB} c_g^{1/p} l_{g,\omega}^{(p+1)/p}} \\
\geq \; & 
( \frac{\omega_2}{\omega_1}) * 
\frac{c_g^{1/p} l_{g,\omega}^{(p+1)/p}}{\sum_{g \in \gB} c_g^{1/p} l_{g,\omega}^{(p+1)/p}} 
&& \mbox{(Since $\sum_{g \in \gB} \gamma_g \geq 0$)} \\
\geq \; & 
( \frac{\omega_2}{\omega_1}) * 
\frac{c_g^{1/p} l_{g,\omega}^{(p+1)/p}}{\sum_{g \in \gG} c_g^{1/p} l_{g,\omega}^{(p+1)/p}} 
&& \mbox{(Since $\gB \subseteq \gG$ and $c_g, l_{g,\omega}$ are non-negative)}.
\end{alignat*}
Therefore, if (\ref{eq:minority_criteria_full}) holds, we have:
\begin{align*}
\gamma_g 
<  
( \frac{\omega_2}{\omega_1}) * 
\frac{c_g^{1/p} l_{g,\omega}^{(p+1)/p}}{\sum_{g \in \gG} c_g^{1/p} l_{g,\omega}^{(p+1)/p}} 
\leq 
( \frac{\omega_2}{\omega_1} + \sum_{g \in \gB} \gamma_g) * 
\frac{c_g^{1/p} l_{g,\omega}^{(p+1)/p}}{\sum_{g \in \gB} c_g^{1/p} l_{g,\omega}^{(p+1)/p}},
\end{align*}
which implies $\gamma_g \in \gB$.
\end{proof}

\begin{corollary_prop}[Generalization Error-based Sampling Selects Underrepresented Group]
Assuming the group-specific scaling laws share the same $p_g=p, q_g=q, \tau_g=\tau, \delta_g=\delta \;\forall g$. Then the definition of underrepresented group $\gB$ is:
\begin{align*}
\gB \coloneqq 
\Bigg\{ g \Big|
\gamma_g < ( \frac{\omega_2}{\omega_1} + \sum_{g \in \gB} \gamma_g) * 
\frac{c_g^{1/p}}{\sum_{g \in \gB} c_g^{1/p}}
\Bigg\}.
\end{align*}
Notice that the criteria for underrepresented groups remains the same even when $n \rightarrow \infty$.

Recall that under the empirical distribution $\gD$, by Assumption \ref{def:group_scaling_law}, the generalization error for a group $g$ is $e_g \coloneqq c_g n_g^{-p} + \tau n^{-q} + \delta$. Then, under a
generalization-error based active sampling policy $I(e_g > t_n)$ with threshold $t_n$, i.e., an example is selected if its generalization exceeds $t_n$. There exists a optimal threshold $t_n$ such that a group will be selected if and only if it belongs to $\gB$.
\label{thm:optimality_cv_active_sampling}
\end{corollary_prop}

\begin{proof}
Under the empirical distribution, the size of each group can be expressed as $n_g = \gamma_g n$. Then, the threshold-based sampling policy implies:
\begin{alignat*}{2}
t_n &< c_g (\gamma_g n)^{-p} + \tau n^{-q} + \delta,
&& \mbox{which implies}
\\
(\gamma_g n)^{p}  &< c_g (t_n - \tau n^{-q} - \delta)^{-1}, 
&& \mbox{which implies}
\\
\gamma_g  &< n^{-1} c_g^{1/p} (t_n - \tau n^{-q} - \delta)^{-1/p}.
\end{alignat*}
Then, equating the last expression with the criteria for the underrepresented group $\gB$, we have:
\begin{align*}
n^{-1} c_g^{1/p} (t_n - \tau n^{-q} - \delta)^{-1/p} &=  ( \frac{\omega_2}{\omega_1} + \sum_{g \in \gB} \gamma_g) * 
\frac{c_g^{1/p}}{\sum_{g \in \gB} c_g^{1/p}}
&& \mbox{which implies}
\\
t_n &=  
C n^{-p} + \tau n^{-q} + \delta,
\end{align*}
where $C=\big[ ( \frac{\omega_2}{\omega_1} + \sum_{g \in \gB} \gamma_g) / 
(\sum_{g \in \gB} c_g^{1/p}) \big]^{-p}$ is a constant that does not depend on $n$. 
Consequently, there exists a threshold $t_n=C * n^{-p} + \tau n^{-q} + \delta$ such that it selects a group $g$ if and only if it belongs to the underrepresented group $\gB$.
\end{proof}


%\newpage
\section{Proof of Propositions}
\subsection{Proof of \Cref{thm:optimal_allocation_frontier_full}}
\label{sec:optimal_allocation_frontier_full_proof}
\input{proof/prop_app_1_proof}


%\newpage
\section{Proof of Lemmas}
\label{eq:lemma_proof}

\subsection{Proof of \Cref{thm:allocation_weighted_risk}}
\label{sec:allocation_weighted_risk_proof}
\input{proof/lemma_1_proof}


\subsection{Proof of \Cref{thm:allocation_worst_risk}}
\label{sec:allocation_worst_risk_proof}
\input{proof/lemma_2_proof}

%\newpage

\begin{assumption}[Group-specific generalization error  \citep{rolf2021representation}]
The group-specific generalization error $R(f_{D}|G=g)=E_{D_g}(L(y, f_D))$ can be approximated by a scaling function of the group sample size $n_g$ and the total sample size $n$. That is, $\exists \, M_g >0$ and  constants $c_g, \tau_g, \delta_g \geq 0$, $p_g, q_g > 0$ such that for a dataset $D_{\alpha, n}$ with sample size $n$ and group allocation $\alpha=\{\alpha_g\}_{g\in \gG}$, and $f_{D_{\alpha, n}}$ the model trained $D$ with a particular algorithm, the generalization error $R(f_{D_{\alpha, n}}|G=g)$ can be approximated as:
\begin{align}
%\nonumber
R(f_{D_{\alpha, n}}|G=g) &\approx 
r(n_g, n | c_g, \tau_g, \delta_g, p_g, q_g) 
= c_g * n_g^{-p_g} + \tau_g * n^{-q_g} + \delta_g.
\label{eq:group_scaling_law}
\end{align}
The above is assumed to hold for any $\alpha \in \Delta^{|\gG|}$ and any $n$ such that $n_g = \lfloor \alpha_g n \rfloor \geq M_g$.
\vspace{-0.5em}
\label{def:group_scaling_law}
\end{assumption}
Assumption \ref{def:group_scaling_law} essentially states that each group has an unique learning rate $o(c_g n^{-p_g} + \tau_g n^{-q_g})$, which includes a $\tau_g n^{-q_g}$ term to allow the overall data size to influence the risk of group $g$. The scaling coefficients $(c_g, \tau_g, p_g, q_g)$ describes the difficulty of the learning problem.
%, where higher values of $(c_g, \tau_g)$ and lower values of $(p_g, q_g)$ indicate that the group $g$ is more difficult to learn (i.e., the generalization error decreases slower with respect to sample size). Note that for common choices of loss function, we expect $p_g, q_g$ to be bounded in a small range (e.g.,  $p_g, q_g  < 1$ for squared loss, since the optimal parametric learning rate is $n^{-1}$ \citep{bach2017breaking}). It should be acknowledged that the Assumption \ref{def:group_scaling_law} is simplistic, as it assumes that the scaling coefficients $(c_g, \tau_g, p_g, q_g)$ are not impacted by the group composition of the training data $\alpha$. However, 
\citet{rolf2021representation} shows that (\ref{eq:group_scaling_law}) holds exactly in classic settings such as linear regression, and verified that it approximated holds empirically in, e.g., image classification tasks using ResNet models.


==> sections/background_backup.tex <==
Given a dataset $D \sim \gD$ and a loss function $L$ , we consider learning the prediction function 
\[f_D = \argmin_{f \in \gF} L(f, y|D), \text{ where } L(y, f|D)=\sum_{\{\rvx_i, y_i\}\in D} L(y_i, f(\rvx_i)).\] Following the previous work \citep{pfau2013generalized}, we denote the \textit{ensemble predictor}:
\[\bar{f} = \argmin_{f\in \gF} E_{D\sim\gD}(L(f_D, f))\]
over ensemble members $f_D$'s, where each $f_D$ is trained on a random draw of training dataset $D \sim \gD$. 
% We also denote $f^*=\argmin_{f \in \gF} E_{D^*}L(f, y|D^*)$ the \textit{oracle predictor} that is learned from the infinitely-large and perfectly-balanced oracle training set $D^*$. Note that $f^*$ is deterministic due to the infinitely large size of $D^*$.
For test example $\{y_i, \rvx_i\}$, we can decompose the predictive error of a trained model $f_D(\rvx)$ using a generalized bias-variance decomposition for Bregman divergence:
\begin{proposition}[Noise-Bias-Variance Decomposition under Bregman divergence \citep{domingos2000unified, pfau2013generalized}] 
Given a loss function of the Bregman divergence family, for a test example $\{y, \rvx\}$ the expected prediction loss $L(y, f_D(\rvx))$ of an empirical predictor $f_D$ can be decomposed as:
\begin{align}
E_D \big[ L(y, f_D(\rvx)) \big]
&= 
\underbrace{E_{D} \big[ L(y, \tilde{y}(\rvx)) \big]}_\text{{\color{OliveGreen} Noise}}
+ \quad
\underbrace{L(\tilde{y}(\rvx), \bar{f}(\rvx))}_\text{{\color{Maroon} Bias}}
\quad + \quad
\underbrace{E_{D} \big[ L(\bar{f}(\rvx), f_D(\rvx)) \big]}_\text{{\color{RoyalBlue} Uncertainty}}
\label{eq:error_decomposition}
\end{align}
\vspace{-1.5em}
\label{thm:error_decomposition_app}
\end{proposition}
%Proof is in \Cref{sec:error_decomposition_proof}. \Cref{thm:error_decomposition} is a generalization of the classic noise-bias-variance decomposition result \citep{domingos2000unified} to account for the model mis-specification error in $\gF$. This is achieved by defining $f^*=\argmin_{f \in \gF} E_{D^*}L(f, y|D^*)$ as the best-achievable function within the model class $\gF$, rather than the Bayes optimal predictor $f^{opt}(\rvx_i) = \argmin_{y'} E_{y\sim P(y|\rvx_i, g_i)}L(y, y')$. 
We now interpret each of the terms defined above: \\
\emph{\bf Noise:} Given a fixed data distribution $\gD$, the first term {\color{OliveGreen} $E_{D} \big[ L(y, f^*(\rvx)) \big]$} quantifies the {\color{OliveGreen} \textit{irreducible noise}} that is due to the stochasticity in the noisy observation $y$. \\%or the mis-specification in the model class $\gF$. 
\emph{\bf Uncertainty:} The third term {\color{RoyalBlue} $E_{D} \big[ L(\bar{f}(\rvx), f_D(\rvx)) \big]$} quantifies the {\color{RoyalBlue} \textit{model uncertainty}} in the prediction, which can be due to variations in the finite-size data $D$, the stochasticity in the randomized learning algorithm $\gF \times D \rightarrow f_D$, or the randomness in the initialization of an  overparameterized model \citep{adlam2020understanding}. \\
\emph{\bf Bias:} Finally, the middle term {\color{Maroon} $L(\tilde{y}(\rvx), \bar{f}(\rvx))$} quantifies the gap between  $\tilde{y}(\rvx)$ (i.e., the ``true label") and the ensemble predictor $\bar{f}$ learned from the empirical data $D \sim \gD$. For the examples $\rvx$ coming from the under-represented groups with $\gamma_g \ll \frac{1}{|\gG|}$, the bias term can be further decomposed into:
\begin{align}
L(\tilde{y}(\rvx), \bar{f}(\rvx))
&= 
\underbrace{L(\tilde{y}(\rvx), \bar{f}^*(\rvx))}_\text{{\color{Maroon} \textit{Bias, Model}}}
+
\underbrace{\gE(\bar{f}^*(\rvx), \bar{f}(\rvx))}_\text{{\color{Maroon} \textit{Excess Bias, Data}}},
\label{eq:bias_decomposition}
\end{align}
where $\bar{f}^\ast = \argmin_{f\in \gF} E_{D^\ast \sim \gD^\ast}(L(f_{D^\ast}, f))$ is the optimal ensemble predictor based on size-$n$ datasets $D^\ast$ sampled from the optimal distribution $\gD^\ast$ where all groups have equal representation. Here, $L(\tilde{y}(\rvx), \bar{f}^*(\rvx))$ is the bias inherent to the model class and cannot be eliminated by ensembling. It can be caused by model misspecification, missing features, or regularization. On the other hand, $\gE(\bar{f}^*(\rvx), \bar{f}(\rvx)) = L(\tilde{y}(\rvx), \bar{f}(\rvx)) - L(\tilde{y}(\rvx), \bar{f}^*(\rvx))$ indicates the ``excess bias" for the under-represented groups caused by the imbalance in the group distribution $P(G)$ in the data-generation distribution $\gD$. 

To make the idea concrete, consider a simple example where we fit a ridge regression model $f(\rvx_i)=\beta^\top \rvx_i$ to the Gaussian observation data $y_i=\theta^{\top} \rvx_i + \epsilon, \epsilon \sim N(0, \sigma^2)$ under an imbalanced experiment design, where we have $|\gG|$ treatment groups and $n_g$ observations in each group. Here, $\rvx_i = [1_{g_i = 1}, ..., 1_{g_i = |\gG|}]$ is a $|\gG| \times 1$ one-hot indicator of the membership of $g_i$ for each group in $\gG$, and $\theta=[\theta_1, \dots, \theta_{|\gG|}]$ is the true effect for each group. Then, under ridge regression, the noise-bias-variance decomposition for group $g$ is $E_D(L(y, f_D))={\color{OliveGreen} \sigma^2} + {\color{Maroon} \frac{(\lambda\theta_g)^{ 2}}{(n_g + \lambda)^2}} + {\color{RoyalBlue} \frac{\sigma^2 n_g}{(n_g + \lambda)^2}}$, where the regularization parameter $\lambda$  modulates a trade-off between the {\color{Maroon} \textit{bias}} and {\color{RoyalBlue} \textit{uncertainty}} terms 
(\Cref{sec:error_decomposition_ridge}). Consequently, for an underrepresented group with small size $\gamma_g \ll \frac{1}{|\gG|}$, its predictive bias ${\color{Maroon} \frac{(\lambda\theta_g)^{\ast 2}}{(n_g + \lambda)^2}}$ is exacerbated due to lacking sufficient statistical information to counter the regularization bias, incuring an excessive bias of $\gE(\bar{f}^*(\rvx), \bar{f}(\rvx))\approx \frac{\lambda \theta_g}{n \gamma^\ast_g \gamma_g}(\gamma^\ast_g - \gamma_g)$ when compared to an optimal ensemble predictor $\bar{f}^*$ trained from a perfectly balanced size-$n$ datasets with $\gamma^\ast_g=1/|\gG|$.

Finally, note that in \Cref{eq:error_decomposition}, the first two terms combined constitute the traditional bias term $E_D[L(y, \bar{f})]=E_{D} \big[ L(y, f^*(\rvx)) \big] + L(f^*(\rvx), \bar{f}(\rvx))$ in the classic bias-variance decomposition. To this end, the conceptual significance of Equations (\ref{eq:error_decomposition})-(\ref{eq:bias_decomposition}) is to isolate data imbalance as a distinct source of systematic error (i.e., that is different from those due to label noise or model misspecification), motivating us to explore the practical approximation of $\gE(\bar{f}^*(\rvx), \bar{f}(\rvx))$ for improving model performance under dataset bias (\Cref{sec:bias_estimation}).

As an aside, when the predictive model $f_D$ is probabilistic (e.g., the model generates a posterior predictive distribution $P(f|D)$ rather than a point estimate $f$), the {\color{RoyalBlue} \textit{model uncertainty}} in \Cref{eq:error_decomposition} is further decomposed as:
\begin{align}
E_D \big[ L(\bar{f}(\rvx), f_D(\rvx)) \big]= 
\underbrace{ E_D \big[ L(\bar{f}(\rvx), \mu_D(\rvx))  \big]}_\text{
{\color{RoyalBlue}\textit{Ensemble Diversity}}} + 
\underbrace{E_D E_{f \sim P(f|D)} \big[ L(\mu_D(\rvx), f(\rvx)) \big] }_\text{
{\color{RoyalBlue}\textit{Posterior Variance}}}
\end{align}
where $\mu_D(\rvx)=E_{f\sim P(f|D)}[f(\rvx)]$ is the posterior mean. As shown, comparing to an ensemble of deterministic models, the ensemble of probabilistic models provides additional flexibility in quantifying model uncertainty via the extra term of expected posterior variance.


==> sections/intro_backup.tex <==
\input{figures/acc_fair_intro}

The modern \glsfirst{DNN} models are commonly trained on the large-scale, in-the-wild datasets \citep{deng2009imagenet}.
These data often exhibits an imbalanced long-tail distribution with many small population subgroups, reflecting the nature of the physical and social processes underlying the data distribution 
\citep{zhu2014capturing, feldman2020neural%yang2020rethinking,
}. 
This imbalance in training data distribution, i.e., \textbf{\textit{dataset bias}}, has prevented the \gls{DNN} models from generalizing equitably to the under-represented population groups
\citep{hasnain2007disparities%, ekstrand2018all, hofmanninger2020automatic
}. {\color{red} mention spurious correlation}

\textbf{Accuracy-Fairness Frontier:} In response, the existing bias mitigation literature has focused on improving the training procedure under a fixed and imbalanced training dataset, striving to produce a balanced performance between model accuracy and fairness (e.g., the average-case v.s. worst-group performance)
\citep{agarwal2018reductions, martinez2020minimax, martinez2021blind}%, sagawa2020investigation, liu2021just}
. Formally, this goal corresponds to identifying a optimal model $f \in \gF$ that attains the \textit{Pareto efficiency frontier} of the accuracy-fairness trade-off (e.g., see \Cref{fig:acc_fair_frontier_intro}), so that under the same training data $D=\{y_i, \rvx_i\}_{i=1}^n$, we cannot find another model $f' \in \gF$ that outperforms $f$ in both accuracy and  fairness. In the literature, this \textit{accuracy-fairness frontier} is often characterized by a trade-off objective \citep{martinez2021blind}:
\begin{align}
    f_\lambda = \argmin_{f\in \gF} F_{\lambda}(f|D); 
    \qquad
    F_{\lambda}(f|D) \coloneqq R_{acc}(f|D) + \lambda R_{fair}(f|D),
    \label{eq:frontier_risk_intro}
\end{align}
\vspace{-1.5em}

where $R_{acc}$ and $R_{fair}$ are risk functions for a model's accuracy and fairness, and $\lambda > 0$ a trade-off parameter.
Then, $f_\lambda$ cannot be outperformed by any another $f'$ at the trade-off level $\lambda$.
The entire frontier under a dataset $D$ can then be characterized by finding $f_\lambda$ that minimizes the fairness-accuracy objective (\ref{eq:frontier_risk_intro}) at every trade-off level $\lambda$, and tracing out their $(R_{acc},  R_{fair})$ performances
%on a 2D plane 
(\Cref{fig:acc_fair_frontier_intro}).

\textbf{Goal:} However, bias-robust learning under a fixed and imbalanced dataset comes with inherent challenges.
The limited size of the tail-group examples restricts the \gls{DNN} model's worst-group performance, leading to a compromised accuracy-fairness frontier 
% (i.e., a high value in the $min_{f \in \gF} F_\lambda(f|D)$)
\citep{zhao2019inherent, dutta2020there%vzliobaite2015relation, menon2018cost
}. 
Recognizing this inherent limitation brought by the dataset distribution, we ask: 

\textit{Under a fixed learning algorithm, can we meaningfully push the model's accuracy-fairness frontier by improving the training data distribution using active learning?} 

That is, denoting $D_{\alpha, n}=\{(y_i, \rvx_i)\}_{i=1}^n$ a training dataset with $K$ subgroups and the group size distribution $\alpha = [\alpha_1, \dots, \alpha_K]$, we study that if a model's accuracy-fairness performance $F_\lambda$ can be improved by improving the group distribution of the training data $\alpha$, i.e., we seek to optimize an outer problem:
\begin{align}
% F_\lambda^* = 
{\color{Maroon} \minimize_{\alpha \in \Delta^{|\gG|}}}
\Big[ \min_{f \in \gF} F_{\lambda}(f|D_{{\color{Maroon}\alpha},n}) \Big],
\label{eq:al_objective_intro}
\end{align}
where $\Delta^K$ is the simplex of all possible group distributions \citep{rolf2021representation}. In practice, the uncertainty-based \gls{AL} holds promise to achieve this exact objective: given a sampling model with \textit{well-calibrated} uncertainty (i.e., the model uncertainty is well-correlated with generalization error), \gls{AL} can pro-actively identify the unlabelled examples from the under-represented subgroups, and add them to the training data to reach a more balanced data distribution \citep{branchaud2021can}. 
% This this undoubtly appealing
% This helps the model to improve its worst-group performance without significantly sacrificing accuracy, thereby breaking the accuracy-fairness frontier otherwise ``locked" by an imbalanced data distribution \citep{idrissi2022simple} (\Cref{fig:acc_fair_frontier_intro}).

\textbf{Challenges with DNN Uncertainty under Bias:} However, the recent work suggest that the \gls{DNN} model's uncertainty estimate is less trust-worthy under spurious correlations and distributional shift, potentially compromising the \gls{AL} performance under dataset bias.
For example, \citet{ovadia2019can} shows that the \gls{DNN}'s expected calibration error rises as the testing data distribution deviates from the training data distribution, and \citet{ming2022impact} shows that \gls{DNN}'s ability in detecting out-of-distribution examples is significantly hampered by the spurious patterns. Looking deeper, \citet{liu2022simple, ming2022impact, van2020uncertainty} suggests that this failure mode in \gls{DNN} uncertainty can be caused by an issue in representation learning known as \textit{feature collapse}, where the model over-focused on correlational features that helps to distinguish between the output classes on the training data, but ignored the non-predictive but still semantically meaningful input features that are important for uncertainty quantification (\Cref{fig:2d_example}). In this work, we show that this failure mode can be provably mitigated by a training procedure we term \textit{introspective training}(\Cref{sec:method}). Briefly
introspective training adds an auxiliary \textit{introspection} task to model training, asking the model to predict whether an example belongs to the under-represented groups. 
It comes with a guanrantee in injecting \textit{bias-awareness} into model representation (\Cref{thm:bias_awareness}), encouraging it to learn diverse hidden features that distinguishes the minority-group examples from the majority group, even if these features are not correlated with the target labels on the training dataset. As a result, introspective training helps the model to circumvent the well-known pathology of \textit{feature collapse} under spurious correlation, leading to improved uncertainty quality for the tail groups (\Cref{fig:2d_example}). 

\textbf{Contributions:} In this work, we study the problem of improving a \gls{DNN} model's fairness-accuracy frontier by improving the training data distribution using active learning 
(\Cref{eq:al_objective_intro}).
%\vspace{-1em}
\begin{itemize}[noitemsep,topsep=0pt,leftmargin=0.5cm]
    \item We first introduce \textbf{\gls{ISP}}, a simple training approach to improve a \gls{DNN} model's uncertainty quality for the under-represented groups (\Cref{sec:method}). Using group annotations from the training data, \gls{ISP} conducts \textit{introspective training} to provably improves a \gls{DNN}'s representation and uncertainty quality for the tail groups. When the group annotation is not available, \gls{ISP} additionally estimates it using a cross-validation-based procedure that conducts a noise-bias-variance decomposition of model's generalization error \citep{domingos2000unified}.
    \item \textbf{Theoretical Analysis.} Complementing the method development, we conduct a initial theoretical analysis the optimization problem (\ref{eq:al_objective_intro}) under a group-specific learning rate model \citep{rolf2021representation} (\Cref{sec:theory}). Our result elucidates the role of training data distribution $\alpha$ in the model’s best-attainable accuracy-fairness frontier $F_\lambda$. In particular, it confirms the theoretical necessity of up-sampling the under-represented groups for obtaining the optimal accuracy-fairness frontier, and revealed an non-obvious fact that the notion of \textit{under-representation} is in fact a interplay of the subgroup's learning difficulty and its population prevalence.
    \item \textbf{Empirical Effectiveness.} Under two challenging real-world tasks (census income prediction and toxic comment detection), we empirically validate the effectiveness of \gls{ISP} training in improving a \gls{DNN} model's active learning performance under dataset bias. \gls{ISP} helped uncertainty-based \gls{AL} methods to achieve much improved tail-group sampling rate, meaningfully pushing the accuracy-fairness frontier of the final model.
\end{itemize}

==> sections/intro_bullet.tex <==
\jereliu{logic flow: accuracy-fairness frontier $\rightarrow$ importance of data distribution $\rightarrow$ active learning $\rightarrow$ caveat of deep learning uncertainty $\rightarrow$ ISP}
\balaji{Sycned with Jeremiah: these bullet points will eventually go away}

% Background:
% \begin{itemize}
% \item The modern \gls{DNN} models are commonly trained on the large-scale, in-the-wild datasets. \citep{deng2009imagenet}
% \item These data tend to exhibit an imbalanced long-tail distribution with many small population subgroups, reflecting the natural or societal mechanisms underlying the data generation process \citep{zhu2014capturing, yang2020rethinking, feldman2020neural}. 
% \item This imbalance in training data distribution (i.e., \textit{dataset bias}) has prevented the \gls{ML} models from generalizing equitably to the underrepresented population groups. \citep{hasnain2007disparities, ekstrand2018all, hofmanninger2020automatic}.
% \item In response, many spurious correlation and fairness research has focused on improving model training under a fixed and imbalanced training dataset, striving towards a balanced model performance that offers competitive utility (average-case performance) while ensuring fairness (e.g., worst-case performance) \citep{martinez2021blind, martinez2020minimax, agarwal2018reductions, sagawa2020investigation, liu2021just} (see \Cref{sec:related_debiasing_supervised} for a review).
% \item Formally, developing models with balanced accuracy-fairness tradeoff. Measured by accuracy-fairness frontier \citep{martinez2020minimax, martinez2021blind, agarwal2018reductions, little2022fairness}.
% \end{itemize}

% Goal:
% \begin{itemize}
% \item 
% However, fairness learning under a fixed dataset comes with inherent challenges.
% The limited size of the tail groups invariably restricts the model's worst-group performance, leading to a compromised frontier in the accuracy-fairness tradeoff  (i.e., a high value in the $min_{f \in \gF} F_\lambda(f|D)$)
% \citep{zhao2019inherent, dutta2020there%vzliobaite2015relation, menon2018cost
% }. 
% \item In this work, recognizing this inherent limitation brought by this imbalanced distribution, we ask an orthogonal question: \textit{under a fixed learning algorithm, can we ``break" the accuracy-fairness frontier of the model by improving the distribution of the training data?} That is, for example, given a fixed model class $\gF$ and denote $D_{\alpha, n}$ a size-$n$ training dataset with group-size allocation $\alpha = [\alpha_g]_{g \in \gG}$, we study that if we can improve the accuracy-fairness frontier $F_\lambda(f|D_{\lambda, n})$ by studying the outer optimization problem \citep{rolf2021representation}:
% \begin{align}
% F_\lambda^* = 
% {\color{Maroon} \min_{\alpha \in \Delta^{|\gG|}} }
% \Big[ \min_{f \in \gF} F_{\lambda}(f|D_{{\color{Maroon}\alpha},n}) \Big],
% \label{eq:al_objective_intro}
% \end{align}
% where $\Delta^{|\gG|}$ is the simplex of all possible group size allocations. 
% \item Concretely, we study uncertainty-based \glsfirst{AL} as an approach to optimize the above objective in practice. 
% We expect this direction to be fruitful: 
% By diversely sampling from the under-represented tail groups, \gls{AL} is expected to attain a well-balanced dataset that offers richer sets of examples from the tail population, helping the model $f \in \gF$ to naturally achieve a better performance for the worst-case group, and thereby ``breaking" the accuracy-fairness frontier otherwise ``locked" by an imbalanced data distribution without needing additional modeling change
% \citep{rolf2021representation, chen2018my, idrissi2022simple, branchaud2021can}.
% \end{itemize}

% Challenges:
% \begin{itemize}
%     \item (Caveat in Deep Uncertainty) 
%     However, \gls{DNN} models exhibits failure modes in the presence of spurious correlation and subpopulation shifts 
%     \citep{sagawa2020investigation}
%     \citep{tran2022plex}. Can be traced to issue in the embedding space \citep{liu2022simple}. 
%     \item (Unknown bias) There exists many situations where the sources of biases are unknown or hidden, where it is infeasible to manually categorize or annotate all sources of the underlying data biases due to its enormous size or the external regulatory constraints \citep{ekstrand2018all, veale2017fairer, holstein2019improving}.
%     \item (Secondary, Label Noise) Furthermore, labeling noise is known to be pervasive in real-world data curation process and annotation pipelines (more so for tail groups), creating additional challenges for bias estimation techniques  \citep{li2022more, northcutt2021pervasive}.
% \end{itemize}

% \vspace{5em}

Contribution I: Method
\begin{itemize}
    \item We propose \textit{\glsfirst{ISP}}, a simple approach to improve the uncertainty quality of a deep neural network under dataset bias. ISP adds an auxiliary \textit{introspection} task to model training, asking the model to predict whether an example belongs to an under-represented group. {\color{red} (mention representation learning guanrantee).}
    \item In the situation of unknown bias, \gls{ISP} estimates the bias label using a cross-validation-based \textit{self-play} procedure. It answers the aforementioned challenges by estimating bias label using noise-bias-variance decomposition \citep{domingos2000unified}
    .
\end{itemize}
\Cref{sec:related_work} surveys related work.

Contribution II: Theory
\begin{itemize}
    \item Complementing the method development, we also conduct an initial theoretical investigation to elucidate the role of training data distribution in the model's ability in obtaining the optimal accuracy-fairness frontier.
    \item Specifically, under a group-specific learning rate model \citep{chen2018my, rolf2021representation}, we derive the optimal group distribution $\alpha^*$ that minimizes the frontier risk (\ref{eq:frontier_risk}), analyzing how it interacts with both the empirical prevalence and the inherent learning difficulty of each group (\Cref{thm:optimal_allocation_frontier_main}).
    \item Our result reveals two simple yet non-obvious insights: 
    \begin{itemize}
        \item to attain optimal worst-group accuracy (i.e., the minimax group fairness \citep{rawls2001justice, lahoti2020fairness, martinez2020minimax, gil2022minimax}), the group distribution should be primarily informed by the relative learning difficulty of each group, rather than their existing prevalence in the data \citep{nam2020learning}.
        \item Furthermore, it confirms that to attain an optimal fairness-accuracy performance, a group needs to be upsampled only if their existing prevalence doesn't justify their learning accuracy. i.e., the definition of ``under-represented groups" is a joint property of the group's empirical prevalence and its learning difficulty.
    \end{itemize}
    \item Further justifying active sampling policy informed by model's  generalization error.
\end{itemize}

We conclude the paper with an empirical investigation.
Contribution III: Experiments



==> sections/theory.tex <==

Denote by $\Delta^K$ the $K$-simplex so that $\forall \alpha=[\alpha_1, \dots, \alpha_K] \in \Delta^K$,  $\sum_k \alpha_k = 1$ and $\forall k$, $\alpha_k > 0$. Let $D_{\alpha, n}$ denote a dataset of size $n$ sampled with group allocations $\alpha \in \Delta^{|\gG|}$, i.e., $\alpha_g$ represents the fraction of the dataset sampled from group $g \in \gG$. Our goal is to find the optimal allocation that minimizes a weighted combination of the population risk and the worst-case risk over all subgroups.

\begin{definition}[Risk and Fairness Risk] Given $f \in \gF$, let $R(f|\alpha, n)\coloneqq \sum_{g\in \gG} \gamma_g R(f|G=g)$ be the risk where $\gamma \in \Delta^{|\mathcal{G}|}$ represents the true subgroup proportions in the underlying data distribution, and $\Rfair(f)$ be the fairness risk which is the worst-case risk among the groups $g\in \gG$: 
$\Rfair(f) \coloneqq \max_g R(f|G=g)$. 
\vspace{-1em}

\end{definition}
% related work \citep{zhao2019inherent, menon2018cost, little2022fairness}

%This is the form of the fairness-accuracy tradeoff objective we introduced in \Cref{sec:intro}, i.e., $F_\omega \propto R + \frac{\omega_2}{\omega_1} \Rfair$, where the standard risk $R$ is combined with a ``fairness constraint" $\Rfair$ under a trade-off parameter $\frac{\omega_2}{\omega_1}$.

Let $\hat{R}$ and $\Rfairhat$ denote the empirical estimates of $R, \Rfair$ estimated based on the finite dataset $D_{\alpha, n}$:
\[\hat{R}_{\alpha, n, g}\br{f} = \frac{\sum_{(x, y) \in D_{\alpha, n, g}} L\br{f\br{x}, y}}{|D_{\alpha, n, g}|} , \hat{R}_{\alpha, n}\br{f}=\sum_g \gamma_g \hat{R}_{\alpha, n, g}\br{f}, \Rfairhatan\br{f} = \max_g \hat{R}_{\alpha, n, g}\br{f}\]

where $D_{\alpha, n, g}$ is the subset of $D_{\alpha, n}$ with group label $g$. Let $\hat{f}$ denote the classifier obtained as per $\gamma$-weighted empirical risk minimization (ERM)
$\hat{f}_{\alpha, n} = \argmin_{f \in \gF} \hat{R}_{\alpha, n}\br{f}$. 

\begin{definition}[Accuracy-Fairness Frontier Risk]
For non-negative weighting coefficients $\omega \in [0, 1]$, the accuracy-fairness frontier risk is defined as:
\begin{align}
F_{\omega}(\alpha, n) \coloneqq 
\omega E[R(\hat{f}_{\alpha, n})] + (1-\omega) E[\Rfair(\hat{f}_{\alpha, n})]
\label{eq:frontier_risk}
\end{align}
where the expectation is taken wrt the randomness inherent in $\hat{f}$ as it is estimated based on a random dataset $D_{\alpha, n}$ drawn iid from the underlying data distribution.  
\vspace{-1em}
\label{def:fairness_accuracy_frontier}
\end{definition}
As we sweep over $\omega$ going from $0$ to $1$ and find the best classifier/allocation for each value, we would trace an accuracy fairness frontier as in \Cref{fig:acc_fair_frontier_intro}.

% \subsection{Analyzing optimal allocation between subgroups}
\textbf{Analyzing optimal allocation between subgroups.} We theoretically analyze the optimization problem
$\alpha^* = 
 \argmin_{\alpha \in \Delta^{|\gG|}} 
\Big[ F_{\omega}(\alpha, n) \Big].$
% in order to obtain an initial understanding of the potential impact of training data's group distribution in the resulting model's accuracy-fairness performance. 
%\martin{As written, this doesn't quite work. $F_\omega$ is independent of $\alpha$. We need to state that $f$ is obtained by optimizing the empirical loss for a given $\alpha$ and then $\alpha^*$ leads to the $f$ with the lowest risk for the true $\gamma$. As written $f$ directly optimizes the loss for $\gamma$.}
We build on the theoretical models for group-specific scaling laws of generalization error introduced in previous work. \citep{chen2018my, rolf2021representation}. We assume that the group-specific true risk decays with the size of the dataset at a rate of the form:
\[E[R\br{\hat{f}_{\alpha, n}|G=g}]=c_g \br{\alpha_g n}^{-p} + \tau n^{-q} + \delta\]
for some $p >0, q > 0, c_g > 0, \tau, \delta > 0$. The first term represents the impact of the group representation, the second  the aggregate impact of the dataset size, and the third term a constant offset (the irreducible risk for this group). In particular, $c_g$ represents the ``difficulty`` of learning group $g$, as the larger $c_g$ is, the higher the risk is for group $g$ for any given allocation $\alpha$.

\begin{theorem}[Optimal Group-size Allocation for Accuracy-Fairness Frontier Risk (Informal)]
The optimal allocation $\alpha^\star$ is of the form $\alpha_g^\star \propto \br{\gamma_g c_g \theta_g}^{\frac{1}{p+1}}$ where
$\theta_g \geq \omega$ represents an up-sampling factor for group $g$. Let $g_1, g_2, \ldots$ be the subgroups sorted in ascending order according to the value $\gamma_g c_g^{-1/p}$, which represents the subgroup representation normalized by the difficulty of learning the subgroup. Then, it holds that there exists an integer $k > 0$ such that $\theta_{g_i} = \omega$ for $i = k, \ldots |\gG|$, $\theta_{g_i} > \omega$ for  $i= 1, \ldots, k$. Thus, the subgroups with low normalized representation are systematically up-sampled in the optimal allocation. 
\label{thm:optimal_allocation_frontier_main}
\end{theorem}

Based on the above theorem, we can the set of underrepresented groups as 
$\mathcal{B}=\{g_1, g_2, \ldots g_k\}.$, validating the idea that underrepresented groups can be formally defined. While the result above is derived under a simplified theoretical model, it validates the intuition behind ISP: indeed, ISP attempts to infer whether datapoints belong to $\mathcal{B}$ and systematically up-samples them via active learning to increase the overall representation and achieve an allocation closer to the theoretically optimal allocation defined above. We present a full theorem statement and proof in \Cref{sec:optimal_allocation_frontier_proof} and a discussion in \Cref{sec:optimal_allocation_frontier_discussion}

\begin{comment}

x%\dvij{I think we should summarize the results below with an informally stated theorem. I think the details are anyway not very interesting as the assumptions made are quite restrictive. What's more important is the insight that the optimal allocation}

To this end, the below theorem 
% elucidates the importance of the training data's group-size allocation on the resulting model's fairness - accuracy performance. Importantly, \Cref{thm:optimal_allocation_frontier_main} theoretically
confirms that a model's fairness-accuracy frontier can be improved by careful design of the training data (i.e., by sufficiently representing data groups that are under-represented in the population). 
%This necessity notably does not vanish even under extremely large $n$, thereby highlighting the fact that the {\color{Maroon} \textit{data bias}} error in (\ref{eq:error_decomposition}) persists even in the asymptotics. 
Interestingly, it also provides a mathematical characterization for the heuristic notion of ``under-represented group" (i.e., \cref{eq:minority_group_criteria_main}), in terms of whether a group's population prevalence $\gamma_g$ is comparable to its relative learning difficulty (\Cref{eq:minority_group_criteria_main}).

\begin{theorem}[Optimal Group-size Allocation for Fairness-Accuracy Frontier]
Assuming the group-specific scaling laws (Assumption \ref{def:group_scaling_law}) differ only by the multiplicative coefficient $c_g$, so that the approximated group-specific risk is $\hat{R}(f_{D_{\alpha, n}}|G=g) \coloneqq c_g n_g^{-p} + \tau n^{-q} + \delta$. Denote the approximate population risk as $\hat{R}(\alpha, n) = \sum_g \gamma_g \hat{R}(f_{D_{\alpha, n}}|G=g)$ and the approximated worst-case risk as $\Rfairhat(\alpha, n) = \sup_v \sum_{g\in \gG} [ v_g \hat{R}(f_{D_{\alpha, n}}|G=g)]$. Then:
\begin{itemize}[leftmargin=0.5cm]
\item [(I)] \textbf{(Population Risk},  \citet{rolf2021representation})  If  $F_{\omega=\{1,0\}}(\alpha, n)=R(\alpha, n)$ is the standard population risk. The optimal training-data group distribution $\alpha^*$ that minimizes $\hat{R}(\alpha, n)$ is
$\alpha^*_g = 
\frac{(\gamma_g c_g)^{1/(p+1)} }
{\sum_{g\in \gG}(\gamma_g c_g)^{1/(p+1)}}.$
\item [(II)] \textbf{(Worst-case Risk)} If  $F_{\omega=\{0, 1\}}(\alpha, n)=\Rfair(\alpha, n)$ is the worst-case risk. The optimal 
training-data group distribution $\tilde{\alpha}^*$ that minimizes $\Rfairhat(\alpha, n)$ is
$\tilde{\alpha}^*_{g} = 
\frac{(c_g)^{1/p} }
{\sum_{g\in \gG}(c_g)^{1/p}}$, i.e., the relative learning difficulty of group $g$.
% \item [(III)] \textbf{(Fairness-Accuracy Frontier, Average-group Risk)} 
% Let $R_{fair}$ be the average-group risk $\bar{R}(\alpha, n)$ so that
% $F_{\omega}(\alpha, n) \coloneqq 
% \omega_1 * R(\alpha, n) + \omega_2 * \bar{R}(\alpha, n)$.
% The optimal training-set group-size allocation $\alpha^*$ that minimizes the approximated accuracy-fairness frontier $\hat{F}_\omega(\alpha, n)$ is: 
% \begin{align*}
% \alpha^*_g = \frac{(r_g c_g)^{1/(p+1)}}{\sum_{g\in \gG} (r_g c_g)^{1/(p+1)}}, 
% \quad \mbox{where} \quad
% r_g = \omega_1  \gamma_g + \omega_2 \frac{1}{|\gG|}.
% \end{align*}
\item [(III)] \textbf{(Fairness-Accuracy Frontier Risk)} 
For general $\omega>\mathbf{0}$, the optimal training-set group distribution $\alpha^*$ that minimizes the  $\hat{F}_\omega(\alpha, n) \coloneqq 
\omega_1 \hat{R}(\alpha, n) + \omega_2 \Rfairhat(\alpha, n)$ is: 
\begin{align}
\alpha^*_g = \frac{(r_g c_g)^{1/(p+1)}}{\sum_{g\in \gG} (r_g c_g)^{1/(p+1)}}, 
\quad \mbox{where} \quad
r_g = \max\Big[
\gamma_g, \;\;
\Big(\frac{\omega_2}{\omega_1} + \sum_{g \in \gB} \gamma_{g} \Big)\Big( \frac{c_g^{1/p}}{\sum_{g \in \gB} c_g^{1/p}} \Big) \Big].
\label{eq:optimal_sampling}
\end{align}
Here $\gB \subseteq \gG$ is the set of under-represented groups whose population prevalence $\gamma_g$ satisfy:
\begin{align}
\gB \coloneqq 
\Bigg\{ g \Big|
\gamma_g \leq 
\Big(\frac{\omega_2}{\omega_1} + \sum_{g \in \gB} \gamma_{g} \Big)\Big( \frac{c_g^{1/p}}{\sum_{g \in \gB} c_g^{1/p}} \Big)
\Bigg\}.
\label{eq:minority_group_criteria_main}
\end{align}
Furthermore, a sufficient condition for $g \in \gB$ is
$\gamma_g 
< 
\frac{\omega_2}{\omega_1} * (\frac{c_g^{1/p}}{\sum_{g \in \gG} c_g^{1/p}})$, where
$\frac{c_g^{1/p}}{\sum_{g \in \gG} c_g^{1/p}}$ is the relative learning difficulty of group $g$, and $\frac{\omega_2}{\omega_1}$ the relative weights of the worst-case and population risks.
\end{itemize}
\label{thm:optimal_allocation_frontier_main}
\end{theorem}
Proof is in \Cref{sec:optimal_allocation_frontier_proof}. In the above, Part (I) (Population Risk) is due to \citet{rolf2021representation}, it shows a striking fact that the optimal group sizes $\alpha^*$ minimizing the approximated empirical risk is \textit{not} the empirical distribution $\gamma=\{ \gamma_g \}_{g \in \gG}$, thereby highlighting the importance of training data design in achieving optimality in even the standard generalization performance\footnote{In \Cref{thm:allocation_weighted_risk} 
(\Cref{sec:lemma}), we go beyond the previous work to show that in a more general setting where the group-specific scaling coefficient $p_g$ is not equal, the optimal sampling allocation $\alpha^*$ in fact disproportionally favors the more difficult-to-learn groups as $n \rightarrow \infty$.}. Parts (II)-(III) are new to this work. Specifically, (II) highlights that to optimize the model's fairness performance (as measured by worst-case risk $\Rfair$), the group sizes in the training data should be proportional to the group's inherent learning difficulty (as characterized by $c_g^{1/p}$), \textit{irrespective} to the prevalence of these groups in the population $\gamma_g$. Finally, (III) highlights that the accuracy-fairness trade-off under a fixed learning algorithm can be improved by properly sampling the data groups.
%should be sampled according to whether it is \textit{under-represented}, i.e., if its population prevalence $\gamma_g$ does not sufficiently reflect its relative learning difficulty  {\scriptsize $c_g^{1/p}/(\sum_g c_g^{1/p})$} (\cref{eq:minority_group_criteria_main}).
In particular, under the assumption that we have oracle knowledge of the scaling laws $c_g n_g^{-p} + \tau n^{-1} + \delta$, Part (III) hints at a sampling procedure that guarantees optimality: Given a data group $g \in \gG$, if $g$ doesn't belong to the under-represented group $\gB$, sample it  according to a likelihood function that is proportional to population prevalence $\gamma_g$, otherwise sample it according to a likelihood function (\cref{eq:optimal_sampling}) that is lower bounded by the group's relative learning difficulty $c_g^{1/p}/(\sum_g c_g^{1/p})$ scaled by the relative weight of the fairness and accuracy risks $\omega_2 / \omega_1$. 

\end{comment}

==> sections/theory_long.tex <==

Given a dataset $D_{\alpha,n}$ with sample size $n$ and group allocation $\alpha=\{\alpha_g\}_{g\in \gG}$, we denote $f_D$ the model learned from $D$. We also denote the group-specific distribution as $D_g=P(y, \rvx|G=g)$, and the group-specific generalization error of a given model $f$ is $R(f|G=g)=E_{D_g} \big[ L(y, f|D_g) \big]$. Finally, denote $\Delta^K$ the space of $K$-simplex so that $\forall \alpha=[\alpha_1, \dots, \alpha_K] \in \Delta^K$, it satisfies $\sum_k \alpha_k = 1$ and $\alpha_k > 0 \, \forall k$. 

We consider the below notion of accuracy-fairness frontier:
\begin{definition}[Accuracy-fairness Frontier Risk] Given a predictive function $f$, let $R(f|\alpha, n)\coloneqq \sum_{g\in \gG} \gamma_g R(f|G=g)$ be the standard empirical risk, and $\tilde{R}(f|\alpha, n)$ be the \textit{``fairness" risk} which is the worst-case risk among the groups $g\in \gG$:
$$\tilde{R}(f|\alpha, n) \coloneqq \sup_v \sum_{g\in \gG} [ v_g R(f|G=g)],$$ 
\vspace{-1.5em}

where $v \in \Delta^{|\gG|}$. Then, for non-negative weighting coefficients $\omega=\{\omega_1, \omega_2\}$, the accuracy-fairness frontier risk is defined as:
\begin{align}
F_{\omega}(f|\alpha, n) \coloneqq 
\omega_1 * R(f|\alpha, n) + \omega_2 * \tilde{R}(f|\alpha, n).    
\label{eq:frontier_risk}
\end{align}
\vspace{-2em}
\label{def:fairness_accuracy_frontier}
\end{definition}
% related work \citep{zhao2019inherent, menon2018cost, little2022fairness}

The form of the frontier risk in \Cref{def:fairness_accuracy_frontier} is common among objective functions in fairness literature, i.e., $F_\omega \propto R + \frac{\omega_2}{\omega_1} \tilde{R}$, where the standard risk $R$ is combined with a ``fairness constraint" $\tilde{R}$ under a trade-off parameter $\frac{\omega_2}{\omega_1}$. Then, for a fixed dataset, a point $(\tilde{r}, r^*)$ on the accuracy-fairness frontier can be identified by fitting a sequence of candidate models under different degrees of fairness-accuracy trade-off $\frac{\omega_2}{\omega_1}$, and then identify the best-achievable accuracy risk  $r^*$ among the models whose accuracy risk $\tilde{R}$ is less than $\tilde{r}$ \citep{little2022fairness}. Clearly, due to the Lagrangian form of \Cref{eq:frontier_risk}, a lower value of $F_\omega$ indicates a better accuracy-fairness tradeoff.

% In practice, a common goal is to search along the frontier to identify a model $f$ that attains the lowest fairness risk $\tilde{R}$ under the condition that its utility is above certain threshold (i.e., the standard risk $R > \lambda$). As we will show, this is equivalent to searching for a $f$ that minimizes \cref{eq:frontier_risk} under a particular value of $\frac{\omega_2}{\omega_1}$.

% When $\frac{\omega_2}{\omega_1}=1$, the frontier risk $F_{\omega}(f|\alpha, n)$ has a geometric interpretation as the perimeter of the rectangle defined by a point on the accuracy v.s. fairness trade-off curve (up to a scaling constant). 
% Given a trade-off level $\frac{\omega_2}{\omega_1}$, a model $f$ that attains a lower $F_\omega$ effectively attains a more advanced accuracy - fairness performance. 

To date, most of the prior work have focused on improving model performance by studying algorithms that better solve $\min_{f \in \gF} F_{\omega}(f|\alpha=\gamma, n)$ under a fixed (imbalanced) dataset \citep{martinez2020minimax, sagawa2019distributionally}, where $\gamma=\{\gamma_g\}_{g\in \gG}$ is the imbalanced group prevalences in the population. 

In this work, recognizing that the data imbalance can impose an inherent limitation on model performance 
%\citep{zhao2019inherent}
(i.e., \cref{eq:error_decomposition})
, we ask an orthogonal question: \textit{under a fixed learning algorithm, can we ``break" the accuracy-fairness frontier of the method by improving the distribution of the training data?} That is, we study the outer problem of the below optimization objective:
$$\alpha^* = 
{\color{Maroon} \argmin_{\alpha \in \Delta^{|\gG|}} }
\Big[ \min_{f \in \gF} F_{\omega}(f|\alpha, n) \Big]$$
where $\alpha \in \Delta^{|\gG|}$ is the allocation of group sizes in the training data. This question is of particular importance in active learning, {\color{red} because...}

In this section, our goal is to obtain an initial understanding of the potential impact of training data's group distribution in the resulting model's accuracy-fairness performance. Specifically, we would like to understand if and how a data group's population prevalence $\gamma_g$ and learning difficulty (in terms of finite-sample learning rate $o(c_g n^{-p_g})$) plays a role in the optimal distribution $\alpha^*$ that minimizes different fairness-relevant risk objectives. 

To maintain mathematical tractability in this initial analysis, we follow the previous literature to consider the below simple theoretical model for group-specific scaling laws for generalization error \citep{chen2018my, rolf2021representation}:

\begin{assumption}[Group-specific generalization error  \citep{rolf2021representation}]
The group-specific generalization error $R(f_{D}|G=g)=E_{D_g}(L(y, f_D))$ can be approximated by a scaling function of the group sample size $n_g$ and the total sample size $n$. That is, $\exists \, M_g >0$ and  constants $c_g, \tau_g, \delta_g \geq 0$, $p_g, q_g > 0$ such that for a dataset $D_{\alpha, n}$ with sample size $n$ and group allocation $\alpha=\{\alpha_g\}_{g\in \gG}$, and $f_{D_{\alpha, n}}$ the model trained $D$ with a particular algorithm, the generalization error $R(f_{D_{\alpha, n}}|G=g)$ can be approximated as:
\begin{align}
%\nonumber
R(f_{D_{\alpha, n}}|G=g) &\approx 
r(n_g, n | c_g, \tau_g, \delta_g, p_g, q_g) 
= c_g * n_g^{-p_g} + \tau_g * n^{-q_g} + \delta_g.
\label{eq:group_scaling_law}
\end{align}
The above is assumed to hold for any $\alpha \in \Delta^{|\gG|}$ and any $n$ such that $n_g = \lfloor \alpha_g n \rfloor \geq M_g$.
\vspace{-0.5em}
\label{def:group_scaling_law}
\end{assumption}
Assumption \ref{def:group_scaling_law} essentially states that each group has an unique learning rate $o(c_g n^{-p_g} + \tau_g n^{-q_g})$, which includes a $\tau_g n^{-q_g}$ term to allow data from other groups to influence the risk of group $g$. The scaling coefficients $(c_g, \tau_g, p_g, q_g)$ describes the difficulty of the learning problem, where higher values of $(c_g, \tau_g)$ and lower values of $(p_g, q_g)$ indicate that the group $g$ is more difficult to learn (i.e., the generalization error decreases slower with respect to sample size). Note that for common choices of loss function, we expect $p_g, q_g$ to be bounded in a small range (e.g.,  $p_g, q_g  < 1$ for squared loss, since the optimal parametric learning rate is $n^{-1}$ \citep{bach2017breaking}). It should be acknowledged that the Assumption \ref{def:group_scaling_law} is simplistic, as it assumes that the scaling coefficients $(c_g, \tau_g, p_g, q_g)$ are not impacted by the group composition of the training data $\alpha$. However, \citet{rolf2021representation} shows that it is indeed true in classic settings such as linear regression with group-specific intercepts {\color{red} (add more detail)}, and empirically verified that \cref{eq:group_scaling_law} approximated holds in, e.g., image classification tasks using ResNet models.

To this end, the below theorem 
% elucidates the importance of the training data's group-size allocation on the resulting model's fairness - accuracy performance. Importantly, \Cref{thm:optimal_allocation_frontier_main} theoretically
confirms that a model's fairness-accuracy frontier can be improved by careful design of the training data (i.e., by sufficiently representing data groups that are under-represented in the population). 
%This necessity notably does not vanish even under extremely large $n$, thereby highlighting the fact that the {\color{Maroon} \textit{data bias}} error in (\ref{eq:error_decomposition}) persists even in the asymptotics. 
Interestingly, it also provides a mathematical characterization for the heuristic notion of ``under-represented group" in the fairness literature (i.e., \cref{eq:minority_group_criteria_main}), in terms of whether a group's population prevalence $\gamma_g$ is comparable to its relative learning difficulty (as characterized by learning rate coefficients $c_g$, $p_g$ (\cref{eq:group_scaling_law})) when compared to the rest of the groups.

\begin{theorem}[Optimal Group-size Allocation for Fairness-Accuracy Frontier]
Assuming the group-specific scaling laws (Definition \ref{def:group_scaling_law}) differ only by the multiplicative coefficient $c_g$, so that the approximated group-specific risk is $\hat{R}(f_{D_{\alpha, n}}|G=g) \coloneqq c_g n^{-p} + \tau n^{-q} + \delta$. Denote the approximate population risk as $\hat{R}(\alpha, n) = \sum_g \gamma_g \hat{R}(f_{D_{\alpha, n}}|G=g)$ and the approximated worst-case risk as $\hat{\tilde{R}}(\alpha, n) = \sup_v \sum_{g\in \gG} [ v_g \hat{R}(f_{D_{\alpha, n}}|G=g)]$. Then:
\begin{itemize}[leftmargin=0.5cm]
\item [(I)] \textbf{(Population Risk},  \citet{rolf2021representation})  If  $F_{\omega=\{1,0\}}(\alpha, n)=R(\alpha, n)$ is the standard population risk. The optimal training-data group distribution $\alpha^*$ that minimizes $\hat{R}(\alpha, n)$ is
$\alpha^*_g = 
\frac{(\gamma_g c_g)^{1/(p+1)} }
{\sum_{g\in \gG}(\gamma_g c_g)^{1/(p+1)}}.$
\item [(II)] \textbf{(Worst-case Risk)} If  $F_{\omega=\{0, 1\}}(\alpha, n)=\tilde{R}(\alpha, n)$ is the worst-case risk. The optimal 
training-data group distribution $\tilde{\alpha}^*$ that minimizes $\hat{\tilde{R}}(\alpha, n)$ is
$\tilde{\alpha}^*_{g} = 
\frac{(c_g)^{1/p} }
{\sum_{g\in \gG}(c_g)^{1/p}}$, i.e., the relative learning difficulty of group $g$.
% \item [(III)] \textbf{(Fairness-Accuracy Frontier, Average-group Risk)} 
% Let $R_{fair}$ be the average-group risk $\bar{R}(\alpha, n)$ so that
% $F_{\omega}(\alpha, n) \coloneqq 
% \omega_1 * R(\alpha, n) + \omega_2 * \bar{R}(\alpha, n)$.
% The optimal training-set group-size allocation $\alpha^*$ that minimizes the approximated accuracy-fairness frontier $\hat{F}_\omega(\alpha, n)$ is: 
% \begin{align*}
% \alpha^*_g = \frac{(r_g c_g)^{1/(p+1)}}{\sum_{g\in \gG} (r_g c_g)^{1/(p+1)}}, 
% \quad \mbox{where} \quad
% r_g = \omega_1  \gamma_g + \omega_2 \frac{1}{|\gG|}.
% \end{align*}
\item [(III)] \textbf{(Fairness-Accuracy Frontier Risk)} 
For general $\omega>\mathbf{0}$, the optimal training-set group distribution $\alpha^*$ that minimizes the  $\hat{F}_\omega(\alpha, n) \coloneqq 
\omega_1 \hat{R}(\alpha, n) + \omega_2 \hat{\tilde{R}}(\alpha, n)$ is: 
\begin{align}
\alpha^*_g = \frac{(r_g c_g)^{1/(p+1)}}{\sum_{g\in \gG} (r_g c_g)^{1/(p+1)}}, 
\quad \mbox{where} \quad
r_g = \max\Big[
\gamma_g, \;\;
\Big(\frac{\omega_2}{\omega_1} + \sum_{g \in \gB} \gamma_{g} \Big)\Big( \frac{c_g^{1/p}}{\sum_{g \in \gB} c_g^{1/p}} \Big) \Big].
\label{eq:optimal_sampling}
\end{align}
Here $\gB \subseteq \gG$ is the set of under-represented groups whose population prevalence $\gamma_g$ satisfy:
\begin{align}
\gB \coloneqq 
\Bigg\{ g \Big|
\gamma_g \leq 
\Big(\frac{\omega_2}{\omega_1} + \sum_{g \in \gB} \gamma_{g} \Big)\Big( \frac{c_g^{1/p}}{\sum_{g \in \gB} c_g^{1/p}} \Big)
\Bigg\}.
\label{eq:minority_group_criteria_main}
\end{align}
Furthermore, a sufficient condition for $g \in \gB$ is
$\gamma_g 
< 
\frac{\omega_2}{\omega_1} * (\frac{c_g^{1/p}}{\sum_{g \in \gG} c_g^{1/p}})$, where
$\frac{c_g^{1/p}}{\sum_{g \in \gG} c_g^{1/p}}$ is the relative learning difficulty of group $g$, and $\frac{\omega_2}{\omega_1}$ the relative weights of the worst-case and population risks.
\end{itemize}
\label{thm:optimal_allocation_frontier_main}
\end{theorem}
Proof is in \Cref{sec:optimal_allocation_frontier_proof}. In the above, Part (I) (Population Risk) is due to \citet{rolf2021representation}, it shows a striking fact that the optimal group sizes $\alpha^*$ minimizing the approximated empirical risk is \textit{not} the empirical distribution $\gamma=\{ \gamma_g \}_{g \in \gG}$, thereby highlighting the importance of training data design in achieving optimality in even the standard generalization performance\footnote{In \Cref{thm:allocation_weighted_risk} 
(\Cref{sec:lemma}), we go beyond the previous work to show that in a more general setting where the group-specific scaling coefficient $p_g$ is not equal, the optimal sampling allocation $\alpha^*$ in fact disproportionally favors the more difficult-to-learn groups as $n \rightarrow \infty$.}. Parts (II)-(III) are new to this work. Specifically, (II) highlights that to optimize the model's fairness performance (as measured by worst-case risk $\tilde{R}$), the group sizes in the training data should be proportional to the group's inherent learning difficulty (as characterized by $c_g^{1/p}$), \textit{irrespective} to the prevalence of these groups in the population $\gamma_g$. Finally, (III) highlights that the accuracy-fairness trade-off under a fixed learning algorithm can be improved by properly sample the data groups.
%should be sampled according to whether it is \textit{under-represented}, i.e., if its population prevalence $\gamma_g$ does not sufficiently reflect its relative learning difficulty  {\scriptsize $c_g^{1/p}/(\sum_g c_g^{1/p})$} (\cref{eq:minority_group_criteria_main}).
In particular, under the assumption that we have oracle knowledge of the scaling laws $c_g n_g^{-p} + \tau n^{-1} + \delta$, Part (III) hints at a sampling procedure that guarantees optimality: Given a data group $g \in \gG$, if $g$ doesn't belong to the under-represented group $\gB$, sample it  according to a likelihood function that is proportional to population prevalence $\gamma_g$, otherwise sample it according to a likelihood function (\cref{eq:optimal_sampling}) that is lower bounded by the group's relative learning difficulty $c_g^{1/p}/(\sum_g c_g^{1/p})$ scaled by the relative weight of the fairness and accuracy risks $\omega_2 / \omega_1$. 

{\color{red} Outline for transitioning paragraph below:}

{\color{red}
Begs the question.
\begin{enumerate}
    \item how to sample when group membership / group-specific scaling law are not known? Answer: use generalization error. empirically verified by \citep{liu2021just}.
    \item how to sample in active learning. where the generalization error is not known for sampling candidates? Answer: introspective training. Importantly, not only provides an estimate of generalization error, but also a guanrantee in bias-awareness.
    Improve uncertainty-sampling performance.
\end{enumerate}
}
 
{(Introduce Introspective Self-play)

Intuition: predict under-represented group / generalization error.

Deep implication in uncertainty-awre active learning under dataset bias: 
\begin{itemize}
    \item Injects bias-awareness into model representation.
    \item Improves bias-awareness in uncertainty quantification.
\end{itemize}
Improved model uncertainty under dataset bias / spurious correlation.
}
